Characteristic Gluing with $\Lambda$: II. Linearised equations in higher dimensions

We prove a gluing theorem for linearised vacuum gravitational fields in Bondi gauge on a class of characteristic hypersurfaces in static vacuum $(n+1)$-dimensional backgrounds with cosmological constant $ \Lambda \in \mathbb{R}$, $n\ge 4$. This generalises, in the linearised case, the pioneering analysis of Aretakis, Czimek and Rodnianski, carried-out on light cones in four-dimensional Minkowski spacetime.

==> CKVonS.tex <==

\subsubsection{Example on $S^{n-1}$}
 \label{ss26X23.1}

On $S^{n-1}$ the functions $\zspaceD_A\chi^A $ are linear combinations of $\ell=1$ spherical harmonics, and so \eqref{4X23.1} will fail unless the projection of $\zspaceD_A \xi^A$ on the space spanned by $\ell=1$ harmonics vanishes:
%
\begin{equation}\label{4X23.3}
  (\zspaceD^A \xi_A )^{[=1]} = 0
  \,.
\end{equation}
%
Now, the proper conformal Killing vectors are gradients of $\ell=1$ spherical harmonics. So let $\chi_A = \zspaceD_A \varphi \in \CKV$, since  $\xi_A\in \CKVp$ by hypothesis we have for all such $\chi_A$'s
%
\begin{equation}\label{4X23.4}
  0 =  \int_{\dmanif} \xi^A \zspaceD_A \varphi
    \,\sm =  - \int_{\dmanif}  \varphi \zspaceD_A\xi^A
    \,\sm
    \,,
\end{equation}
%
which implies that \eqref{4X23.3} holds.

Note that this calculation shows that, on $S^{n-1}$, we have
%
\begin{equation}\label{4X23.5}
  \xi_A^{[S]}=\zspaceD_A\phi \in \CKVp
  \qquad
  \Longleftrightarrow
  \qquad
   \phi = \phi^{[> 1]}
   \,,
\end{equation}
%
up to the addition of (an irrelevant) constant to $\phi$.




==> ContinuityBefore11IV24.tex <==
\subsection{Regularity}
 \label{s18VIII23.1}
 \ptcr{section completely rewritten 5IV24; old version in  ContinuityOld}
The gluing construction of~\cite{ACR1,ACR2,ACR3}  requires a deformation of the section $\secNtwo$ of $\mcN$ in the spacetime $(\mcMtwo,\fourgtwo)$, as well as $u$-derivatives of this deformation, as needed to control some of the gauge-dependent radially conserved charges. One needs furthermore to include in the construction a diffeomorphism $\Phi^A$ of $\secN$, as well as its $u$-derivatives. Last but not least, one  needs to make sure that  the regularity of the resulting fields on the deformed co-dimension-two submanifold, say $\secNtwoNew$, is consistent with the characteristic constraint equations and their $u$-derivatives.

 \ptc{macros $\fr$ and  $\secNtwoNew$,  different from $\zsecN$,since needs adjusting for $r$, to be checked for consistency}
The new section $\secNtwoNew$  will be  given by the equations
%
\begin{equation}\label{30III24.1}
 \secNtwoNew=\{
    u =f(x^A)
   \,,
  \
    r=\fr(x^A)
    \}
   \,.
\end{equation} 
% 
We  suppose that there exists a large  $k_\gamma$, with threshold to be made precise during the argument,
 \ptc{....}
 so that 
%
\begin{equation}\label{16VII23.3} 
 f \in H_{k_\gamma+2 }(\secN)
   \,,
   \qquad
   \fr  \in H_{k_\gamma+ ????}(\secN)
       \,.
\end{equation}
% 
 
The gauge transformations on $\secN$ will be implemented by a map $\Phi^A:=\Phi^A_1$  which is the  $t=1$ solution of the flow
%
\begin{equation}
 \frac{d\Phi^A_t}{dt}(x^B) = X^A\big(\Phi_t(x^B)\big)
  \,,
  \qquad
  \Phi^A_0(x^B)=x^A
  \,,
  \label{5IV24.2}
 \end{equation}
% 
 with $X^A$ 
 of the form
%
\begin{equation}\label{5IV24.3}
  X^A(u,x^B) = \os{X}{0}^A(x^B)
  +  \os{X}{2}^A(x^B)\big(u-f(x^A)\big)
   + \ldots
  +  \os{X}{k}^A(x^B)\frac{\big(u-f(x^A)\big)^k}{k!}
  \,,
\end{equation} 
%
with vector fields $ \os{X}{i} \in H_{k_\gamma+1-2i }(\secN)$. Thus
%
\begin{align}\label{5IV24.5}
  X^A|_\zsecN 
   & =  
    \os{X}{0}^A \in H_{k_\gamma+1 }(\secN)
   \,, \quad
  \partial_uX^A|_\zsecN =  \os{X}{1}^A \in H_{k_\gamma-1 }(\secN)
   \,, \quad
   \ldots\,, 
   \nonumber
\\    
  \partial_u^kX^A|_\zsecN 
  & =  \os{X}{k}^A \in H_{k_\gamma+1-2k }(\secN)
  \,.
\end{align}
%
This implies
%
\begin{align}\label{5IV24.5b}
  \Phi^A|_\zsecN   \in H_{k_\gamma+1 }(\secN) 
   \,, \quad
 \partial_u \Phi^A|_\zsecN   \in H_{k_\gamma-1 }(\secN) 
   \,, \quad
   \ldots 
   \,,
   \quad
  \partial_u^k\Phi^A|_\zsecN  
   \in H_{k_\gamma+1-2k }(\secN)
  \,.
\end{align}
%
We set
 \ptc{at the end use extensions to make things elegant or if needed; checkwith Hoermander}
%
\begin{align}
    \zx^A (u,x^B) & =
     \Phi^A (u,x^B) 
    \,.
    \label{6IV24.1}
\end{align}
%

Next, for $u$ near $f$ we set 
%
\begin{align} 
   \zu(u,x^A)  &=  \psi_1(x^A )
    \big( u- f (x^A)\big) 
     + \psi_2(x^A )
   \frac{ \big( u- f (x^A)\big)^2}2 
        + \ldots
  % ( \psi_1 \circ \Phi )( u- f \circ \Phi)
%     + 
%   ( \psi_2 \circ \Phi) \frac{( u- f \circ \Phi)^2}2 
%        + \ldots
         \nonumber
 \\
  &        
    + 
      \psi_k(x^A )
   \frac{ \big( u- f (x^A)\big)^k}{k!} 
   % \frac{\psi_k(x^A)}{k!} (  u- f(x^A) )^k
    \,,
     \label{15IX23.1}
\end{align}
% 
with functions $\psi_i \in H_{k_\gamma+2-2i }(\secN)$, and where $\psi_1 >0$. 
 We find 
%
\begin{align}\label{5IV24.5}
  \zu|_\zsecN 
   =   0
   \,,  
   \quad
  \partial_u\zu |_\zsecN
    =   \psi_1 
    \in H_{k_\gamma  }(\secN)
    \,,
    \quad
    \ldots
    \,,
    \quad
  \partial_u^k \zu|_\zsecN 
  =
  \psi_k
    \in H_{k_\gamma+2-2k }(\secN)
  \,.
\end{align}
%

 We restrict attention to the region where 
 %
 $  \{\zu=0\}
 $
 %
 coincides with $\{u=f\}$. 
On $\{r=r_2\}$ we replace the coordinates $(u,x^A)$ by a new set of coordinates $(\zu,\zx^A )$, and we define the coordinates $(\cu,\checkr,\cx^A)$ by setting $\checkr = r$ and  flowing along the null geodesics orthogonal to $\{u=f\,,\, r=r_2\}$, as above.  

 
For simplicity we  assume that the metric $\fourg_2$ is of the form
 \ptc{nu r changed to exp 2 beta, but not consistent with the other section...}
%
\begin{equation}
   \fourg_2
    = -\alpha du^2 - 2\red{e^{2\beta}}  du dr  + g_{AB} dx^A dx^B
      \,,
%      \quad
%       \red{e^{2\beta}}>0
%       \,,
     \label{19VII23.11asdf}
\end{equation}
%
and is smooth near $\zsecN$. Now, \eqref{20III221bcd}
shows that to understand the regularity of the metric in the $\mtdx$-coordinates we need the derivatives $\partial_{\mtdx^\mu} x^\nu$. These can be obtained by inverting the Jacobi matrix  $\partial_{x^\mu} \mtdx^\nu$, but for this the $\partial_r \mtdx^\nu$-derivatives are still missing.
So we proceed now to determine these.

% in the relevant region before the coordinate transformation \eqref{6IV24.1}-\eqref{15IX23.1} has been applied.
\ptc{I don't know how to do it without null.tex }
%commented out, direct calculation of radial derivatives from the null normals, but seems that this is not needed}
\input{nullWithr}



Then for $0\le i\le \bzk$ it holds that:
 \ptcr{2 VI 24: not updated yet from now on, please ignore}

\begin{enumerate}

\item  The partial derivatives $\partial_u^i\lowX_A$ of  the vector field defined in \eqref{8IV24.3}are of differentiability class $H_{k_\gamma-1-2i}(\secN)$.

\item The partial derivatives $\partial_u^i\partial_r \mtdx^\mu|_{\secNtwo}$ are in  $H_{k_\gamma-2i}(\secN)$ by 
    \eqref{14IX23.1a}-\eqref{14IX23.1b} together with \eqref{30III24.10}.
     \ptc{this misses r}
     \ptcr{the radial derivative do not match our interior assumptions when i is not zero, but perhaps this is not a problem?}

\item It now follows that all the entries of the Jacobi matrix $\partial \mtdx^\alpha/ \partial x^\beta|_{\secNtwo}$
 are in $H_{k_\gamma}(\secN)$ or better. Hence all the entries of the matrix
    $\partial x^\alpha/ \partial \mtdx^\beta|_{\zsecN }$, which is the inverse of
    ${ \partial \mtdx^\alpha}/{\partial x^\beta}  |_{\secNtwo}$,
    are also in $H_k(\secN)$. Subsequently we find that 
    %
    \begin{equation}\label{13IX23.4}
      \partial^i_u
       \left( \frac{ \partial x^\alpha}{\partial \mtdx^\beta}
      \right)
      \Big|_{\zsecN} \in H_{k_\gamma -2i}(\secN)
      \,.
    \end{equation}
    %
    It further follows from
    %
 $$
     \frac{\partial}{\partial \mtdx^B} =
     \frac{\partial u }{\partial \mtdx^B}  \partial_u +
     \frac{\partial x^A }{\partial \mtdx^B} \partial_A
     \,,
     \qquad
     \frac{\partial}{\partial \mtdu} =
     \frac{\partial u }{\partial \mtdu}  \partial_u +
     \frac{\partial x^A }{\partial \mtdu} \partial_A
     \,,
$$
%
that
    %
    \begin{equation}\label{13IX23.4b}
      \partial^i_\mtdu
       \left( \frac{ \partial x^\alpha}{\partial \mtdx^\beta}
      \right)
      \Big|_{\zsecN} \in H_{k_\gamma -2i}(\secN)
      \,.
    \end{equation}
    %


  \item  The definition \eqref{20VII23.w1} of $\ysqr$ shows that $\partial_u^i\ysqr|_{\secNtwo} \in  H_{k_\gamma -2i }(\secN)$.
   \ptcr{actually one better if Lambda is the identity?}
  \item This propagates through \eqref{18VIII23.f1}-\eqref{18VIII23.f2}
to give
 \ptc{but this we already knew from the above, something needs rewriting, but in any case this appears to be correct albeit duplicate; perhaps clearer than the previous argument?}
%
$$
 \mbox{$\partial_u^i U_{\mtdr}|_{\secNtwo} \in  H_{k_\gamma -2i }(\secN)$
   and $\partial_u^i X^A_{\mtdr}|_{\secNtwo}\in  H_{k_\gamma -2i }(\secN)$.}
 $$
 %
 \item Equation \eqref{20III221bcd} shows now that
  \ptcr{problem with g u r?}
 %
 \begin{eqnarray}
  &
    \partial_u^i g_{\mtdu\mtdu} |_{\secNtwo} \in  H_{k_\gamma-1 -2i }(\secN)
    \,,
    \qquad
    \partial_u^i g_{\mtdu\mtdA} |_{\secNtwo} \in  H_{k_\gamma-1 -2i }(\secN)
    \,,
    &
    \nonumber
 \\
 &
    \partial_u^i g_{\mtdu\mtdr} |_{\secNtwo} \in  H_{k_\gamma-1  -2i }(\secN)
    \,,
    \qquad
    \partial_u^i g_{\mtdA\mtdB} |_{\secNtwo} \in  H_{k_\gamma  -2i }(\secN)
    \,.
    &
     \label{13IX23.1}
 \end{eqnarray}
 %

 \item Finally,  the differentiability properties of the metric components need to be reexamined as functions of the new coordinates $(\mtdu,\mtdx^A)$. Indeed, we have on $\mcHtwo$
    %
    \begin{equation}\label{13IX23.3}
      \partial_{\mtdA} g_{\mtdu\mtdu} =  U_{\mtdA} \partial_u g_{\mtdu\mtdu}
      + \Lambda^B{}_ {\mtdA}  \partial_B g_{\mtdu\mtdu}
      \,,
      \qquad
      \partial_{\mtdu} g_{\mtdu\mtdu} =  U_{\mtdu} \partial_u g_{\mtdu\mtdu}
      + X^A_{\mtdu}  \partial_A g_{\mtdu\mtdu}
      \,,
    \end{equation}
 %
 similarly for the remaining metric functions. This leads to
  \ptcr{not done yet}
 %
 \begin{eqnarray}
  &
    \partial_u^i g_{\mtdu\mtdu} |_{\secNtwo} \in  H_{k_\gamma-1 -2i }(\secN)
    \,,
    \qquad
    \partial_u^i g_{\mtdu\mtdA} |_{\secNtwo} \in  H_{k_\gamma-1 -2i }(\secN)
    \,,
    &
    \nonumber
 \\
 &
    \partial_u^i g_{\mtdu\mtdr} |_{\secNtwo} \in  H_{k_\gamma-1  -2i }(\secN)
    \,,
    \qquad
    \partial_u^i g_{\mtdA\mtdB} |_{\secNtwo} \in  H_{k_\gamma  -2i }(\secN)
    \,.
    &
     \label{13IX23.2}
 \end{eqnarray}

\end{enumerate}






==> EndInduction.tex <==

\subsubsection{Continuity of $\partial_u^{i}\tilde\hBo_{uA}$}
 \label{ss15X21}
 
{\redca{10VII, moved here from the end of the section} 
While this is not needed for the current argument, we note that a  conserved, gauge dependent, radial charge involving  $\partial_u h_{uA}$   is derived in Appendix~\ref{sApp14IV23.2}. 

To continue, let
}
 $k$ be the order at which we want to perform the gluing, i.e.\ the number of $u$-derivatives of $h_{\mu\nu}$ which we want to be continuous, and let $1\le {p}\le k$.

\paragraph{{\underline{The case $m=0$:}}} After performing a gauge transformation, Equation \eqref{18VI22.1} at order $i={p}$ together with \eqref{26IX22.1i} provides a gluing equation of the form, 
%
\begin{align}
    \partial_u^{{p}}
    \zhTB_{uA}|_{\tilde\secN_2}
    &=
     -
    \frac{1}{ 2r_2^2}
    \Done (\zspaceD^C\partial_u^{{p}-1}\kxi{2}{}_C)
    -\Big(\partial_u^{{p}+1}\kxi{2}{}_A
     +  \frac{\alpha^2}2
      \zspaceD_A\zspaceD^C\partial_u^{{p}-1}\kxi{2}{}_C\Big)
    + \overset{({p})}{X}_A%(u,r,x^A)
    \nonumber
\\
    &\qquad
    + \sum_{0\leq j+\ell \leq {p},\ell \ne {p}}
 \overset{({p},j,\ell)}{\chi}
 (r)\partial_r^j \zspaceD^B P^{\ell} \hBo_{AB}
    + \sum_{0\leq j+\ell \leq {p},\ell \ne {p}}
 \overset{ ({p},j,\ell) }{\chi}(r)
 \partial_r^j \zspaceD^B P^{\ell} \Big(2r^2C(\kzeta{2})_{AB}\Big)
               \nonumber
\\
    &\qquad
    + \sum_{j=0}^{{p}}\zspaceD^B\int_{r_1}^{r_2} \overset{({p},j)}{\chi}(r_2)P^j \tilde\hBo_{AB}(s)\, ds
    \nonumber
\\
    &=
    \left\{
      \begin{array}{ll}
 \displaystyle
 \overset{({p})}{\tilde X}_A
    + \sum_{j=0}^{{p}} \sum_{\ell = 1}^{{p}+4}\zspaceD^B\int_{r_1}^{r_2} \overset{({p},j)}{\ochi}_{\ell}(r_2) \hkappa_{\ell}(s) P^j \wh_{AB}(s)\, ds,
 & \hbox{${p}\le k-2$;}
\\
 \displaystyle
          -\partial_u^{{p}+1}\blue{\kxi{2}{}_A }
     +
         \overset{({p})}{\tilde X}_A
    + \sum_{j=0}^{{p}} \sum_{\ell = 1}^{{p}+4}\zspaceD^B\int_{r_1}^{r_2} \overset{({p},j)}{\ochi}_{\ell}(r_2) \hkappa_{\ell}(s) P^j \wh_{AB}(s)\, ds,
    \quad
    & \hbox{${p}=k-1,k$,}
      \end{array}
    \right.
     \nonumber
\\
    &= \left\{
         \begin{array}{ll}
 \displaystyle
 \overset{({p})}{\tilde X}_A
    + \sum_{j=0}^{{p}} \sum_{\ell = 1}^{{p}+4} \overset{({p},j)}{\ochi}_{\ell} (r_2)\zspaceD^B P^j  \kphi{\ell}^{[\TTt^\perp]}_{AB} ,
   & \hbox{${p}\le k-2$;} \\
 \displaystyle
            -\partial_u^{{p}+1}\blue{\kxi{2}{}_A}
     + \overset{({p})}{\tilde X}_A
    + \sum_{j=0}^{{p}} \sum_{\ell = 1}^{{p}+4} \overset{({p},j)}{\ochi}_{\ell} (r_2)\zspaceD^B P^j  \kphi{\ell}^{[\TTt^\perp]}_{AB},\qquad
 & \hbox{${p}=k-1,k$.}
         \end{array}
       \right.
    \label{6X22.w8}
\end{align}
%.
 \ptcheck{20X22}
Here we used the fact that the fields   $\partial_u^{\ell }\kxi{2}{}_C^{{[\CKVp]}}$ with $\ell \le k-1$ are already known  from Section~\ref{s10IX22.1}, and   included them, together with all
other already known fields, in  $\overset{({p})}{\tilde X}_A =\overset{({p})}{\tilde X}_A(r,x^A) $.
Recall that $ \kphi{1}_{AB}$ has been determined in Section~\ref{ss3VIII22.1}, $ \kphi{4}_{AB}$  in  \eqref{29VII22.1}, and we further set
%
$$
\kphi{2}_{AB}=\kphi{3}_{AB}
 = 0
 \,.
$$
%
For the sake of induction, suppose  that the fields $ \kphi{\ell}_{AB}$ with $4\le \ell \le {p}+3$ are known.
\ptchd{the fields $\kphi{\ell}^{[\leq \ell-3]}_{AB}$ in fact remains free \\ -- \\ ptc: do you see a mechanism to exploit this?}
 Together with $\overset{({p})}{\tilde X}_A  $ and $\partial_u^p\zhTB_{uA}|_{\tilde\secN_2}$ we collect them   into a term $\overadd{{p}}{\hat {\tilde X}}_{A}$, so that the requirement that $\partial_u^{{p}} \tilde h_{uA}$ be continuous at $r_2$  results in an equation of the form 
  \ptcr{should be $\kphi{{p}+4}^{[\kerLrpp]}_{AB}$? but careful how this fit with the remaining arguments}
%
\begin{align}
   \zspaceD^B\Big(
    \underbrace{
   \sum_{j=0}^{{p}}  \overset{({p},j)}{\ochi}_{{p}+4} (r_2)  P^j 
   }_{=:\kchi{p}(P)} 
   \kphi{{p}+4}^{[\TTt^\perp]}_{AB}
   \Big)
     	 &=
        \left\{
         \begin{array}{ll}
            - \overadd{{p}}{\hat {\tilde X}}_{A} ,
   & \hbox{${p}\le k-2$;} \\
 \displaystyle
             \partial_{\tdu}^{{p}+1} \xiA{2}
            - \overadd{{p}}{\hat {\tilde X}}_{A},
            \qquad
 & \hbox{${p}=k-1,k$.}
         \end{array}
       \right.
    \label{24X22.91}
\end{align}
%
Now, the operator at the left-hand side of this equation, 
namely 
%
$$
 L_p := \zdivtwo \circ \kchi{p}(P)
  \,,
$$
%
has a non-trivial cokernel. For instance, on $S^2$,  the cokernel is $30$-dimensional when ${p}=2$ and  $48$-dimensional when ${p}=3$.  Indeed, the cokernel on $S^2$ is the space of spherical harmonic vectors with index $1\le \ell \le {p}+1$, see Appendix \ref{ss27XI22.1}. 
For all $p\le k$ we can therefore find a unique $ \kphi{{p}+4}^{[\kerLrpp]}_{AB}$
satisfying
%
\begin{equation}\label{10VII23.5}
  \big( L_p (\kphi{{p}+4}^{[\kerLrpp]})
  \big)_{A} = 
  -  
   \overadd{{p}}{\hat {\tilde X}}{}_{A} 
    ^{[\kerLrpp]}
    \,.
\end{equation}
%
For $p\le k-1$ the $\imLrp$-part of $\overadd{{p}}{\hat {\tilde X}}_{A} $ constitutes thus a further obstruction to the solvability of  \eqref{24X22.91}, as it is not clear whether or not the right-hand side is orthogonal to the cokernel.

However, if $p=k$ or $k+1$,  since the fields $ \partial_{\tdu}^{k } \xiA{2}$ and $ \partial_{\tdu}^{k+1} \xiA{2}$ are unconstrained so far, we can use \eqref{24X22.91} to choose these fields  so that continuity of $\partial_u^{k-1} \tilde h_{uA}$ and $\partial_u^{k} \tilde h_{uA}$ at $r_2$ holds:
%
\begin{equation}\label{10VII23.6}
 \imLrp \ni 
  \partial_{\tdu}^{{p}+1} \kxi{2}_A %{}^{[\kerLrp]}_A
             :=  
              \overadd{{p}}{\hat {\tilde X}}{}_{A}
              ^{[\imLrp]}
               \,.
\end{equation}
%

\paragraph{The case $m\neq 0$:} After performing a gauge transformation, Equation \eqref{18VI22.1} at order $i={p}$ together with \eqref{26IX22.1i} provides a gluing equation of the form,
 \ptcr{where is the X p term? other ones are ok}
 \ptcheck{19XI22, and rechecked by wan 20XI}
%
\begin{align}
    \partial_u^{{p}}
    \zhTB_{uA}|_{\tilde\secN_2}
    &=
     -
    \frac{1}{ 2r_2^2}
    \Done (\zspaceD^C\partial_u^{{p}-1}\kxi{2}{}_C)_A
   -
     \partial_u^{{p}+1}\kxi{2}{}_A
      {
      -  \big(\frac{\alpha^2}2 + \frac{m}{r^3}
     \big)
     }
      \zspaceD_A\zspaceD^C\partial_u^{{p}-1}\kxi{2}{}_C
    + \overset{({p})}{X}_A%(u,r,x^A)
    \nonumber
\\
    &\qquad
    + \sum_{0\leq j+\ell \leq {p},\ell \ne {p}}
 \overset{({p},j,\ell)}{\chi}
 (r)\partial_r^j \zspaceD^B P^{\ell} \hBo_{AB}
    + \sum_{0\leq j+\ell \leq {p},\ell \ne {p}}
 \overset{ ({p},j,\ell) }{\chi}(r)
 \partial_r^j \zspaceD^B P^{\ell}
 \Big(
  2r^2C(\kzeta{2})_{AB}\Big)
               \nonumber
\\
    &\qquad
    + \sum_{j=0}^{{p}}\zspaceD^B\int_{r_1}^{r_2} \overset{({p},j)}{\chi}(r_2)P^j \tilde\hBo_{AB}(s)\, ds
    \nonumber
\\
    &=
    -\partial_u^{{p}+1}\kxi{2}{}_A
    +
 \overset{({p})}{\tilde X}_A
    + \sum_{j=0}^{{p}} \sum_{\ell = 1}^{{2p}+4}\zspaceD^B\int_{r_1}^{r_2} \overset{({p},j)}{\ochi}_{\ell}(r_2) \hkappa_{\ell}(s) P^j \wh_{AB}(s)\, ds
     \nonumber
\\
    &=
    -\partial_u^{{p}+1}\kxi{2}{}_A
    +
 \overset{({p})}{\tilde X}_A
    + \sum_{j=0}^{{p}} \sum_{\ell = 1}^{{2p}+4} \overset{({p},j)}{\ochi}_{\ell} (r_2)\zspaceD^B P^j  \kphi{\ell}_{AB}\,,
    \label{6X22.w8b}
\end{align}
%
where  we  assumed that the fields $\partial_u^{j}\kxi{2}{}_A$ for $j\leq p$ have been determined in terms of known fields, and have collected these, together with all other already known fields, into $\overset{({p})}{\tilde X}_A$. For the sake of induction, we shall also assume that the fields
$\kphi{\ell}_{AB}$ for $\ell\leq 2p+2$ are known
  and collect them, together with $-\partial_u^p\zhTB_{uA}|_{\tilde\secN_2}$, into a new term $\overset{({p})}{\hat{\tilde X}}_A$, allowing us to rewrite
  the $L^2$-projections on $\CKV$ and $\CKVp$ of
  \eqref{6X22.w8b} respectively as
%
\begin{align}
 \partial_u^{p+1}\kxi{2}{}_A^{[\CKV]}
 & =
 \overset{({p})}{\hat{\tilde X}} {}^{[\CKV]}_A
    \,,
    \label{9XI22.w1a}
\\
 -  \overset{({p},0)}{\ochi}_{2p+4} (r_2)\zspaceD^B  \kphi{2p+4}{}^{[\TTt^\perp]}_{AB}
 &
  =
 -\partial_u^{{p}+1}\kxi{2}{}^{[\CKVp]}_A
    +
 \overset{({p})}{\hat{\tilde X}}{{}^{[\CKVp]}_A}
    \nonumber
\\
    &\quad
    + \zspaceD^B (\overset{({p},0)}{\ochi}_{2p+3} (r_2) + \overset{({p},1)}{\ochi}_{2p+3} (r_2) P)\kphi{2p+3}{}^{[\TTt^\perp]}_{AB}
    \,.
    \label{9XI22.w1}
\end{align}
%
 \ptcr{this should now be based on hat L?}
An argument identical to that below \eqref{18X22.1} shows that,
   both on $S^2$ and $\T^2$,
  \eqref{9XI22.w1a} determines $\partial_u^{p+1}\kxi{2}{}_A^{[\CKV]}$ uniquely in terms of $\overset{({p})}{\hat{\tilde X}}{{}^{[\CKV]}_A}$ while \eqref{9XI22.w1} determines  $\kphi{2p+4}{}_{AB}^{[\TTt^\perp]}$ uniquely in terms of $\overset{({p})}{\hat{\tilde X}}{{}^{[\CKVp]}_A}$, $\kphi{2p+3}{}^{[\TTt^\perp]}_{AB}$ and $\partial_u^{p+1}\kxi{2}{}_A^{[\CKVp]}$; the fields $\kphi{2p+3}{}^{[\TTt^\perp]}_{AB}$ and $\partial_u^{p+1}\kxi{2}{}_A^{[\CKVp]}$ remain free to use for
  other gluing equations. On negatively curved sections with higher genus, \eqref{9XI22.w1} determines $\kphi{2p+4}{}^{[\TTt^\perp]}_{AB}$ in terms of $\overset{({p})}{\hat{\tilde X}}_A$, $\kphi{2p+3}{}^{[\TTt^\perp]}_{AB}$  and $\partial_u^{p+1}\kxi{2}{}_A^{[\CKVp]}=\partial_u^{p+1}\kxi{2}{}_A$, with the fields $\kphi{2p+3}{}^{[\TTt^\perp]}_{AB}$ and $\partial_u^{p+1}\kxi{2}{}_A$
   remaining free.


%\subsubsection{Gluing equation for $\partial_u^{{p}} \hBo_{uu}$}
% \ptcr{maybe not needed anymore?}
%
%We set the field $\partial^{{p}}_u \hBo_{uu}$ on $\mcN_{(r_1,r_2)}$ by imposing
%%
%\begin{equation}
%   \partial_r  \kochi{{p}+1}|_{\mcN_{(r_1,r_2)}} =
%   0\,,
%\end{equation}
%%
%with initial value $\kochi{{p}+1}[\dt_{\tilde{\secN}_1}]$ at $r_2$.
%
%\ptcr{change the last step in the induction to have no obstructions at $\Ctwo$, and somewhat less obstructions at higher dims}



==> Family.tex <==
%
 \ptcr{Family.tex, to be synchronised eventually with the nonlinear paper}
{\redc
\begin{equation}\label{4V24.1}
   \left\{
     \begin{array}{ll}
%       \mbox{Kerr metrics}, & \hbox{when $\Lambda =0$, $\secN\approx S^2$;} \\
       \mbox{Kerr-(A)dS metrics}, & \hbox{when $\Lambda \in \R$, $\secN\approx S^{n-1}$, $n\ge 3$;} \\
 %      \mbox{Myers-Perry metrics}, & \hbox{when $\Lambda =0$, $\secN\approx S^{n-1}$, $n\ge 4$;}\\
       \mbox{Birmingham-Kottler metrics}, & \hbox{when $\Lambda\in \R$, $R(\zgamma) <0$, $n\ge 3$.}
     \end{array}
   \right.
\end{equation}
% 
\ptcr{and perhaps: odd $n$ and Kerr-AdS with negatively curved; and maybe Klemm but not clear} 
} 

==> Family2.tex <==
%
{\redc
\begin{equation*}\label{4V24.1v2}
   \left\{
     \begin{array}{ll}
%       \mbox{Kerr metrics}, & \hbox{when $\Lambda =0$, $\secN\approx S^2$;} \\
       \mbox{Kerr-(A)dS metrics}, & \hbox{when $\Lambda \in \R$, $\secN\approx S^{n-1}$ or a quotient thereof, $n\ge 3$;} \\
 %      \mbox{Myers-Perry metrics}, & \hbox{when $\Lambda =0$, $\secN\approx S^{n-1}$, $n\ge 4$;}\\
       \mbox{Birmingham-Kottler metrics}, & \hbox{when $\Lambda\in \R$, $R(\zgamma) <0$, $n\ge 3$.}
     \end{array}
   \right.
\end{equation*}
%  
} 
 

==> HDBianchi.tex <==
The divergence identity
%
\begin{eqnarray}
  0 &\equiv & \nabla_\mu \delta \red{\mcE}^{\mu}{}_A
    \nonumber
\\
 &= &
 r^{-2}\partial_r(r^2  \delta \red{\mcE}^r{}_A)
   + \partial_u \delta \red{\mcE}^u{}_A
    + \zspaceD_B \delta \red{\mcE}^B{}_A
 \,,
 \label{2X22.6}
\end{eqnarray}
%
together with its $u$-derivatives,
shows that we also have
%
\begin{eqnarray}
 \forall \
  0 \le i \le k \qquad
  0 & =  &
   \Big(
  r^{-2}\partial_r(r^2  \partial_u^i\delta \red{\mcE}^r{}_A)
    + \zspaceD_B \partial_u^i\delta \red{\mcE}^B{}_A
    \Big)\Big|_{\blue{\mcN_{[r_0,r_2)}}}
 \,.
  \label{1X22.3}
\end{eqnarray}
% 

==> HDKappas.tex <==
\section{Constructing the $\kappa_i$'s}
 \label{App13VIII22.1}
\ptcr{most of this is duplicate except for adding logs, to discard if logs are not added; to reword if kept}

Recall that $\hat \kappa_i(s)=s^{-i}$.

We wish to construct a  sequence  of smooth functions $\red{\kappa}_i$  compactly supported in $(r_1,r_2) $ satisfying
%
\begin{eqnarray}
  &
  \displaystyle
\ip{\kappa_i}{\hat \kappa_j} \equiv
\int_{r_1}^{r_2} \kappa_i(r) \hat \kappa_j(r) \, dr = 0
 \quad \mbox{for $j<i$}
  \,,
  &
  \label{13VIII22.1}
   \\
   &
  \displaystyle
 \ip{\kappa_i}{\hat \kappa_i}  = 1
  \,.
  &
  \label{13VIII22.2}
\end{eqnarray}
%
This can be done as follows:
  Let $\red{\chi}$ be any smooth  non-negative function supported away from neighborhoods of $\red{r}_1$ and $\red{r}_2$, with integral 1. Let
   \ptcr{clash of notation chi}
  %
  $$
   \red{\kappa}_i  = c_i \red{\chi} f_i
   \,,
   $$
   %,
   where the $f_i$'s are constructed by a Gram-Schmidt orthonormalisation procedure from the family of monomials in $1/r$, namely $\{1,\red{r}^{-1},\red{r}^{-2},\ldots\}$, in the space $\mathbb{H}:= L^2([\red{r}_1,\red{r}_2],\red{\chi} d\red{r})$,
    so that
    the scalar product is
%
$$
 \langle \phi,\psi\rangle_{\mathbb{H}}  =
  \int_{\red{r}_1}^{\red{r}_2} (\phi \psi \red{\chi})(r) \, dr
  \,,
$$
%
and the $c_i$'s are constants  chosen so that
\eqref{13VIII22.2} holds; the possibility of doing so will be justified shortly.
Then, by construction, $f_i$ is a polynomial of order $i$ in $1/r$ which is $\mathbb{H}$-orthogonal to any such polynomial of order $j<i$; this  is precisely \eqref{13VIII22.1}.
As for \eqref{13VIII22.2}, we note that each of the functions
$\red{r}^{-i}$ can be decomposed in the basis $\{f_j\}_{j\in\N}$ as $\red{r}^{-i}= \sum_{j=0}^i a_{ij} f_j(\red{r})$, with $a_{ii}\ne 0$ since otherwise the right-hand side would be a polynomial in $1/r$ of order less than or equal to $i-1$.
This  shows that
%
$$
 \int_{\red{r}_1}^{\red{r}_2}r^{-i} f_i(r) \red{\chi}(r) \, dr= a_{ii}\ne 0
 \,,
$$
%
so that we can indeed choose $c_i = 1/a_{ii}$ to fulfill  \eqref{13VIII22.2}.

\ptc{the log discussion moved to kappsWithLogs, perhaps to reuse in higher dim} 

==> HDLemmaStratgey.tex <==
Our  gluing procedure for such fields rests on the following elementary result. Let
 \red{$a<b<c$}, and  let us for simplicity  assume that all fields
$\partial_u^i h_{\mu\nu}$, $i\in \N$, on $\mcN_{(a,b]}$  and $\mcN_{[b,c)}$  are smooth in all variables, up-to-and-including the common boundary  at  $b$. A similar result for finitely-differentiable fields, with distinct finite losses of differentiability for distinct fields, can be established using the results of Section~\ref{ss25IV22.1}, and is left as an exercise to a concerned reader.

\begin{Lemma}
 \label{L30IX22.1}
 Let $k\in \N$.
Two smooth data  sets in Bondi gauge on $\mcN_{(a,b]}$ and  $\mcN_{[b,c)}$, with   $h_{AB}$ extending  smoothly across  $\{r=b\}$ , extend to smooth $C^k$ data  on $\mcN_{(a,c)}$  if and only if, for   $0\le i\le k$ the fields
 \ptcr{wording requires some thought; some conditions here are not independent; maybe the number of derivatives can be improved in this scheme too, or some of the Einstein equations can be satisfied to lower order; and there are possibly losses in derivatives in this scheme in any case, so this is probably not quite right as stated}
%
\begin{enumerate}
  \item
   \label{p30IX22.1}
    $\partial_u^ih_{ur}$,  and
  \item
   $\partial_u^i\partial_r h_{uA}$, and
  \item  $\partial_u^ih_{uA}$, and
  \item  $\partial_u^i h_{AB}$, and
  \item
   \label{p30IX22.2} $\partial_u^i h_{uu}$
\end{enumerate}
extend by continuity  at $\{r=b\}$ to  continuous fields.
 \end{Lemma}

%
\proof
%
The necessity is obvious. The sufficiency
follows easily from the equations  in Sections \ref{sec:28VII22.1}-\ref{sec:25VII22.1}, together with their $u$-derivatives, as follows

Indeed, suppose that $\delta \beta$ extends by continuity at $b$, then \eqref{CHG28XI19.4aa} shows that $\delta \beta$ extends to a smooth function. Next, \eqref{24VII22.1} shows that continuity of
$ \partial_r(r^{-2} h_{uA}) $ at $b$ guarantees a smooth extension of $ \partial_r(r^{-2} h_{uA}) $. But then, by another integration, continuity of $   h_{uA}  $ at $b$ guarantees smooth extendability. One can now use  \eqref{27III2022.3b} and \eqref{eq:31III22.3p0} to similarly show that continuity at $b$ of $ \delta V$ and $\partial_u h_{AB}$ leads to  smooth extensions.
In particular $\partial_u h_{AB}$ is now smooth on $\mcN_{(a,c)}$, and one can apply the argument just given to the equations obtained by $u$-differentiating the vacuum Einstein equations to obtain smoothness on $\mcN_{(a,c)}$ of $\partial_u h_{\mu\nu}$ and $\partial^2_u h_{AB}$.

Iterating this reasoning a finite number of times establishes the result.
%
\qedskip
% 

==> HDPureChargeField.tex <==
\section{``Pure charge'' solutions}
 \label{s13VII22.1}


Consider the linearised metric perturbation:
 \ptcheck{14VIII22}
%
\begin{eqnarray}
 \mathring h
  &
 =
  &
  \bigg(
   \frac{\red{\red{\mathring \mu}}(u,x^B)}{r}
    - \frac{\zspaceD^A \red{\mathring \Ipsi}_A(u,x^B)}{2 r^2}
    +   \zspaceD^A \red{\mathring \Ichi}_A(u,x^B)   r
    \bigg)
      du^2
      \nonumber
\\
      &&
        +
  \bigg(
    \frac{\red{\mathring \Ipsi}_A(u,x^B)}{r}
     + r^2 \red{\mathring \Ichi} _A(u,x^B)
      \bigg)dx^A  du
  \,,
 \label{13VIII22.11}
\end{eqnarray}
%
with
%
\begin{align}\label{13VIII22.12a}
 TS\big[\zspaceD_A   \red{\mathring \Ichi}_{B}
     \big]
        = 0 =
TS\big[\zspaceD_A   \red{\mathring \Ipsi}_{B}
       \big]
       \,,
       &
       \quad
       (\Delta_{\ringh} +1)\red{\mathring \Ichi}_{B}= 0
       = (\Delta_{\ringh} +1)\red{\mathring \Ipsi}_{B}
%       \zspaceD^A   \red{\mathring \Ipsi}_{A} = 0
        \,,
\\
    3 \alpha^2 \zspaceD^A\red{\mathring \Ipsi}_A   +2 \partial_u \red{\mathring \mu}  =0
   %= \zspaceD^A\red{\mathring \mu}_A
   \,,
   &
       \quad
    3 \partial_u \red{\mathring \Ipsi}_A -  \zspaceD_A  \red{\red{\mathring \mu}}  = 0
  %  \,,
%    \quad
%   \zspaceD_A \partial_ u \red{\mathring \Ichi}^A + \alpha .... =0
   \,.
    \label{13VIII22.12b}
\end{align}
%
One checks that the tensor field $ \red{\mathring h}$
solves the linearised Einstein equations, cf.\ Sections~\ref{sec:28VII22.1} and \ref{sec:25VII22.1}.
It follows from  \eqref{13VIII22.12b} that
%
\begin{equation}\label{22VIII22.1}
   (\Delta_{\ringh} +1)
      \zspaceD_A  \red{\red{\mathring \mu}}
    =  3 (\Delta_{\ringh} +1)
     \partial_u \red{\mathring \Ipsi}_A   = 0
    \,,
     \qquad
     2 \partial_u ^2 \red{\mathring \mu} = - 3 \alpha^2 \Delta_{\ringh} \red{\mathring \mu}
     \,.
\end{equation}
%
In particular,
on $S^2$ the  ``mass aspect function''  $\red{\red{\mathring \mu}}$ is a linear combination of $\ell=0$ and $\ell=1$ spherical harmonics, so that
%
\begin{equation}\label{22VIII22.11}
       \partial_u ^2 \red{\mathring \mu} =
     \left\{
       \begin{array}{ll}
         3   \alpha^2 \red{\mathring \mu}, & \hbox{$\mathring \mu$ has no $\ell=0$ harmonics;} \\
          0, &  \hbox{$\mathring \mu$ has no $\ell=1$ harmonics.}
       \end{array}
     \right.
\end{equation}
%


On $S^2$ the second equation in \eqref{13VIII22.12a} follows from the first one, so that the space of $\mathring \Ipsi$'s satisfying \eqref{13VIII22.12a} is six-dimensional. For the remaining topologies of $\secN$ one finds $\mathring \Ichi_A\equiv \mathring \Ipsi _A\equiv 0$, and $\mathring \mu$ must be $u$ and $x^A$-independent.

Again on $S^2$, the tensor field $\red{\mathring h}$ carries the full set of conserved \red{radial charges} along $\mcN_{(r_0,r_3)}$
 \ptcr{to check, also in higher dim?}
 when $\red{\red{\mathring \mu}}$ and  $\red{\mathring \Ipsi}_A$
%and $\red{\mathring \mu}_A$
run over the set of solutions of \eqref{13VIII22.12a}-\eqref{13VIII22.12b}:
 %
 \begin{align}
     \kQ{1}{}(\pi) = -3 \int_{\secN}\pi^A \mathring \Ipsi_A \,\sm \,,
     \qquad
      \kQ{2}{}(\lambda) = -\int_{\secN}\lambda \mathring \mu \,\sm \,,
 \end{align}
 %
 where $\pi$ and $\lambda$ satisfy, respectively,
 \eqref{6III22.3} and \eqref{24VII22.6}.



It follows that any linearised vacuum data on $\mcN_{(r_0,r_1]}$ can be glued to any linearised vacuum data on $\mcN_{[r_2,r_3)}$ after adding to one of them a suitable field of the form \eqref{13VIII22.11}, possibly, but not necessarily, with $\mathring \Ichi_A=0$.
\ptcr{either the comment, or the whole appendix, should be moved elsewhere}


==> HDRemark.tex <==

{\blueca{13VII22; moved on 20VIII and perhaps move elsewhere}
We start by noting that the gluing of $h_{uA}$ is obtained by integrating a second-order equation, and hence requires matching two fields at $r=r_2$, e.g. $h_{uA}|_{r_2}$ and $\partial_r h_{uA}|_{r_2}$.
%The remaining constrained fields, namely $h_{uu}$ and $\partial_u h_{AB}$, are matched by integrating first order equations, whence only one matching equation for each of these fields will arise at $r_2$.
This suggests that two equations for each $u$-derivative might be  needed at $r_2$ when matching $u$-derivatives of  $h_{uA}$. This turns out not to be the case:  one equation suffices because of the Bianchi identities. Indeed, the analysis in Section~\ref{sec:25VII22.1} shows that if \eqref{9XI20.t1}, or its $u$-derivatives of any order, are  satisfied at $r=r_1$, as is implemented in our argument, then \eqref{9XI20.t1}, or its $u$-derivatives, will also be satisfied at $r=r_2$.
}


==> HDStrategyOld.tex <==
\input{StrategyHd}
%\section{Strategy}
 \label{ss10IX22.1}

To achieve linearised characteristic $\Ck$-gluing in the $\delta \beta = 0$ gauge, it is sufficient to find a continuous interpolation on $\mcN$ of the fields
%
\begin{align}
    \{
   \chi,\overadd{*}{\Hf}_{uA}, \overadd{0}{\Hf}_{uA}, \overadd{\ell}{\Hf}_{uA}, \overadd{\ell}{q}_{AB}
    \}_{\ell=1}^{k}
    \,.
    \label{4V23.1}
\end{align}
%
We will justify this shortly.

We consider first the case where the pair $(n,k)$ is convenient with \underline{$m=0=\alpha$}, because it contains most of the main ideas without
the technical complications which come with the remaining cases.
Then the transport equation for a field $\chi$,  $H$ or $q$
 appearing in \eqref{4V23.1} generally takes the form
%
  \begin{align}
      \partial_r \Hf = r^{q} \hat{D}(h_{AB})
      \,,
      \label{5V23.2}
  \end{align}
%
for some $q\in \Z/2$ and for a  linear differential operator $\hat{D}$ in the $x^A$-variables acting on $h_{AB}$;
we list the exponents $q$ and the operators $\hat{D}$ for the various fields in Table~\ref{T6V23.1}.\ptcheck{2VI23}%
%
\input{TableOfOperatorsNew}
%
 Integrating \eqref{5V23.2} from $r_1$ to $r_2$ gives
%
  \begin{align}
       \Hf|_{\secN_2} - \Hf|_{\secN_1} = \int_{r_1}^{r_2} s^{q} \hat{D}( h_{AB}(s)) \, ds\,;
      \label{5V23.2b}
  \end{align}
%
this integrated transport equation tells us how to choose $h_{AB}$ along $\mcN_{[r_1,r_2]}$ to achieve \textit{continuous} gluing of $\Hf[\dt_{\secN_1}]$ with $\Hf[\dt_{\secN_2}]$.

However, it follows from \eqref{5V23.2} that $\Hf{}^{[\ker \hat{D}^\dagger]}$ is a \textit{radially conserved charge}, since for any
%
  \begin{equation*}
      \mu \in \ker \hat{D}^\dagger \,,
  \end{equation*}
%
we have
%
\begin{align}
    \partial_r \int_{\secN_r} \mu \Hf \sm
     =
      r^{q} \int_{\secN_r} \mu \hat{D}( h_{AB}) \sm
      =
       r^{q} \int_{\secN_r}\big( \hat{D}^\dagger \mu \big){}^{AB}h_{AB} \sm
       = 0\,.
\end{align}
%
 This shows that no choice  of $h_{AB}$ along $\mcN_{[r_1,r_2]}$ can  achieve the  gluing of $\Hf{}^{[\ker \hat{D}^\dagger]}$. Moreover, a necessary condition  to achieve characteristic gluing-up-to-gauge is the existence of a gauge transformation so that
%
\begin{equation}
    \widetilde\Hf{}^{[\ker \hat{D}^\dagger]}|_{\tilde\secN_2} -  \widetilde\Hf{}^{[\ker \hat{D}^\dagger]}|_{\tilde\secN_1} = 0\,,
    \label{5V23.1}
\end{equation}
%
where $\widetilde{\Hf{}}$ denote the gauge-transformed counterpart of $\Hf{}$.
 \ptc{add to index if notation tilde H used elsewhere}

Let us denote  by $\myhatopL$ the linear differential operator occurring in the formula for the gauge-transformation of the charge associated with $\Hf$:
%
\begin{equation}
     \int_{\secN_2} \mu \Hf \sm \rightarrow \int_{\tilde\secN_2} \mu (\Hf
      + \myhatopL(\hat \xi) )\sm
     \,,
      \label{6V23.p1}
\end{equation}
%
where $\hat \xi$ stands for a gauge field from  the collection $\{\partial^i_u\kxi{2}^A, \kxi{2}^u\}_{i=0}^{k+1}$.

We will check that for all the  operators $ \myhatopL$ and $\hat D$ occurring  in Table~\ref{T6V23.1} we have (see Appendix~\ref{s25X23.1-})
%
\begin{equation}\label{6V23.1}
 \fbox{$(\ker \myhatopL^\dagger)^\perp = \im \myhatopL$, similarly $(\ker \hat{D}^\dagger)^\perp = \im \hat D$.
 }
\end{equation}
%
Then for all $\mu\in(\ker \hat{D}^\dagger)\cap(\ker \myhatopL^\dagger)$ it holds that
%
\begin{align}
    \int_{\secN_2} \mu \tilde\Hf \sm =\int_{\secN_2} \mu (\Hf
     + \myhatopL(\hat \xi) )\sm = \int_{\tilde\secN_2} \mu \Hf \sm\,.
\end{align}
%
In other words, the $L^2$-orthogonal projection  $\Hf{}^{[(\ker \hat{D}^\dagger)\cap(\ker \myhatopL^\dagger)]}$ of  $\Hf$
is gauge-invariant and the fields $\Hf|_{\secN_1}$ and $\Hf|_{\secN_2}$ cannot be continuously glued-up-to-gauge unless
%
\begin{equation}\label{15XII23.1}
\fbox{$\Hf{}^{[(\ker \hat{D}^\dagger)\cap(\ker \myhatopL^\dagger)]}|_{\secN_1}=\Hf{}^{[(\ker \hat{D}^\dagger)\cap(\ker \myhatopL^\dagger)]}|_{\secN_2} \,.
$
}
\end{equation}
%
We shall refer to such projections as \textit{gauge-invariant obstructions} to gluing.


Thus:
%
\begin{itemize}
    \item[(i)] The $L^2$-orthogonal projection  to
    %
    $$
     \ker (\hat{D}^\dagger)\cap\im (\myhatopL )
     =
     \ker (\hat{D}^\dagger)\cap\ker (\myhatopL^\dagger)^\perp
     $$
      %
      of the gauge-transformed version of the condition \eqref{5V23.1} can be achieved using the gauge field $\hat\xi ^{[(\ker \myhatopL)^\perp]}$ by solving the equation
%
    \begin{align}
        \myhatopL(\hat\xi^{[(\ker \myhatopL)^\perp]}) = \Hf{}^{[(\ker \hat{D}^\dagger)\cap(\ker \myhatopL^\dagger)^\perp]}|_{\secN_1} - \Hf{}^{[(\ker \hat{D}^\dagger)\cap(\ker \myhatopL^\dagger)^\perp]}|_{\secN_2} \,,
    \end{align}
%
    with a unique field $\hat\xi^{[(\ker \myhatopL)^\perp]}$ solving this equation.
    \item[(ii)] The projection onto $\im \hat D =(\ker \hat{D}^\dagger)^\perp$  of the gauge-transformed version of the condition \eqref{5V23.2b} results in the equation
    %
    \begin{align}
    \int_{r_1}^{r_s} r^q \hat D (\tilde h_{AB}(s)) ds = \widetilde \Hf{}^{[(\ker \hat{D}^\dagger)^\perp]}|_{\secN_2} - \widetilde \Hf{}^{[(\ker \hat{D}^\dagger)^\perp]}|_{\secN_1}  \,,
     \label{6V23.2}
    \end{align}
    %
    which can be solved for a unique field $\kphi{-q}^{[(\ker \hat{D})^\perp]}_{AB}$.
%
\end{itemize}
%
To summarise: we solve the integrated transport equation \eqref{5V23.2b} up to gauge by projecting it onto three parts. Then the part

\begin{enumerate}
  \item   $\ker \hat D^\dagger \cap \ker \myhatopL^\dagger$ gives a gauge-invariant obstruction;
  \item   $\ker \hat D^\dagger \cap (\ker \myhatopL^\dagger)^\perp$ is solved by the gauge field $\hat\xi^{[(\ker \myhatopL)^\perp]}$;  and
  \item $(\ker \hat D^\dagger)^\perp$ is solved by the interpolating field $\kphi{-q}^{[(\ker \hat{D})^\perp]}_{AB}$.
\end{enumerate}

To make this work one needs to isolate the operators involved, establish their mapping properties, and make sure that the powers $r^q$ arising in the integrals \eqref{6V23.2} are distinct for distinct fields $H$ from the collection \eqref{4V23.1}.
As an example, we provide an analysis of all operators involved in the case when $\secN \approx S^{n-1}$ in Appendix~\ref{ss20X22.1}.

The strategy of the case with non-vanishing $\alpha$ and/or $m$, and of the inconvenient case, is more involved due to the coupling between various equations, but comes with less obstructions to gluing. These cases will be treated in detail below, in Section \ref{ss30VI.1}.

We sketch now the linearised characteristic $\Ck$-gluing. This can be achieved in three steps:
%
\begin{enumerate}
  \item
  We solve the integrated transport equations for each field appearing in the set \eqref{4V23.1}. These will determine the gauge fields $\kxi{2}{}_A$ and $\kxi{2}^u$ and the interpolating fields $\kphi{p}_{AB}$, as well as the conditions on $\dt_1$ and $\dt_2$ associated with the gauge-invariant-obstructions.
  We list the  fields involved in Tables \ref{T11III23.2}-\ref{T11XII23.1}, and present more details  in the next section. All remaining free fields, such as $\partial_u^p\kxi{1}$, not appearing in these tables are   set to zero. The last columns (denoted as ``obstructions'') in these tables list the gauge-invariant radial charges associated to the indicated fields appearing in the respective rows.  See Table~\ref{T8VI23.1} for an explicit list of the spaces involved in the case $\secN \approx S^{n-1}$, $n\ge 4$, and $\alpha=0=m$.
  %
\input{TableOnSphere}
%

    \item Once the gauge fields and the fields $\kphi{p}_{AB}$ with $4-n \leq p \leq k_{\red{[m]}}+4$
    have been determined, we let $\tilde h_{AB}$ be as in \eqref{16III22.2old} and use this to construct the fields $\partial_u^p\tilde\hBo_{\mu\nu}$ on $\tmcN_{[r_1,r_2)}$ using the explicit formulae in Sections 
    \ref{sec:28VII22.1} and \ref{sec6III23.1}:
\seccheck{12XII23}

     \begin{enumerate}

     \item[i.] $\partial_u^p \tilde h_{ur}$ for $0\leq p\leq k$: We set $\partial_u^p \tilde h_{ur}|_\tmcN \equiv 0$, which guarantees both smoothness of $\tilde h_{ur}$ and the validity of  the equations, for all $i$,
%
    \begin{eqnarray}
    0
   &  = &
  \partial_u^i \delta \mcE _{rr}  |_\tmcN
  \equiv
  - \partial_u^i \delta \mcE ^u{}_{r}  |_\tmcN
  \equiv
  \partial_u^i \delta \mcE ^{uu}  |_\tmcN
   \,.
   \label{30IX22.11}
    \end{eqnarray}
%
         \item[ii.]
          $\partial_u^p\tilde\hBo_{uA}$ for $0\leq p \leq k$: We determine $\partial_u^p\tilde\hBo_{uA}|_{\mcN_{[r_1,r_2]}}$ by integrating \eqref{6III23.w1a}, with all $h_{\mu\nu}$'s there replaced by $\tilde h_{\mu\nu}$'s.
          Note that\eqref{6III23.w1a} can be solved in a recursive way together with the transport equations for $\overadd{p}{q}_{AB}$: one first obtains $\tilde h_{uA}|_{\mcN_{[r_1,r_2]}}$ by integrating the gauge-transformed version of \eqref{6III23.w1a} with $i=0$, cf.\ \eqref{21II23.2}:
          %
          \begin{align}
              \overadd{0}{\tilde\Hf}_{uA}(r) = \overadd{0}{\tilde\Hf}_{uA}|_{r_1} +
    \int_{r_1}^r \frac{1}{s^4}  \zspaceD^B \tilde h_{AB} \ ds
    \,.
          \end{align}
          %
          Next we solve similarly the integrated transport equation for $\overadd{p}{q}_{AB}$ (see item iv.\ below) starting with $p=1$, to obtain $\partial_u^p \tilde h_{AB}|_{\mcN_{[r_1,r_2]}}$, which is then used in the equation for $\overadd{p}{\tilde\Hf}_{uA}$, from which one obtains $\partial^{p}_u \tilde h_{uA}|_{\mcN_{[r_1,r_2]}}$. This will then be used for the transport equation of $\overadd{p+1}{q}_{AB}$ and so on. Satisfying the transport equation \eqref{6III23.w1a} for $i=p$
          guarantees that on $\tmcN_{[r_0,r_2)}$ we have
%
      \begin{equation}\label{15XI22.w1}
          \partial_u^p \delta  \mcE _{rA}|_{\tmcN_{[r_0,r_2)}}  \equiv -  \partial_u^p \delta \mcE ^u{} _{A}|_{\tmcN_{[r_0,r_2)}} = 0
         \,.
      \end{equation}
%
    It follows that
    %
    \begin{equation}
        \partial^p_u \delta\mcE^A{}_B|_{\blue{\tmcN_{[r_0,r_2)}}} =  g^{AC}\partial^p_u\delta \mcE_{CB}|_{\blue{\tmcN_{[r_0,r_2)}}}\,.
        \label{15XI22.w2}
    \end{equation}
    %
    The divergence identity
%
\begin{eqnarray}
  0 &\equiv & \nabla_\mu \delta \mcE ^{\mu}{}_A
    \nonumber
\\
 &= &
 r^{-(n-1)}\partial_r(r^{n-1}  \delta \mcE ^r{}_A)
   + \partial_u \delta \mcE ^u{}_A
    + \zspaceD_B \delta \mcE ^B{}_A
 \,,
 \label{2X22.6}
\end{eqnarray}
%
together with its $u$-derivatives, shows that we also have
%
\begin{equation}
 \forall \
  0 \le i \le k-1  \quad
   \Big(
  r^{-(n-1)}\partial_r(r^{n-1}  \partial_u^i\delta \mcE ^r{}_A)
    + \zspaceD_B \partial_u^i\delta \mcE ^B{}_A
    \Big)\Big|_{\tmcN_{[r_0,r_2)}}
     =0
 \,.
  \label{1X22.3}
\end{equation}
%
%
         \item[iii.]
         $\partial_u^p \tilde \hBo_{uu}$ for $0\leq p \leq k$: We impose \eqref{1XI22.w1} together with its higher derivatives along $\tmcN_{[r_1,r_2)}$ (note that $r=r_2$ is omitted), i.e.,
         %
         \begin{equation}
             \partial_r \partial_u^p\tilde\chi = \frac{(n-3)r^{n-5}}{n-1}\zspaceD^A\zspaceD^B \partial_u^p \tilde h_{AB} \,,
         \end{equation}
         %
         with the initial conditions (compare \eqref{1III23.1})
         %
    \begin{align}
    \label{1III23.1c}
    \partial_u^p\tilde\chi|_{r_1} &=
    \partial_u^p \chi|_{r_1}
    - \frac{2r_1^{n-3}(n-2)}{(n-1)^2} \TSzlap ( \TSzlap + (n-1) \twoscsign) \partial_u^p\kxi{1}^u\
    \,,
    \end{align}
    %
         and using the value of $\partial_u^{p}\tilde\hBo_{AB}|_{\tmcN_{[r_1,r_2)}}$ (when $p>0$) determined in iv.\ below. The resulting field $\partial_u^p\tilde\chi|_{\tmcN_{[r_1,r_2)}}$, together with $\partial_u^{p}\tilde\hBo_{uA}|_{\tmcN_{[r_1,r_2)}}$ determined in  point ii., is used to find $\partial_u^p \tilde \hBo_{uu}$ along $\tmcN_{[r_1,r_2)}$. This ensures
          %
      \begin{equation}\label{15XI22.w3}
           \partial^p_u\delta\mcE _{ru}|_{\blue{\tmcN_{[r_0,r_2)}}}
           - \frac 1{(n-2)r}
  \zspaceD ^A  \partial^p_u\delta \mcE _{rA}|_{\blue{\tmcN_{[r_0,r_2)}}}  = 0\,.
      \end{equation}
      %
      Together with \eqref{15XI22.w1}, Equation~\eqref{15XI22.w3} guarantees that
      %
      \begin{equation}\label{1X22.2}
    \partial_u^p \delta  {\mcE}_{ru}|_{\tmcN_{[r_0,r_2)}}
     \equiv
    -
    \partial_u^p \delta  \mcE^u{}_{ u}|_{\tmcN_{[r_0,r_2)}}
      = 0\,.
      \end{equation}
      %
%
         \item[iv.] $\partial_u^p\tilde\hBo_{AB}$ for $1\leq p \leq k$:
         We use the representation formulae obtained by integrating \eqref{6III23.w6} in $r$, with all $h_{\mu\nu}$'s replaced by $\tilde h_{\mu\nu}$'s, and making use of $\partial_u^{p-1} \tilde h_{uA}|_{[r_0,r_2)}$ obtained in point ii., to determine $\partial_u^{p} \tilde h_{AB}|_{[r_0,r_2)}$. This ensures that
    %
    \begin{equation}\label{15XI22.w4}
  \TS\big(
   \delta \partial^{p-1}_u \mcE _{AB}
    \big)
  \big|_{\tmcN_{[r_0,r_2)}}
   =0
    \,.
    \end{equation}
    %
    The $u$-differentiated divergence identity reads
    %
    \begin{align}
     0 &\equiv \nabla_\mu \partial_u^p \delta \mcE ^{\mu}{}_r
     \nonumber
     \\
     &=
     \partial^p_u  \delta  \mcE ^u{}_r
   +
   \frac{1}{r^{n-1}} \partial_r  (r^{n-1}  \delta  \partial^{p-1}_u\mcE ^r{}_r )
   \nonumber
    \\
    &\qquad
   +   \frac{1}{\sqrt{|\det \zgamma |}} \partial_A (\sqrt{|\det \zgamma |} \delta  \partial^{p-1}_u\mcE ^A{}_r )
   -
   \frac{1}{r}
        g^{AB}
    \delta \partial^{p-1}_u\mcE _{AB}
   \,,
   \label{C21X22.5ii}
    \end{align}
    %
    so that, in view of \eqref{30IX22.11}, \eqref{15XI22.w1} and \eqref{1X22.2}, we have now
    %
    \begin{equation}\label{1X22.6}
    \forall \
     0 \le i \le k \qquad
      0 =
      \frac{1}{r}
        g^{AB}
      \partial_u^i  \delta \mcE _{AB}
        \big|_{\tmcN_{[r_0,r_2)}}
   \,.
    \end{equation}
    %
    Together with \eqref{15XI22.w4}, it follows that
    %
    \begin{equation}\label{2X22.4}
 \forall \
  0 \le i \le k-1 \qquad
   \partial_u^i \delta \mcE _{AB}
  \big|_{\tmcN_{[r_0,r_2)}}
   =0
    \,.
    \end{equation}
    %
    Equation \eqref{1X22.3} then gives
    %
    \begin{align}
     \forall \
      0 \le i \le k-1 \qquad
        0 & =r^{-(n-1)}\partial_r(r^{n-1}
       \partial_u^i \delta \mcE ^r{}_A) |_{\tmcN_{[r_0,r_2)}}
       \nonumber
       \\
        &=
         - r^{-(n-1)}\partial_r(r^{n-1}
       \partial_u^i
       \delta \mcE _{uA}) |_{\tmcN_{[r_0,r_2)}}
       \,,
        \label{15XI22.w5}
    \end{align}
    %
    where we have used
    %
    $$ \partial_u^i\delta \mcE^{r}{}_A |_{\tmcN_{[r_0,r_2)}}
     = - g_{uu}  \partial_u^i\delta \mcE_{r A}|_{\tmcN_{[r_0,r_2)}} -  \partial_u^i\delta \mcE _{u A}|_{\tmcN_{[r_0,r_2)}}
      =   -  \partial_u^i\delta \mcE _{u A}|_{\tmcN_{[r_0,r_2)}}
      \,;
    $$
    %
    note that the last equality is justified by \eqref{15XI22.w1}. Continuity at $r_1$, where all the fields $
   \partial_u^i  \mcE _{\mu\nu} $, $i\in \N$, vanish when the data there arise from a smooth solution of linearised Einstein equations, together with \eqref{15XI22.w5} implies that
    %
    \begin{equation}
     \forall \
      0 \le i \le k-1 \qquad
       \partial_u^i  \delta \mcE ^r{}_A  |_{\tmcN_{[r_0,r_2)}}=0 = \partial_u^i  \delta \mcE _{uA} |_{\tmcN_{[r_0,r_2)}}
        \,.
         \label{2X22.8}
    \end{equation}
    %

    Meanwhile, the divergence identity for the Einstein tensor with a lower index $u$ now reduces to
    %
    \begin{equation}
     \forall \
      0 \le i \le k-1 \qquad
      0  \equiv  \partial_u^i \nabla_\mu  \delta \mcE ^{\mu}{}_u
        \big |_{\tmcN_{[r_0,r_2)}}
       = r^{-(n-1)} \partial_r (r^{n-1} \partial_u^i \delta \mcE^r {} _u)
        \big |_{\tmcN_{[r_0,r_2)}}
       \,.
    \end{equation}
    %
    Continuity and vanishing at $r_1$
     together with \eqref{30IX22.11}
     and  \eqref{1X22.2}
     implies that
    %
    \begin{equation}\label{2X22.7}
     \forall \
      0 \le i \le k-1 \qquad
       0 = \partial_u^i  \delta \mcE _{uu}
        \big |_{\tmcN_{[r_0,r_2)}}
         =  -  \partial_u^i  \delta \mcE ^r{}_{u}
        \big |_{\tmcN_{[r_0,r_2)}}
         =   \partial_u^i  \delta \mcE ^{rr}
        \big |_{\tmcN_{[r_0,r_2)}}\,.
    \end{equation}
    %
         \end{enumerate}
%
     \item
     The construction above guarantees
     the continuous gluing at $r_2$ of $\tilde\hBo_{uu}$, $\partial_u\tilde\hBo_{AB}$, $\overadd{p}{\tilde\Hf}_{uA}$ with $0\leq p \leq k$, and $\overadd{i}{\tilde q}_{AB}$ with $2\leq i \leq k$. Continuity of the fields $\partial^p_u \tilde\hBo_{uA}$
     %, $\partial_r\partial^p_u \tilde\hBo_{uA}$
     and $\partial_u^p\tilde\hBo_{uu}$ for $1 \leq p \leq k$  and
     $\partial^{i}_u \tilde\hBo_{AB}$ for $2 \leq i \leq k$
     at $r_2$ follows now
          by induction: The integrated transport equation for $\overadd{1}{\widetilde\Hf}_{uA}$ and the explicit form \eqref{9XI20.t1} of the equation $ \delta \mcE _{uA} =0$ can be solved simultaneously for $\partial_u \tilde h_{uA}|_{[r_1,r_2)}$ and $\partial_r \partial_u \tilde h_{uA}|_{[r_1,r_2)}$. The solutions will be given in terms of the previously obtained fields $\{\tilde\hBo_{uu}, \tilde\hBo_{uA}, \tilde\hBo_{AB}, \partial_u\tilde\hBo_{AB}\} $, which are continuous at $r_2$, hence ensuring continuity of $\partial_u \tilde h_{uA}$ and $\partial_r \partial_u \tilde h_{uA}$ at $r_2$. This in turn guarantees the continuity of $\partial_u^2 \tilde h_{AB}$ at $r_2$.

    Meanwhile the explicit form \eqref{13VIII20.t3} of $ \delta \mcE_{u u}=0$ together with continuity  at $r_2$ of $\tilde\hBo_{uu}$, $\tilde\hBo_{uA}$  and $\partial_u\tilde\hBo_{AB}$, ensures the continuity of $\partial_u\tilde\hBo_{uu}$ at $r_2$.

     Now, suppose that the continuity of the fields $\partial_u^p\tilde\hBo_{uu}$, $\partial_r\partial_u^p\tilde\hBo_{uA}$ and $\partial_u^{p+1}\tilde\hBo_{AB}$ has been achieved up to $p=k-1$. It follows that we have $\partial^{k-2}_u\delta \mcE _{uA}|_{\tmcN} =0$ and thus $\partial_r \kQ{1,k-1}{}(\pi^A)|_{\tmcN}=0$ (compare \eqref{6X22.w1}).

     Next, by differentiation of \eqref{20II23.3aw} we obtain the explicit form of \eqref{2X22.8} with $i=k-1$:
    %
    \begin{align}
      - r^{n+1}\partial_{r}\partial^k_{u}\left(\frac{h_{uA}}{r^{2}}\right)
& =
r^{n-3}\zspaceD^{B}\zspaceD_{A}\partial^{k-1}_{u}{h}_{uB}
- r^{n-3}\zspaceD^{B}\zspaceD_{B}\partial^{k-1}_{u}{h}_{uA}
+  r^{n-3}\partial^k_{u} \zspaceD^{B}{h}_{A B}
\nonumber
\\
&\quad
- 2 (n-2) r^{n-1}(\alpha^2 + {2m r^{-n}}) \partial^{k-1}_{u}h_{uA}
- r^{2}\partial_{r}(r^{n-3}\zspaceD_{A}\partial^{k-1}_{u}{h}_{uu})
\nonumber\\
&\quad
-r^{(n-2)}(\twoscsign - r^2(\alpha^2+ {2mr^{-n}}) )((n-3)\partial_r \partial^{k-1}_{u} h_{uA} + r\partial^2_r \partial^{k-1}_{u} h_{uA})
\,.
    \label{9XI20.t1c}
    \end{align}
    %
    Equation \eqref{9XI20.t1c} and the integrated transport equation \eqref{6III23.w1a} with $i=k$, together with the continuity of
    $\partial^{k-1}_u\tilde\hBo_{uu}$,
     $\partial_u^{k-1}\tilde \hBo_{uA}$ and $\partial^k_u\tilde\hBo_{AB}$,
       ensures the continuity of $\partial_u^{k} \tilde\hBo_{uA}$ and $\partial_r\partial_u^{k} \tilde\hBo_{uA}$ at $r_2$. This in turn guarantees the continuity of $\partial_u^{k+1} \tilde\hBo_{AB}$ at $r_2$.

       Finally, the explicit form of \eqref{2X22.7} with $i=k-1$,
    i.e.
        %
    \begin{eqnarray}
      0 & = &  \partial_u^{k-1}  \delta \mcE _{uu}
        \big |_{\mcN_{[r_1,r_2)}}
      \nonumber
    \\
     & = &     \frac{1}{ r^2}\bigg[
       2\partial^k_{u} \zspaceD^{A} {h}_{u A}
        + \partial_r \left(\frac{V}{r}\right)  \zspaceD^{A} \partial_u^{k-1}{h}_{u A}
        - \frac{V}{r^{n-1}}  \partial_{r} \bigg(r^{n-2} \zspaceD^{A}\partial_u^{k-1} {h}_{u A}\bigg)
 \nonumber
\\
 &&
 +\frac{V}{r^3} \bigg(\zspaceD^{A} \zspaceD^{B} -\zR^{AB} \bigg)\partial_u^{k-1} h_{A B}
 -\left(r (n-1) (\partial_{u}
 -\partial_r\left(\frac{V}{r}\right)) +  R[\gamma] + \zspaceD^{A} \zspaceD_{A}\right)\partial_u^{k-1}{h}_{u u}
 \nonumber
\\
& &
   + \frac{(n-1)V}{r^{2n-4}} \partial_{r}(r^{2n-4} \partial_u^{k-1} {h}_{u u})\bigg]
    + 2 \Lambda \partial_u^{k-1} h_{uu}
    \, , \phantom{xxxxx}
    \label{13VIII20.t3rs}
    \end{eqnarray}
    %
    together with smoothness  at $r_2$ of $\partial_u^{k-1}\tilde\hBo_{uu}$, $\partial_u^{k-1}\tilde\hBo_{uA}$, $\partial_u^{k}\tilde\hBo_{uA}$  and $\partial^{k-1}_u\tilde\hBo_{AB}$, ensures the continuity of $\partial^k_u\tilde\hBo_{uu}$ at $r_2$.

 \end{enumerate} 

==> HDSummaryTable.tex <==
%
\begin{table}[t]
\hspace{-1.5cm}
 \begin{tabular}{|c||c|c|c|c||}
  \hline
  \hline
    & Gluing field & Gauge field & Obstruction\\
  \hline
    $h_{AB} $
        & $\interph_{AB} $
                & -
                     & -
  \\
  \hline
    $\partial^i_u\tilde\hBo_{ur}\,,\  i\ge 0$
        & -
                &  $\partial_u^{i+1}\kxi{1}^{u }$
                and $\partial_u^{i+1}\kxi{2}^{u }$
                     & -
  \\
  \hline
    $\tilde\hBo_{uu}$
        &  $\kphi{5-n}_{AB}$ \checkmark
                &  -
                     &     $\kQ{2}{}[\dt_{\secN_1}]=\kQ{2}{}[\dt_{\secN_2}]$
  \\
  \hline
    $\partial_r \tilde\hBo_{uA}$
        &   $\kphi{4-n}_{AB}^{[\TTtp]}$
            & -
                &  $\kQ{1}{}[\dt_{\secN_1}](\pi^A)=\kQ{1}{}[\dt_{\secN_2}](\pi^A)$
 \\
         &
             &
                & $\pi^A\in\CKV$
\\
  \hline
    $\tilde\hBo_{uA}$
        &  $\kphi{4}_{AB}^{[\TTtp]}$
             & $\partial_u\kxi{2}{}_A^{[\CKV]}$
                 & -
\\
  \hline
    $\partial_u\tilde\hBo_{AB}$, $\alpha=0$
        & $\kphit{AB}{(9-n)/2}$
         (typeset as ? $\kphi{(9-n)/2}_{AB}$ )
            &   -
                &  $\ker(\overadd{1}{\psi}(P))$
\\
    \phantom{$\partial_u\tilde\hBo_{AB}$, }$\alpha\neq 0$
        & $\kphit{AB}{(5-n)/2}$ ($n>5$)
            &   -
                &  -
\\
\hline
    $\partial_u^p\tilde\hBo_{AB}$, $2\leq p \leq k$
        &
            &   %
                &    %
\\
    $n$ even, $\alpha = 0$
        & $\kphit{AB}{(7-n+2p)/2}$
            &  -
                & $\ker(\overadd{p}{\psi}(P))$
\\
    $n$ even, $\alpha \neq 0$
        & $\kphit{AB}{(7-n-2p)/2}$
            &  -
                & -
\\
    $n$ odd
        &  tbc
            &  tbc
                &  tbc
\\
  \hline
    $\partial_u^p\tilde\hBo_{uA}$,  $1\leq p \leq k$
        &
            & %
                & %
\\
    $n$ even
        &  $\kphi{p+4}^{[\TTtp]}_{AB}$
            & %$\partial_u^{p+1} \kxi{2}_A^{[1\leq \ell\leq p+1]}$ 
            $\partial_u^{p+1} \kxi{2}_A^{[\ker(\overadd{p}{\chi}(P) \circ C)]}$
                & -
\\
    $n$ odd, $1 \leq p < \frac{n-3}{2}$
         & 
            & 
                &  
\\
    $n$ odd,  $\frac{n-3}{2} \leq p \leq k$
         & tbc
            & tbc
                &  tbc
\\
  \hline
    $\partial_u^p\tilde\hBo_{uu}$,  $1\leq p \leq k$
        & -
            & -
                & -
\\
  \hline
    $\partial_u^p\partial_r\tilde\hBo_{uA}$,  $1\leq p \leq k$
        & -
            & -
                & -
  \\
  \hline
  \hline
\end{tabular}
\caption{Fields used to ensure the continuity at $r_2$ when $m=0$.
  The continuity for the fields in the last two lines follows from Bianchi identities.
 The fields $\tilde\hBo_{\mu\nu}$ are the gauge-transformed fields
  $ \hBo_{\mu\nu}$
 using the gauge fields $\protect\kxi{1}$
 for $r\le r_1$ and $\protect\kxi{2}{}$ for $r\ge r_2$, cf.\ Section~\ref{ss11III23.1};
  the fields $\interph_{AB}$ and $\protect\kphi{p}_{AB}$
  are defined  in \eqref{16III22.2old} and \eqref{27VII22.1a}-\eqref{27VII22.1a+};  projections such as
  $(\cdot)^{[\TTt]}$ or $(\cdot)^{[\CKVp]}$
  are defined in Section~\ref{s26XI22.1};
  the radial charges  $\protect\kQ{a}{}$, $a=1,2$, are defined in \eqref{24VII22.4} and \eqref{20VII22.1};  the operator $P$ has been defined in \eqref{16V22.1b}; the operators $\protect\overset{(p)}{\ochi}(P)$ are defined in \eqref{6III23.w2}.
}\label{T11III23.1}
\end{table} 

==> HDTraceEqn.tex <==
\section{Trace equations}
\label{ss3X22.1}

{\blueac{15X22; can one use some of these equations to get rid of some obstructions?}
The aim of this appendix is to prove the curious identity
\ptcheck{12XI22, by Wan}
%
\begin{align}
    r^{-1} \gamma^{AB} \delta G_{AB} =  - \frac 12  \gamma^{AB}  \partial_r
          \delta R_{AB}
        +
        \zspaceD^A   \delta G_{rA}
     \,,
     \label{5X22.w4}
\end{align}
%
\red{when $\partial_u^i\delta\beta=0$ (i.e., $\partial_u^i\delta G_{rr} = 0$) for $i=0,1$.}}

For this, we start by noting that the operator $g^{AB}R_{AB}$ is related to that appearing in  \eqref{3X22.1}, which can be seen as follows:  From the definition \eqref{2X22.2} of the Einstein tensor $G_{\mu\nu}$ and the Bondi parametrisation of the metric \eqref{23VII22.1} we have
%
\begin{align}
\label{5X22.w1}
    G_{ur} = \frac{1}{2}e^{2\beta}g^{rr}G_{rr} - U^A G_{rA} + \frac{1}{2}e^{2\beta} g^{AB} R_{AB}\,.
\end{align}
%
% In particular when the equation $G_{rr} = 8\pi T_{rr}$ holds, we have
% %
% \begin{align}
%    2 e^{-2\beta} r^2( G_{ur}+ U^A G_{rA}) = r^2 g^{AB} R_{AB} + 8\pi r V e^{-2\beta} T_{rr}\,.
% \end{align}
% %
 Explicitly, the operator $g^{AB}R_{AB}$ reads,
%
\begin{align}
   g^{AB}R_{AB}&= e^{-2\beta}\left(\frac{4 D_{A}U^{A}}{r} + D_{A}\partial_rU^{A}-  \frac{\gamma_{AB} r^2\partial_rU^{A}\partial_rU^{B}}{2 e^{2 \beta}} -  \frac{2\partial_rV}{r^2}\right)
   \nonumber
\\
    & \qquad
     -  \frac{2 \gamma^{AB} D_{B}D_{A}\beta}{r^2} -  \frac{2 \gamma^{AB} \partial_{A}\beta \partial_{B}\beta}{r^2}
    +\frac{1}{r^2} R[\gamma]\,.
    \label{8X22.w1}
\end{align}
%
Next, the equation $e^{2\beta}g^{AB}G_{AB}=0$ can be written as
%
\begin{align}
    0&=
      -  \frac{2 D_{A}U^{A}}{r} -  D_{A}\partial_rU^{A} + \frac{2 e^{2 \beta} \gamma^{AB} D_{B}D_{A}\beta}{r^2} \nonumber
\\
    &\qquad
    - 4 U^{A} \partial_{A}\partial_r\beta + \frac{4 e^{2 \beta} \gamma^{AB} \partial_{A}\beta \partial_{B}\beta}{r^2} -  \frac{2 V\partial_r\beta}{r^2} -  \gamma^{BC} D_{B}U^{A}\partial_r\gamma_{AC} + \frac{\gamma^{AB} \gamma^{CD} V\partial_r\gamma_{AC}\partial_r\gamma_{BD}}{4 r} \nonumber
\\
    &\qquad
    - 2 \partial_{A}\beta\partial_rU^{A} -  \frac{\gamma_{AB} r^2\partial_rU^{A}\partial_rU^{B}}{e^{2 \beta}} + \frac{2\partial_r\beta\partial_rV}{r} + \frac{2 V\partial_r\partial_r\beta}{r} + \frac{\partial_r\partial_rV}{r} \nonumber
\\
    &\qquad
    - 4\partial_r\partial_{\partial_{u}{}}\beta -  \tfrac{1}{2} \gamma^{AB} \gamma^{CD}\partial_r\gamma_{AC} \partial_{\partial_{u}{}}\gamma_{BD}
     \,.
\end{align}
% 

==> HDduhab.tex <==
\subsubsection{Continuity of $\partial_u\tilde\hBo_{AB}$}
 \label{ss1VIII22.102}
 \wcb{this section may be obsolete: consider merging into the $\partial_u^p h_{AB}$ section?}
Taking into account the allowed gauge perturbations to Bondi data, it follows from \eqref{3IX22.1HD} and \eqref{7III23.w1} that the gluing of $\partial_u h_{AB}$ requires
%
\begin{align}
    & q_{AB}|_{\secN_2} - \tilde q_{AB}|_{\tilde{\secN}_1}
    \nonumber
    \\
    &\quad
    - r_2^{(n-3)/2}
    \left(
    \frac{2}{n-1} \TS[\zspaceD_A\zspaceD_B\zspaceD_C\kxi{2}^C] - \left( \frac{4}{n+1} P -\frac{n-1}{2} (\twoscsign - r_2^2 (\alpha^2+\ {2mr_2^{-n}}) \right)  C(\kxi{2})_{AB}
    \right)
     \nonumber
\\
    & \quad
     + \frac{r_2^{(n-5)/2}}{2} \left( (n-3)\twoscsign - (n+1) r_2^2 \alpha^2 \ {-\frac{(n-1)^2}{{n+1}} 2mr_2^{-n+2}} - \frac{4(n-3)}{(n-2)(n+1)}P\right) \TS[\zspaceD_A \zspaceD_B \kxi{2}^u]
    \nonumber
    \\
    &\quad
    =
    - \frac{(n -1)^2 }{4} m \int_{r_1}^{r_2} \hkappa_{(n+5)/2}(s) \tilde h_{AB} \, ds
    % \nonumber
    % \\
    % & \quad \phantom{ \quad
    % - r_2^{(n-3)/2} \hLop(\kxi{2})_{AB}
    % =}
    + \frac{1}{8}\left(n^2-1\right)\alpha ^2 \int_{r_1}^{r_2}
   \hkappa_{(5-n)/2}(s) \tilde h_{AB} ds
   \nonumber
   \\
   & \quad \quad
    + \int_{r_1}^{r_2} \overadd{1}{\psi}\ofP \, \hkappa_{(9-n)/2}(s) \tilde h_{AB} ds \,.
    \label{7III23.w2}
\end{align}
%
We solve the projection of \eqref{7III23.w2} onto $(\ker \overadd{1}{\psi}\ofP )^\perp$ using the field $\kphi{(9-n)/2}^{[(\ker \overadd{1}{\psi}\ofP )^\perp]}_{AB}$;
the projection of \eqref{7III23.w2} onto $\ker \overadd{1}{\psi}\ofP $ meanwhile calls for different strategies depending on the values of $m$, $\alpha$ and $n$: When $m=0=\alpha$, the projection of \eqref{7III23.w2} onto $\ker \overadd{1}{\psi}\ofP $ gives an gauge-invariant obstruction, see \eqref{19VIII23.1}.

\paragraph{The case $(n,k)$ convenient.} When $m=0$,  $\alpha \neq 0$, the projection of \eqref{7III23.w2} onto $\ker \overadd{1}{\psi}\ofP $ can be solved using the interpolating field $\kphi{(5-n)/2}_{AB}^{[\ker \overadd{1}{\psi}\ofP ]}$.

When $m\neq 0$, the projection of \eqref{7III23.w2} onto $(\ker \overadd{1}{\psi}\ofP )^\perp$ can be solved using the interpolating field $\kphi{(n+5)/2}^{[(\ker \overadd{1}{\psi}\ofP )^\perp]}_{AB}$; the field $\kphi{(5-n)/2}_{AB}$ is then free.

\paragraph{The case $(n,k)$ inconvenient.}
\FG{6VII23: Addition of $n=5$ case.
\\--\\
wan: ok for me}
%
\tcp{First, consider $n=5$: when $m=0$, $\alpha\neq 0$, we have $\kphi{(5-n)/2}_{AB}^{[\ker \overadd{1}{\psi}\ofP ]}=\kphi{0}_{AB}^{[\ker \overadd{1}{\psi}\ofP ]}$. Recall that, in this case, the field $\kphi{0}_{AB}^{[(\ker \mathring L)^\perp]}$ was determined in \eqref{7III23.1} for the gluing of $\chi$. Thus, we solve the projection of \eqref{7III23.w2} onto $\ker \overadd{1}{\psi}\ofP \, \cap \ker \mathring L$ using the free field $\kphi{0}{}{}{}^{[\ker \overadd{1}{\psi}\ofP \, \cap \ker \mathring L]}_{AB}$ which leaves the gauge-invariant obstruction
%
\begin{align}
\label{16VIII23.1}
    q_{AB}^{[\ker \overadd{1}{\psi}\ofP \, \cap (\ker \mathring L)^\perp]}|_{\secN_2}
    = q_{AB}^{[\ker \overadd{1}{\psi}\ofP \, \cap (\ker \mathring L)^\perp]}|_{\secN_1}\,.
\end{align}}
%

When $n\neq 5$ and $m=0$, $\alpha\neq 0$, the field $\kphi{(5-n)/2}_{AB}$ is free up to this point.  Thus, the projection of \eqref{7III23.w2} onto $\ker \overadd{1}{\psi}\ofP $ determines field $\kphi{(5-n)/2}_{AB}^{[\ker \overadd{1}{\psi}\ofP ]}$.

\wcb{this case is not settled yet, the problem being the overlap of power with $\kphi{4+p}_{AB}$ in $\overadd{p}{\Hf}_{uA}$ when $p=\frac{n-3}{2}$}
When $m\neq 0$, the projection of \eqref{7III23.w2} onto $(\ker \overadd{1}{\psi}\ofP )^\perp$ can be solved using the interpolating field $\kphi{(n+5)/2}^{[(\ker \overadd{1}{\psi}\ofP )^\perp]}_{AB}$ (the field $\kphi{(5-n)/2}_{AB}$ is then either free, or determined from \eqref{7III23.1}).


==> HDhigherderivatives18VIII.tex <==
\input{HDduhab}

\subsection{Higher derivatives}
\label{ss26XI22.3}

{\wblueca{20VI}
Gluing of the higher derivatives now proceed hierarchically in this order: 
$$\overadd{1}{\Hf}_{uA} \rightarrow \overadd{2}{q}_{AB} \rightarrow \overadd{2}{\Hf}_{uA} \rightarrow \ldots \rightarrow \overadd{k}{q}_{AB} \rightarrow \overadd{k}{\Hf}_{uA} \,.$$
}
\subsubsection{Continuity of $\partial_u^p \tilde h_{uA}$}

Taking into account the allowed gauge perturbations to Bondi data, it follows from \eqref{6III23.w1a} and \eqref{26V23.1} that the gluing of $\partial_u^p \tilde h_{uA}$, $1 \leq p \leq k$ requires 
\ptcr{To do: check smoothness of the orthogonal of the image to $\zspaceD^B \overadd{p}{\chi}(P)$ for differentiability tracing}
 %
 \begin{align}
      \overadd{p}{\Hf}_{uA}\big|_{\secN_2} - \overadd{p}{\tilde\Hf}_{uA}\big|_{\tilde\secN_1} 
       &= 
       \zspaceD^B \overadd{p}{\chi}(P) \int_{r_1}^{r_2} \hkappa_{p+4}(s) \tilde h_{AB} \ ds
    +  m^p  \overadd{p}{\chi}_m \int_{r_1}^{r_2} \hkappa_{p(n-1)+4}(s) \zspaceD^B \tilde h_{AB} \ ds
     \nonumber
\\
    & \quad
    + \sum_{j,\ell}^{p_*}  m^{j} \alpha^{2\ell} \zspaceD^B \overadd{p}{\chi}_{j,\ell}(P) \int_{r_1}^{r_2} \hkappa_{(p + 4) + j (n - 2) - 2 \ell}(s) \tilde h_{AB} \ ds
\\
    &\quad
     - n \partial_u^{p+1} \kxi{2}_A
    + \text{ gauge fields of lower $u$-derivatives} \,.
    \label{11III23.1}
 \end{align}
 %
\underline{When $m=0$}, the projection of this equation onto $(\ker[ \overadd{p}{\chi}(P) \circ C])^\perp$ can be solved uniquely for the field $\kphi{p+4}_{AB}^{[(\ker[ \zspaceD^A\overadd{p}{\chi}(P))^\perp]}$ in terms of the given data and predetermined gauge fields. We leave out the explicit formula of the gauge fields here; these can be determined order-by-order in the index $p$ using the recursion formula \eqref{6III23.w4} and the gauge transformations \eqref{17III22.1HD}-\eqref{17III22HD}.

\underline{when $m\neq 0$}, the projection of \eqref{11III23.1} onto $\CKVp$ can be solved uniquely for the field $\kphi{p(n-1)+4}_{AB}^{[\TTt^\perp]}$ in terms of the given data and predetermined gauge fields. The other interpolating fields $\kphi{i}_{AB}$ appearing in the sum $\sum_{j,\ell}^{p_*}$ are either predetermined, or free at this point, in which case we set them to zero.

We note that
%
\begin{equation}
    \TTt \subseteq \ker[ \zspaceD^A\overadd{p}{\chi}(P)] \,,
    \label{15VI.6}
\end{equation}
%
which implies that the fields $\kphi{p+4}_{AB}^{[\TTt]}$, $1 \leq p $, remain free at this point.

 \subsubsection{Continuity of $\partial_u^p \tilde h_{AB}$}

 \paragraph{The case $(n,p)$ convenient.} It follows from the transport equation \eqref{6III23.w6}  that the gluing of $\partial_u^p \tilde h_{AB}$ with $p\geq 2$ requires
 %
\begin{align}
    \overadd{p}{q}_{AB} \big|_{\secN_2} -\overadd{p}{\tilde q}_{AB} \big|_{\tilde\secN_1} 
    &=   \int_{r_1}^{r_2} [ \ \overadd{p}{\psi}(P) \hkappa_{(7-n+2p)/2}(s) \tilde h_{AB}
    + \alpha^{2p} \overadd{p}{\psi}_{\alpha} \hkappa_{(7-n-2p)/2}(s) \tilde h_{AB} 
    \nonumber
    \\
    &\phantom{ \int_{r_1}^{r_2} [ \ \quad }
    + m^p \overadd{p}{\psi}_m \hkappa_{(7-n+2p(n-1))/2}(s) \tilde h_{AB} 
    \ ] \ ds
    \nonumber
    \\
    &\quad
    + m (\ldots)
    +\text{ gauge fields}\, .
    \label{11III23.2}
\end{align}
%

First, we note that for $n>3$, $\frac{n-7-2p}{2} \neq -(k+4), n-5$ for any $p\geq 2$, $k \in \mathbb{Z}$ so the fields $\kphit{AB}{(7-n+2p)/2}$ are free at this point. Hence in the case when $m=0=\alpha$, the projection of \eqref{11III23.2} onto $(\ker[\overadd{p}{\psi}(P)])^\perp$ can be solved uniquely for $\kphit{AB}{(7-n+2p)/2}^{[(\ker\overadd{p}{\psi}(P))^\perp]}$. 

\underline{when $m=0$} but $\alpha \neq 0$, \eqref{11III23.2} can be solved uniquely for the interpolating field  $\kphit{AB}{(7-n-2p)/2}$ for all $p \geq 2$ when $n$ is even, and for $2 \leq p < \frac{n-3}{2}$ when $n$ is odd. 

For the latter case,
%
\FG{6VII23: Addition for overlap of $5-n$ fields.}
%
\FG{Again we solve for the projection to $\TTt$ but what about the equations for the projection to $\TTtp$. Does this stop a continuous gluing?}
%
\tcp{when $p=\frac{n-3}{2}$ the field $\kphit{AB}{(7-n-2p)/2}{}^{[\TTt^\perp]} = \kphit{AB}{5-n}^{[\TTt^\perp]}$ has already been determined in \eqref{7III23.1} gluing $\chi$, and only the $\TTt$ part is free. So we solve the projection of \eqref{11III23.2} onto $\TTt$ uniquely for the field $\kphit{AB}{5-n}^{[\TTt]}$. Notice that when $n=5$ this implies $p=1$ and this case was already addressed when gluing $q_{AB}:=\overadd{1}{q}_{AB}$.} \tcp{Likewise, } when $p=\frac{n-1}{2}$, the field $\kphit{AB}{(7-n-2p)/2}{}^{[\TTt^\perp]} = \kphit{AB}{4-n}^{[\TTt^\perp]}$ has already been determined in \eqref{7III23.4} and only the $\TTt$ part, $\kphit{AB}{4-n}^{[\TTt]}$, remains free. We can thus solve the projection of \eqref{11III23.2} with $p=\frac{n-1}{2}$ onto $\TTt$ uniquely for the field $\kphit{AB}{4-n}^{[\TTt]}$.
We are also free to set the remaining free fields $\kphit{AB}{(7-n+2p)/2}$ to any convenient value e.g. to zero.

Similarly, when $m\neq 0 $ the fields $\kphit{AB}{(7-n + 2p(n-1))/2}$ are free up to this point and equation \eqref{11III23.2} can be solved uniquely for the field $\kphit{AB}{(7-n + 2p(n-1))/2}$.

In \eqref{11III23.2}, the $m (\ldots)$ term, which is there only \underline{when $m\neq 0$}, arises from the sum $\sum_{j,\ell}^{p_{**}}$ of \eqref{6III23.w6} with $i=p$. After integrating, this sum contains the fields $\kphi{i}_{AB}$ with $\frac{n+5}{2}-2(p-1) \leq i \leq \frac{7+2p(n-1) - n}{2}$, which are either predetermined, or are free at this point. In the latter case, we set these free fields to zero. 
We leave out the explicit formula of these and the gauge fields appearing in \eqref{11III23.2}; these can be determined order-by-order in the index $p$ using the recursion formula \eqref{6III23.w6} and the gauge transformations \eqref{17III22.1HD}-\eqref{17III22HD}.

\paragraph{The case $n$ odd, $p\geq \frac{n+1}{2}$.}
 It follows from the transport equation \eqref{17IV23.2}  that the gluing of $\partial_u^p \tilde h_{AB}$ requires, for $j\geq 0$,
 %
  \ptcr{a problem with an infinite dimensional space of non-gauge obstructions which shows up???? but perhaps not there if m is non zero}
\begin{align}
    \overadd{\frac{n+1}{2}+j}{q}_{AB} \big|_{\secN_2} -\overadd{\frac{n+1}{2}+j}{\tilde q}_{AB} \big|_{\tilde\secN_1} 
    &=   \int_{r_1}^{r_2} [  \overadd{\frac{n+1}{2}+j}{\psi}(P) \hkappa_{4+j}(s) \tilde h_{AB}
    + \overadd{\frac{n+1}{2}+j}{\psi}_L(P) \circ P \hkappa_{4+j}(s) \log\big(\frac{s}{r_2}\big) \tilde h_{AB}
    \nonumber
    \\
    &\qquad\qquad
    + m^{\frac{n+1}{2}+j} \overadd{\frac{n+1}{2}+j}{\psi}_m \hkappa_{j(n-1)-\frac{n-n^2-6}{2}}(s) \tilde h_{AB} 
    \ ] \ ds
    \nonumber
    \\
    &\quad
    + m (\ldots)
    +\text{ gauge fields}\, .
    \label{15VI.1}
\end{align}
%
In \eqref{15VI.1}, the $m (\ldots)$ term, which is there only \underline{when $m\neq 0$}, arises from the sum $\sum_{k,\ell}^{j_{*'}}$ of \eqref{17IV23.2}.  
In the case $m\neq 0$, we solve \eqref{15VI.1} uniquely for the field $\kphit{AB}{j(n-1)-\frac{n-n^2-6}{2}}$. The other interpolating fields $\kphi{i}_{AB}$ appearing in the sum $\sum_{k,\ell}^{j_{*'}}$ are either predetermined, or free at this point, in which case we set them to zero.

For the case $m = 0$, we first note that Equation \eqref{15VI.3} implies 
%
$$(\ker \overadd{\frac{n+1}{2}+j}{\psi}(P))^\perp\,, (\ker \overadd{\frac{n+1}{2}+j}{\psi}_L(P))^\perp \subseteq \TTt
\,.$$ 
%
However, we also have $P h^{[\TTt]}= P^\dagger h^{[\TTt]}=0$. It follows that logarithmic term in \eqref{15VI.1} vanishes upon projection onto $(\ker \overadd{\frac{n+1}{2}+j}{\psi}(P))^\perp$. Moreover, from \eqref{15VI.6}, the fields $\kphi{4+j}_{AB}^{[\TTt]}$ remain free.
We thus can solve the projection of \eqref{15VI.1} onto $(\ker \overadd{\frac{n+1}{2}+j}{\psi}(P))^\perp$ uniquely for the field $\kphi{4+j}_{AB}^{[(\ker \overadd{\frac{n+1}{2}+j}{\psi}(P))^\perp]}$. 

As in the $(n,p)$ convenient case, we leave out the explicit formula of the $m (\ldots)$ and the gauge fields appearing in \eqref{15VI.1}; these can be determined order-by-order in the index $p$ using the recursion formula \eqref{17IV23.3} and the gauge transformations \eqref{17III22.1HD}-\eqref{17III22HD}.

==> HDkappsWithLogs.tex <==

{\blueca{16viii22; log terms added; need to think this through}

When $\alpha \ne 0$ the construction is marginally more involved. This is due to the fact that for $j<i$  the functions $\overset{(i,j)}{\psi}(s,r)$ and $\overset{(i,j)}{\chi}(s,r)$ are not polynomials in $1/s$ anymore, but are instead linear combinations of $s^k \ln ^\ell s$, $\Z\ni k \ge - (i+3)$, $\ell \in \N$, with coefficients which depend upon $r$. However, the key functions used for the gluing, namely $\overset{(i,i)}{\psi}(s,r)$ and $\overset{(i,i)}{\chi}(s,r)$ are independent of $\alpha$, and thus identical to the case $\alpha =0$.
 \ptcr{chi?}
We also note that the $\ln s$ terms appear only for $i\ge 3$.

The functions $\kappa_i$ are now constructed recursively as follows: \green{For $-2\leq i \leq 0$, let $\hkappa_i:=s^i$.} For $i\ge 1$ let $\{\hat \kappa_k\}_{k \le N_i}$ denote the minimal collection of functions
$s^k \ln ^\ell s$ so that the functions $\overset{(\ell,m)}{\psi}(s,r)$ and $\overset{(\green{\ell-1},m)}{\chi}(s,r)$ with $\ell\le i$ are linear combinations of the $\hat\kappa_k$. We order them so that the collection $\{\hat\kappa_k\}_{k \le N_i}$ are the first functions in $\{\hat\kappa_k\}_{k \le N_{i+1}}$, with
 \ptc{I still need to understand the $\chi$'s to write it right}
 $\hat\kappa_{N_i}= s^{-(i+3)}$.

We let the collection $\{f_k\}$ be obtained by a Gram -Schmidt orthonormalisation of    $\{\hat\kappa_k\}$, with respect to the scalar product  in the space $\mathbb{H}$ above. We set
%
$$   \red{\kappa}_i  = c_i \red{\chi} f_{N_i}
 \,,
$$
%
with a suitably chosen constant $c_i\ne 0$, so that the functions so-defined satisfy
%
\begin{eqnarray}
  &
  \displaystyle
\ip{\kappa_i}{\hat \kappa_j}  = 0
 \quad \mbox{for $j<N_i$}
  \,,
  &
  \label{13VIII22.1c}
   \\
   &
  \displaystyle
 \ip{\kappa_i}{\hat \kappa_{N_i}}  = 1
  \,.
  &
  \label{13VIII22.2c}
\end{eqnarray}
%
} 

==> HDlineariseTrace.tex <==
Linearising in vacuum, with $\partial_u^i\delta \beta =0$, this is the same as
%
\begin{align}
   r^{-1} \gamma^{AB} \delta G_{AB} =      \partial_r^2 \delta V  - (
       2 D_{A}\delta U^{A}  +  r D_{A}\partial_r\delta U^{A}
       )
     \,.
\end{align}
%
Equivalently
%
\begin{align}
\label{9X22.w1}
       r^{-1} \gamma^{AB} \delta G_{AB} =   \partial_r
        \big( \partial_r \delta V -   r D_{A} \delta U^{A}
        \big)
        -
         D_{A}\delta U^{A}
     \,.
\end{align}
%
%When $\chi$ is already known to be constant, we can use \eqref{24IX22.2} to rewrite the equation  $\gamma^{AB} \delta G_{AB}=0$ as
% \ptcr{i am not quite sure about the logic here; and this equation looks pretty bad to me ...}
% %
% \begin{align}
%         \partial_r
%         \big( \partial_r
%         (- \frac{ r}{2}\partial_r  \zspaceD^A  h_{uA}
%        +\frac{1}{2r}  \zspaceD^A\zspaceD^B h_{AB}
%        ) -   r D_{A} \delta U^{A}
%         \big)
%          &=
%          D_{A}\delta U^{A}
%      \,.
% \end{align}
% %
We can instead use \eqref{27III2022.3b}, namely
%
 \begin{align}
             \green{-}\frac 12  \gamma^{AB} \delta R_{AB}
              = \
              &
                 \partial_r( \delta V  -  \frac{ r^{2 }}{2}
                \zspaceD_A \delta U^A)
              -
                 \frac{1}{2}
                  \zspaceD^A\zspaceD^B\zhTB_{AB}
                -
                 r\zspaceD_A\delta U^A
                 \nonumber
\\                   = \
              &
                 \partial_r  \delta V  -  \frac{ r^{2 }}{2}
                \zspaceD_A \partial_r \delta U^A
              -
                 \frac{1}{2}
                  \zspaceD^A\zspaceD^B\zhTB_{AB}
                -
                2 r\zspaceD_A\delta U^A
                  \,.
                   \label{27III2022.3bwr}
           \end{align}
%
to obtain
%
\begin{align}
    r^{-1} \gamma^{AB} \delta G_{AB} =     \partial_r
        \Big[ \green{-} \frac 12  \gamma^{AB} \delta R_{AB}
        +
       \underbrace{
        \partial_r(  \frac{ r^{2 }}{2}
                \zspaceD_A \delta U^A)    + \frac{1}{2}
                  \zspaceD^A\zspaceD^B\zhTB_{AB}
        \Big]
          -
         D_{A}\delta U^{A}
         }
     \,,
\end{align}
%
where the underbraced term is a half of
%
\begin{align}
       2 \zspaceD^A   \delta G_{rA}
        =  \partial_r
        \Big[ 2 r
                \zspaceD_A \delta U^A
                    +    r^{2 }
                \zspaceD_A \partial_r \delta U^A
                    +
                  \zspaceD^A\zspaceD^B\zhTB_{AB}
        \Big]
         &
         -
         2 D_{A}\delta U^{A}
     \,.
\end{align}
%
 i.e.
%
\begin{align}
  4 r
                \zspaceD_A \partial_r\delta U^A
                    +
                    2
                \zspaceD_A \delta U^A
                    +    r^{2 }
                \zspaceD_A \partial_r^2 \delta U^A
                    +
                  \zspaceD^A\zspaceD^B \partial_r \zhTB_{AB}
         -
         2 D_{A}\delta U^{A}
     \,.
     \label{1X22.99}
\end{align}
%
To see this, note that
\eqref{CHG28XI19.5} $= 2r^2  \delta G_{rA}$  gives,
%
\begin{eqnarray}
          &&
           \partial_r \left[r^4  \partial_r \delta U^A
            \right]
            +
             r^2
                   \partial_r \left(r^{-2}
                    \zspaceD^B\red{h}_{AB}\right)
                 \,,
           \end{eqnarray}
%
or,  after dividing by $r^2$,
%
\begin{eqnarray}
          &&
           r^2  \partial_r^2  \delta U^A
           +
           4 r   \partial_r \delta U^A
           +
                   \partial_r \left(r^{-2}
                    \zspaceD^B\red{h}_{AB}\right)
                 \,,
                            \label{1X22.97}
           \end{eqnarray}
%
which agrees with \eqref{1X22.99} after taking $\zspaceD_A$, and establishes \eqref{5X22.w4}.

We check \eqref{5X22.w4} directly. First from \eqref{8X22.w1},
%
 \begin{align}
             \frac 12  \gamma^{AB}\partial_r \delta R_{AB}
              &
              = \frac 12  \partial_r(\gamma^{AB} \delta R_{AB})
          \nonumber
\\              &=
               \partial_r\left(-  \partial_r  \delta V  +  \frac{ r^{2 }}{2}
                \zspaceD_A \partial_r \delta U^A
              +
                 \frac{1}{2}
                  \zspaceD^A\zspaceD^B\zhTB_{AB}
                +
                2 r\zspaceD_A\delta U^A\right)
                \nonumber
\\
    &=
    -\partial^2_r  \delta V  +  r
                \zspaceD_A \partial_r \delta U^A
                 +  \frac{ r^{2 }}{2}
                \zspaceD_A \partial^2_r \delta U^A
                - \frac{1}{r^3} \zspaceD^A\zspaceD^B\hBo_{AB}
                \nonumber
\\&\qquad
                +
                 \frac{1}{2r^2}
                  \zspaceD^A\zspaceD^B \partial_r \hBo_{AB}
                  +
                2 \zspaceD_A\delta U^A
                +
                2 r\zspaceD_A\partial_r \delta U^A
                  \,,
                   \label{7X22.wb1}
           \end{align}
%
while we already have from \eqref{1X22.99},
%
\begin{align}
  \zspaceD^A \delta G_{rA} = 2 r
                \zspaceD_A \partial_r\delta U^A
                    +   \frac{1}{2} r^{2 }
                \zspaceD_A \partial_r^2 \delta U^A
                    +
                  \frac{1}{2} \zspaceD^A\zspaceD^B \partial_r \zhTB_{AB}
     \,.
     \label{1X22.w99}
\end{align}
%
It follows that 
%
\begin{align}
    -\frac{1}{2}\gamma^{AB}\delta R_{AB} &
      + \zspaceD^A \delta G_{rA}
      \nonumber
\\      
    &=\partial^2_r  \delta V  -  r
                \zspaceD_A \partial_r \delta U^A
                 -  \frac{ r^{2 }}{2}
                \zspaceD_A \partial^2_r \delta U^A
                + \frac{1}{r^3} \zspaceD^A\zspaceD^B\hBo_{AB}
                \nonumber
\\&\qquad
                -
                 \frac{1}{2r^2}
                  \zspaceD^A\zspaceD^B \partial_r \hBo_{AB}
                  -
                2 \zspaceD_A\delta U^A
                -
                2 r\zspaceD_A\partial_r \delta U^A
    \nonumber
    \\
    &\qquad
    +2 r
                \zspaceD_A \partial_r\delta U^A
                    +   \frac{1}{2} r^{2 }
                \zspaceD_A \partial_r^2 \delta U^A
                    +
                  \frac{1}{2r^2} \zspaceD^A\zspaceD^B \partial_r \hBo_{AB}
                  -\frac{1}{r^3}\zspaceD^A\zspaceD^B \hBo_{AB}
                  \nonumber
\\
    &=
    \partial^2_r  \delta V  -  r
                \zspaceD_A \partial_r \delta U^A
              -
                2 \zspaceD_A\delta U^A
                 \,,
\end{align}
%
which equals $r^{-1}\gamma^{AB}\delta G_{AB}$ by \eqref{9X22.w1}, hence verifying \eqref{5X22.w4}.

{\redc Indeed, \eqref{5X22.w4} follows from the Bianchi identity when $\partial_u^i \delta G_{rr}=0$ for $i=1,2$. First, note that from the linearisation of \eqref{5X22.w1}, we have, with  $\partial_u^i \delta G_{rr}=0$,
%
\begin{align}
    \label{23X22.w1}
    \frac{1}{2}\ringh^{AB}\delta R_{AB} &= r^2 \delta G_{ur}
    \nonumber
\\
 \implies
 \frac{1}{2}\ringh^{AB}\partial_r \delta R_{AB} &= 2r \delta G_{ur} + r^2 \partial_r\delta G_{ur}\,,
\end{align}
%
and hence identity \eqref{5X22.w4} is equivalent to
%
\begin{align}
    \zspaceD^A \delta G_{rA} - \frac{1}{r} \ringh^{AB}\delta G_{AB} = 2r \delta G_{ur} + r^2 \partial_r\delta G_{ur}\,.
    \label{23X22.w2}
\end{align}
%
Meanwhile, it follows from the divergence identity \eqref{27IX22.2} with $\nu=r$ that
%
\begin{align}
    0&= \frac{1}{\sqrt{|g|}}\partial_{\mu}(\sqrt{|g|}\mcE^{\mu}_r)
    + \frac12 \partial_r(g^{\mu\rho})\mcE_{\mu\rho}\,.
    \label{23X22.w3}
\end{align}
%
The linearisation of \eqref{23X22.w3} with $\partial_u^i \delta G_{rr}=0$ gives,
%
\begin{align}
    0&=
    -\frac{1}{r^2}\partial_r(r^2 \delta G_{ur})
    +\frac{1}{r^2}\zspaceD^A\delta G_{rA} 
    + \frac12 \partial_r\left(\frac{1}{r^2}\ringh^{AB}\right)\delta G_{AB}\,,
\end{align}
%
and hence,
%
\begin{align}
    2r \delta G_{ur} + r^2 \partial_r\delta G_{ur}&=
    \zspaceD^A\delta G_{rA} 
    - \frac1r \ringh^{AB} \delta G_{AB}\,,
\end{align}
%
which agrees with \eqref{23X22.w2}.
}

==> HDorderkkernel.tex <==
Quite generally, for $C^k$-gluing on $S^2$, the operator $\sum_{i=0}^{k}  \overset{(k,i)}{\ochi}_{k+4}  P^i $ appearing in \eqref{24X22.91} is of the form
%
\begin{align}
   \sum_{i=0}^{k}  \overset{(k,i)}{\ochi}_{k+4} (r_2)  P^i
   =
    \blue{\hat c_k}\prod_{i=1}^k (P+a_i)\,,\qquad
   a_i = \frac{1}{2}i(3+i)\,,
   \label{26X22.w1}
 \end{align}
%
where
 \ptcheck{28X}
%
$$\blue{\hat c_k}
= \frac{1}{ (k+3)k!}
\,.
$$
%
This can be verified by induction.

Indeed, when  $k=1$ this is \eqref{26VII22.3c} with $\hat c_1=1/4$. Using the recursion formula \eqref{16VIII22.12} with $\twoscsign=1$, a straightforward calculation shows that the $\hkappa_{k+5}$ component of the $(k+1)$-order coefficient  are  given by
\ptcheck{27X22}
%
\begin{equation}
    \overset{(k+1,i)}{\ochi}_{k+5} = \blue{c_k} \times \left\{
       \begin{array}{lll}
        a_{k+1} \overset{(k ,0)}{\ochi}_{k+4}\,,
          & \hbox{$i=0$}
           \,,
        \\[5pt]
          a_{k+1}\overset{(k ,i)}{\ochi}_{k+4}  + \overset{(k,i-1)}{\ochi}_{k+4}\,,
           &  \hbox{$1\leq i \leq k$}
            \,,
        \\[5pt]
        \overset{(k ,k)}{\ochi}_{k+4}\,,
          &  \hbox{$i = k+1$}
           \,,
       \end{array}
     \right.
\end{equation}
%
with $\blue{c_k} = \frac{k+3}{(k+4)(k+1)}$. Therefore, assuming \eqref{26X22.w1}, the operator at order $k+1$ is actually $r_2$-independent and reads,
\ptcheck{27X22}
%
\begin{align}
    \sum_{i=0}^{k+1}  \overset{(k,i)}{\ochi}_{k+5} (r_2)  P^i
   &= \blue{c_k} \sum_{i=0}^{k}  \left(\overset{(k,i)}{\ochi}_{k+4}   P^{i+1}
   +
   a_{k+1} \overset{(k,i)}{\ochi}_{k+4}   P^i \right)
   \nonumber
   \\
   &=
   \blue{c_k} \sum_{i=0}^{k}  \big(\overset{(k,i)}{\ochi}_{k+4}   P^{i} \big) (P+ a_{k+1})
      \nonumber
   \\
   &=
    \blue{c_k} \hat c_k  (P+ a_{k+1}) \prod_{i=1}^k  (P+a_i)
   \nonumber
   \\
    &=
    \blue{ \hat c_{k+1}}  \prod_{i=1}^{k+1} (P+a_i)\,,
    \qquad \text{with} \ \blue{\hat c_{k+1}}=  \blue{c_k} \hat c_k
    \,.
\end{align}
%
It thus follows from \eqref{26X22.w3} that spherical harmonic vector fields with mode $\ell\ge 0 $ satisfying
%
\begin{align}
    0&=\prod_{i=1}^{k} \left(-\frac{1}{2}\ell(\ell+1)+ 1 + a_i\right)
    =
    \frac{1}{2} \prod_{i=1}^{k} (1+i-\ell)(2+i+\ell)
\end{align}
%
  belong to $\ker\left(\sum_{i=0}^{k}  \overset{(k,i)}{\ochi}_{k+4}  P^i \right)$. The corresponding values of $\ell$ are  $\ell = 2,...,k+1$.
 \ptcheck{27X}



==> HigherDimSolutions.tex <==

\subsection{Linearized Kerr--deSitter in Bondi Gauge}

 \ptcr{either should be moved after the next section; if kept here some crossreferences need changing}
Going one step further we can linearise the metric \eqref{3VI24.f7}
%
\footnote{Again we have dropped the bars on the coordinates and parameters for convenience.}
%
by expanding to linear order in the various rotation parameters $a_i$ which gives the higher dimensional Lense--Thirring metric
%
\begin{align}\label{eq: LTHD}
ds^2_{LT}&=-fd{t}^2+\frac{d{r}^2}{f}+{r}^2\left(\sum_{i=1}^\red{N} {\mu}_i^2d\phi_i^2+\sum_{i=1}^{\red{N}+\delta}\!d{\mu}_i^2 \right)
\nonumber\\
&
+\frac{4m}{r^{n-2}}\left(\sum_{i=1}^\red{N+\delta-1} a_i\mu_i^2dtd\phi_i +a_{N+\delta}\mu_{N+\delta}^2dtd\phi_{N+\delta}\right)
 +\red{O}(a_i^2)
 \,,
\\
  f&=\!\sigma^2-\alpha^2r^2-\frac{2m}{r^{n-2}}+\red{O}(a_i^2)\,.
\end{align}
%
Notice that at this linearised level we are free to rescale $a_{N+\delta}=\sigma^{-2}\bar{a}_{N+\delta}$ and then can rewrite this as a perturbation on the Birmingham--Kottler metrics%\footnote{At least for spherical topologies.}%
~\eqref{23VII22.3} by identifying $\sigma^2=\myGauss$, noting that the term in the brackets of \eqref{eq: LTHD} is just the metric  $\ringh_{AB}dx^A dx^B$ on the $(n-1)$-sphere, torus or hyperbolic space, depending on if $\sigma^2=1,0,-1$ respectively due to the constraint \eqref{3VI24.f5}. Then by performing the coordinate transformation
\begin{equation}
	dt=du+\frac{dr}{f}\,,
\end{equation}
we have,
\begin{equation}\label{21V24f.1}
	ds^2_{LT}={\nobarzg}_{\a \b} dx^\a dx^\b +\frac{4m}{r^{n-2}}\sum_{i=1}^\red{N} a_i\mu_i^2d\phi_i(du+dr/f)+\red{O}(a_i^2)\,.
\end{equation}

This is manifestly not in Bondi gauge as there are $g_{rA}$ components, however we can address this in two ways which turn out to be equivalent. First, outside of all horizons,  we could accompany the change from the $t$- to the $u$-coordinate with   $r$-dependent rotations of the  $(\mu_i,\phi_i)$ planes,
%
\begin{equation}\label{eq: Coord change}
	d\varphi_i=d\phi_i-\frac{2ma_i}{r^{n} f}dr
\,,
\end{equation}
%
which transforms the metric to
\begin{equation}\label{eq: Lin Kerr Bondi}
ds^2_{LT}={\nobarzg}_{\a \b} dx^\a dx^\b +\frac{4m}{r^{n-2}}\sum_{i=1}^\red{N} a_i\mu_i^2d\varphi_idu+\red{O}(a_i^2)\,.
\end{equation}%
%One may wonder if this is a smooth transformation but it is the standard one done for putting Kerr into modified outgoing Eddington-Finkelstein coordinates (see e.g. Appendix C.7 of (\cite{Chrusciel:2002cp} where it is claimed that this is a smooth map).
% \ptcr{to be settled}


Second we could perform an infinitesimal gauge transformation generated by $\zeta^\mu$ to put the perturbation into Bondi form (\`a la Section 3 of~\cite{ChHMS}). Denoting the perturbation in \eqref{21V24f.1} by $h_{\mu\nu}$, the vector $\zeta$ satisfies
\begin{align}
	{\cal L}_\zeta (g_{rr} +h_{rr}) &=0\,,\\
	{\cal L}_\zeta (g_{rA} +h_{rA}) &=0\,,\\
	g^{AB}{\cal L}_\zeta (g_{AB} +h_{AB}) &=0\,.
\end{align}
Given that the nonzero components of $h_{\mu\nu}$ are
\begin{align}
h_{rA}=\frac{2ma_i}{r^{n-2}f} \ringh_{AB}\delta^B_{\phi_i}\,,\quad
h_{uA}=\frac{2m a_i}{r^{n-2}} \ringh_{AB}\delta^B_{\phi_i}
 \,.
\end{align}
%
The first two conditions are equivalent to
%
\begin{align}
\partial_r \zeta^u-\frac{1}{2}h_{rr} &=0\,,\\
\partial_r \zeta^A-\frac{\ringh^{AB}}{r^2}\left(\partial_B \zeta^u-h_{rB}\right)&=0\,,
\end{align}
%
and one can check that~\cite[Section~3]{ChHMS}
%
\begin{equation}
	\zeta^r=-\frac{1}{n-1}\left(r\zspaceD_B\zeta^B+\frac{1}{2r}\ringh^{AB}h_{AB}\right)\,.
\end{equation}

Given that $h_{rr}=0=h_{AB}$ we can choose $\zeta^u=0$, and then the only non zero components of the vector are
\begin{equation}
	\zeta^A=2ma_i\delta^A_{\phi_i}\int_{r_0}^{r}\frac{1}{s^nf}ds\,,
\end{equation}
which puts the metric exactly into \eqref{eq: Lin Kerr Bondi}. Using that $\zeta^A$ generates the infinitesimal transformation $x^A\to x^A+\xi^A$ one can check that this is equivalent to \eqref{eq: Coord change}.


Finally, identifying the angular momentum as  $J_i=m a_i$,
% \ptcr{crosscheck whether the sign is ok, since we have a different sign on the ai's as gibbons}
% \FG{4XI23: Have checked. David et al. use the opposite sign as Gibbons to aid some calculations (this is where the minus comes from). Then the minus here depends on how you define angular momentum. I think we are consistent here.}
 clearly the linearised Kerr--(A)dS spacetime adds the following perturbations
  \ptcr{we should add a conclusion, that this changes the charges}
 %
\begin{equation}
	\delta V=0=\delta \beta\,,\quad \delta U^A=-\frac{2J_i }{r^{n}}\,\delta^A_{\phi_i} \,.
\end{equation}
\FG{worth discussing...}
%It is interesting to note that this is actually a generalization of  this form the solution can easily be generalized upgraded to non-spherical topologies by replacing $f$ with $\zguu:=\myGauss-\alpha^2r^2-{2m}{r^{-(n-2)}}$, the metric on the sphere with the metric on the general transverse space $\secN$, and setting
This form can be reconciled with our linearised Einstein equations in Section~\ref{s3X22.1} by noting that any perturbation of the form
\begin{equation}
\delta U^A=\frac{\zlambda^A(x^C) }{r^{n}} \,, 
\quad
\delta \beta=0\,
\quad	
\delta V=\text{const}.
\end{equation}
where $\zlambda_A(x^C)$ is an arbitrary Killing vector of the transverse space~$\secN$ is a linearized solution. These $	\delta V=\text{const}$ perturbations generate changes in the mass parameter of the Birmingham--Kottler metrics.



==> InconvenientCaseOld.tex <==
\subsubsection{The $(n,k)$ inconvenient case}
\label{ss5IX23.1}


Recall that the case $m = 0$ has already been covered above. We therefore consider here the case $m\neq 0$.
\wcb{below written for $\alpha = 0$; $\alpha \neq 0$ does not change the number of obstructions, and follows a similar scheme; consider adding in later}

In $(n,k)$ inconvenient case, the equation for $\overadd{p}{\Hf}_{uA}$ in \eqref{11III23.1} and that for $\overadd{p}{q}{}^{[\TTtp]}_{AB}$ in \eqref{11III23.2} may involve $\kphi{i}_{AB}^{[\TTtp]}$'s of the same index $i$. This requires us to consider the $\overadd{p}{\Hf}_{uA}$ and $\overadd{p}{q}_{AB}^{[\TTtp]}$ equations together as a system of coupled equations. 

For the $\overadd{p}{\Hf}_{uA}$ fields, recall from \eqref{20VIII23.1} that we require
%
 \begin{align}
     \overadd{p}{S}_{AB}
       &=
    \sum_{i=5}^{p(n-1)+4}
    \overadd{p}{\chi}_{i} \kphi{i}_{AB}^{[\TTtp]}\,, \quad 1 \leq p \leq k\,,
    \label{3IX23.3}
 \end{align}
 %
 where the source term $\overadd{p}{S}_{AB}$ has been defined in \eqref{19VIII23.2}.  In addition, items (i)-(iii) of Section \peqref{e3IX23.1} continues to hold.

 Next, for the $\overadd{p}{q}_{AB}$ fields, equation \eqref{11III23.2} can be still be written, similar as to the convenient case, as 
 \wcb{the lower bound will be $\frac{7-n-2p}{2}$ instead if $\alpha \neq 0$}
 %
\begin{align}
    \overadd{p}{r}_{AB} = \sum_{j=\frac{7+n-2p}{2}}^{\frac{7-n+2p(n-1)}{2}} \overadd{p}{\psi}_j \kphi{j}_{AB} \,,
    \quad
    1 \leq p \leq k \,.
    \label{3IX23.w1}
\end{align}
%
Indeed, the case $ 1 \leq p \leq \frac{n-1}{2}$ follows exactly the analysis in the convenient case, with the source term being defined in \eqref{22VIII23.2}. Meanwhile, from the transport equation \eqref{17IV23.2} for $\overadd{p}{q}_{AB}$, $p \geq \frac{n+1}{2}$, the terms which do not fit into the structure of \eqref{3IX23.w1} are those of the form
\wcb{this is not explicit yet, but follows from the recursion proof; make a statement somewhere, or maybe even rewrite the appendix setting the relevant terms to zero?}
%
\begin{equation}
     \log (\tfrac{r}{r_2}) \hat{\psi}\circ \ck{-2}{P} \ck{-1}{P} P(h)_{AB}
\end{equation}
%
for some arbitrary operator $\hat\psi$. However these are vanishing. Indeed, we have $P(h^{\TTt})=0$, and $\ck{-2}{P} \ck{-1}{P} h^{\TTtp}_{AB}=0$ (cp. \eqref{21VIII23f1}) which together imply $$\ck{-2}{P} \ck{-1}{P} P(h)_{AB}=0 \,.$$

In addition, items (i)-(iii) of Section \peqref{e3IX23.2} continues to hold for $1 \leq p \leq \frac{n-3}{2}$. For $\frac{n-1}{2} \leq p \leq k$, (i) and (iii) continues to hold and (ii) is irrelevant.

Let us now consider the coupled system of equations for $\overadd{p}{\Hf}_{uA}$ and $\overadd{p}{q}{}^{[\TTtp]}_{AB}$. 
For $k \ge 1$ we let
%
\begin{align}
t_k := \left(
             \begin{array}{c}
                \overadd{1}{r}{}^{[\TTtp]}_{AB} \\
                \overadd{1}{S}_{AB} \\
               \vdots \\
                \overadd{k}{r}{}^{[\TTtp]}_{AB}  \\
                \overadd{k}{S}_{AB}  \\
             \end{array}
           \right)
           \,,
           \qquad
 \upsilon_k &:= \left(
             \begin{array}{c}
               \kphi{\frac{9-n}{2}}{}^{[\TTtp]}_{AB} \\
                \kphi{\frac{11-n}{2}}{}^{[\TTtp]}_{AB} \\
               \vdots \\
                \kphit{AB}{4+k(n-1)}{}^{[\TTtp]} \\
             \end{array}
           \right)
           \,.
\end{align}
 %
The system \eqref{3IX23.3} and the projection of \eqref{3IX23.w1} onto $\TTtp$ can then be written as
%
\begin{align}
    t_k = \Lambda_k \upsilon_k\,,
    \label{4IX23.1}
\end{align}
%
where $\Lambda_k$ is a $k \times \frac{2k(n-1)+n+1}{2}$ matrix given by,
%
\begin{align}
    \Lambda_k = \begin{pmatrix}
        \overadd{1}{\psi}_{\frac{9-n}{2}} & \ldots & \overadd{1}{\psi}_{4+k(n-1)} \\
        \overadd{1}{\chi}_{\frac{9-n}{2}} & \ldots & \overadd{1}{\chi}_{4+k(n-1)} \\
        \vdots & \ddots & \vdots\\
        \overadd{k}{\psi}_{\frac{9-n}{2}} & \ldots & \overadd{k}{\psi}_{4+k(n-1)} \\
        \overadd{k}{\chi}_{\frac{9-n}{2}} & \ldots & \overadd{k}{\chi}_{4+k(n-1)}
    \end{pmatrix}
    \,.
\end{align}
 %
Now, it follows from the two item (i)'s above that each of the elements in $\Lambda_k$ is either a scalar, product of operators of the form $L_{a,c}$ in \eqref{20VIII23.3}, or sums thereof. Moreover, these are self-adjoint, pairwise commuting and elliptic. The former two properties follow from Lemma \ref{L18VIII23.1}. The only concern for ellipticity would be the appearance of the operators $\ck{-1}{P}$ and $\ck{-2}{P}$ in the $\overadd{p}{\psi}_j$ coefficients. However, it follows from Appendix \ref{A4IX23.1} that $\ck{-2}{P}$ always appears as $\ck{-2}{P}\ck{-1}{P}$, which vanishes when acting on $h^{[\TTtp]}$ (cp. Appendix \ref{ss13VI.1}), while $\ck{-1}{P}$ is either elliptic (when acting on $h^V$, cp. below \eqref{4IX23.4}) or vanishing (when acting on $h^S$, cp. \eqref{4IX23.3}).

 Thus, there exists a complete set of smooth,
 pairwise $L^2$-orthogonal, joint eigenfunctions $\phi_\ell$ of all the $L_{a,c}$'s appearing in $\Lambda_k$, with a corresponding discrete set of eigenvalues $\lambda_{a,c,\ell}\to_{\ell \to \infty} \infty$. We can therefore write 
 \wcb{$\phi{}_\ell^{[\TTtp]}$?}
 %
 \begin{align}
     t_k = \sum_\ell t_{k,\ell} \phi_\ell \,,\quad 
     \upsilon_k =  \sum_\ell \upsilon_{k,\ell} \phi_\ell
     \label{4IX23.7}
 \end{align}
 %
 and \eqref{4IX23.1} can be solved mode-by-mode:
 %
 \begin{align}
    t_{k,\ell} = \Lambda_k \upsilon_{k,\ell}  
    \iff 
     t_{k,\ell}  = \Lambda_k|_{L_{a,c}\mapsto \lambda_{a,c,\ell}}  \upsilon_{k,\ell}  \,.
 \end{align}
 %

 \begin{Lemma}
 \label{L4IX23.1}
     For each $\ell$, the equation
     %
     \begin{equation} 
     \label{4IX23.5}
     t_{k,\ell}  = \Lambda_k|_{L_{a,c}\mapsto \lambda_{a,c,\ell}}  \upsilon_{k,\ell} 
     \end{equation}
     %
     is solvable. 
     It is also solvable after removing a finite number of rows associated with $\overadd{p}{r}{}^{[\TTtp]}_{AB}$ for $\frac{n-3}{2} \leq p \leq k$ from the equation.
     %\wc{note that these fields \textit{do not} add new $\kphi{j}$'s into the system; i.e., removing them do not reduce the number of free fields and thus the length of $\upsilon$ remains unchanged.}
 \end{Lemma}

 This can be proved in a similar way as in the convenient case. Note in particular that the matrix $\Lambda_k$ is simply made up of rows coming from the matrices $(0_{\frac{n-3}{2}\times \frac{n-3}{2}}\, \chi_k\, M_k)$ of \eqref{22VIII23.5}  and $(\psi_k  \, N_k \, 0_{\frac{n-3}{2}\times \frac{n-3}{2}})$, leading to an adjoint matrix $\Lambda_k^\dagger$ which has a similar structure to that in \eqref{27VII23.w1}:
 %
 \begin{align}
     \label{5IX23.w1}
     \left(\begin{array}{l}
            \begin{array}{|cccccc|}
            \hline
               \overadd{1}{\psi}_{\frac{9-n}{2}}            &  \overadd{1}{\chi}_{\frac{9-n}{2}}  & \dots \quad \dots    & \ldots \quad \dots  & \dots\quad\dots\quad \dots\quad\dots   \quad \ldots    &  \, \overadd{k}{\chi}_{\frac{9-n}{2}} \phantom{LL}
               \\
               \vdots           &  \vdots  &     &   &     &  \, \vdots 
               \\
               \fbox{ $\overadd{1}{\psi}_{\frac{7-n}{2}+(n-1)}$ } &  \overadd{1}{\chi}_{\frac{7-n}{2}+(n-1)}  & \dots \quad \dots    & \ldots \quad \dots  & \dots\quad\dots\quad \dots\quad\dots      \quad \ldots & \, \overadd{k}{\chi}_{{\frac{7-n}{2}+(n-1)}} 
               \\
            \hline
            \end{array}
                \\ \vspace{-.4cm}
        \\
            \begin{array}{|cccccc|}
            \hline
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0       &   \hspace{2cm}    & 0         & \hspace{1cm} \overadd{1}{\chi}_{{\frac{9-n}{2}+(n-1)}}        & \ldots\quad\dots\quad\dots\quad \ldots \quad\dots\quad \ldots & \overadd{k}{\chi}_{{\frac{9-n}{2}+(n-1)}}
              \\
              \phantom{\overadd{k}{\chi}_{,kkk}} \, \vdots        &       & \vdots          & \vdots                                      &                             & \vdots
              \\
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &       & 0        & \hspace{1cm} \fbox{$\overadd{1}{\chi}_{(n-1)+4} $}       & \ldots\quad\dots\quad\dots\quad \ldots\quad\dots\quad \ldots  & \overadd{k}{\chi}_{(n-1)+4}
              \\
            \hline
            \end{array}
        \\
            \begin{array}{cccccc}
                 & \phantom{\overadd{k}{\chi}_{,k}\qquad\qquad}    &  \phantom{\overadd{k}{\chi}_{}\qquad\qquad\qquad}    & \quad \vdots &   &
            \end{array}
        \\
            \begin{array}{|ccccccc|}
            \hline
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &   \hspace{2cm}     & 0        & \ldots \quad\ldots \quad\ldots \quad \dots \quad \dots & 0        &\hspace{0.3cm}  \overadd{k}{\psi}_{(k-1)(n-1)+5} \quad  & \overadd{k}{\chi}_{(k-1)(n-1)+5}
              \\
             \phantom{\overadd{k}{\chi}_{,kkk}} \, \vdots      &       & \vdots        & \ddots \quad\ddots \quad\ddots \quad \ddots \quad \ddots & \vdots        &\, \vdots \quad  & \vdots
              \\
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &       & 0        & \ldots \quad\ldots \quad\ldots \quad \dots \quad \dots & 0 &\hspace{0.3cm} \fbox{$\overadd{k}{\psi}_{\frac{7-n}{2}+k(n-1)} $}\quad  & \overadd{k}{\chi}_{\frac{7-n}{2}+k(n-1)} 
              \\
            \hline
            \end{array}
        \\ \vspace{-.4cm}
        \\
            \begin{array}{|ccccccc|}
            \hline
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &   \hspace{2cm}     & 0        & \ldots \quad\ldots \quad\ldots \quad \dots \quad \dots & 0        &\hspace{1.4cm}  0 \quad  & \hspace{1.2cm} \overadd{k}{\chi}_{\frac{9-n}{2}+k(n-1)}
              \\
             \phantom{\overadd{k}{\chi}_{,kkk}} \, \vdots      &       & \vdots        & \ddots \quad\ddots \quad\ddots \quad \ddots \quad \ddots & \vdots        &\hspace{1.4cm} \vdots \quad  & \hspace{1.2cm} \vdots
              \\
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &       & 0        & \ldots \quad\ldots \quad\ldots \quad \dots \quad \dots & 0 &\hspace{1.5cm}  0 \quad  & \hspace{1.2cm} \fbox{$\overadd{k}{\chi}_{k(n-1)+4}$}
              \\
            \hline
            \end{array}
            \end{array}
     \right)\,.
 \end{align}
 It can be readily verified that $\Lambda_k^\dagger$ has trivial kernel, which is still true after removing a finite number of columns.

 Before proceeding, let us denote $ X_1 := (\im \hLop)^\perp$
 and $X_2 := (\im \Lop)^\perp$.
 %Recall that
 %  when $m=0$, $\overadd{\frac{n-3}{2}}{q}{}_{AB}^{[X_1\cap \ker(\overadd{\frac{n-3}{2}}{\psi}(P))\cap \TTtp]}$ 
 % and 
 % $\overadd{\frac{n-1+j}{2}}{q}{}_{AB}^{[X_2\cap \TTtp]}\,, \ j\geq 0$,
 % were gauge-invariant obstructions to gluing (cp. \eqref{5IX23.w3} and \eqref{26VI.1}).
 % In addition (for any $m$), 
 The integrated transport equation for the fields 
 %
 $$\overadd{\frac{n-3}{2}}{q}{}_{AB}^{[X_1^\perp \cap   \ker \overadd{\frac{n-3}{2}}{\psi}(P)   \cap \TTtp]} 
 \quad \text{and} \quad 
 \overadd{\frac{n-1+j}{2}}{q}{}_{AB}^{[X_2^\perp \cap \TTtp]}\,, \ j\geq 0 \,,$$
 %
 will be solved using gauge fields at the end of this section. At the moment, we consider only the projections 
 %
 $$\overadd{\frac{n-3}{2}}{q}{}^{[ X_1\cup (\ker(\overadd{\frac{n-3}{2}}{\psi}(P))^\perp\cap\TTtp]}_{AB}
 \quad \text{and} \quad 
 \overadd{\frac{n-1+j}{2}}{q}{}^{[X_2\cap\TTtp]}_{AB} \,.$$ 
 %
 We show in Appendix \ref{ss4IX23.2} that the spaces $X_1 \cap \ker(\overadd{\frac{n-3}{2}}{\psi}(P))\cap\TTtp$ and $X_2\cap\TTtp$ are smooth and finite dimensional. It follows that there exists $N_1(k)$ 
 such that these spaces $\subseteq \text{span} \{\phi_{\ell}, \ell<N_1(k)\}$.
 % for all $\ell\geq N_1(k)$, $\phi_\ell^{[X_1\cap \ker(\overadd{\frac{n-3}{2}}{\psi}(P))\cap\TTtp]}=0=\phi_\ell^{[X_2\cap\TTtp]}$

 For any $\ell < N_1(k)$, 
 if $\phi_\ell^{[X_1\cap\TTtp]}=0$ and $\phi_{\ell}\in \ker\overadd{\frac{n-3}{2}}{\psi}$ 
 %(hence $\overadd{\frac{n-3}{2}}{q}_{AB,\ell}$ is already continuous by gauge) 
 we remove the row associated with $\overadd{\frac{n-3}{2}}{q}_{AB}$ from the system \eqref{4IX23.5} and solve it; 
 %\wc{note that we have to remove these rows because it not then it complicates the gauge equation}
 if $\phi_\ell^{[X_2\cap\TTtp]}=0$ we remove the rows associated with $\overadd{\frac{n-1}{2}+j}{q}_{AB}\,, \ j\geq 1$, from the system \eqref{4IX23.5} and solve it; finally in all other cases, we solve the full system \eqref{4IX23.5}. Note that in all cases, the system involved is solvable by Lemma \ref{L4IX23.1}. Up to this point thus, the system \eqref{4IX23.5} has been solved for all $\ell< N_1(k)$.
 
 Moving on to the case $\ell \geq N_1(k)$, we need only to consider the system
 %
 \begin{align}
    \underbrace{ \begin{pmatrix}
         \overadd{1}{r}_{AB}\\
         \vdots \\
         \overadd{\frac{n-5}{2}}{r}_{AB}\\
         \overadd{1}{S}_{AB} \\
         \vdots \\
         \overadd{k}{S}_{AB}
     \end{pmatrix}}_{=: \hat t_k}
     =
     \underbrace{\begin{pmatrix}
    \overadd{1}{\psi}_{\frac{9-n}{2}} &         &                \ldots             &        & & \overadd{1}{\psi}_{4+k} 
    \\
                                      & \ddots  &                                   &        & & 
    \\
    \vdots                            &         &\overadd{\frac{n-5}{2}}{\psi_{1}}  &        & & \vdots
    \\
                                      &         &                   & \overadd{1}{\chi}_{4}  & &
    \\
                                      &         &                   &                  & \ddots &
    \\
    \overadd{k}{\chi}_{\frac{9-n}{2}} & & \ldots & & & \overadd{k}{\chi}_{4+k}
     \end{pmatrix}}_{=:\hat \Lambda_k}
     \underbrace{\begin{pmatrix}
         \kphi{\frac{9-n}{2}}\\
         \vdots\\
         \kphi{1} \\
         \kphi{4}\\
         \vdots\\
         \kphi{4+k}
     \end{pmatrix}}_{=:\hat\upsilon_k}
     +
     \mathcal{N}_k  \rho_k\,,
     \label{4IX23.6}
 \end{align}
 %
 where
 %
 \begin{align}
     \mathcal{N}_k := 
     \begin{pmatrix}
         \overadd{1}{\psi}_{5+k} & \ldots &\overadd{1}{\psi}_{4+k(n-1)} \\
         \vdots & \ddots & \vdots \\
        \overadd{\frac{n-5}{2}}{\psi}_{5+k} & \ldots &\overadd{\frac{n-5}{2}}{\psi}_{4+k(n-1)} \\
        \overadd{1}{\chi}_{5+k} & \ldots &\overadd{1}{\chi}_{4+k(n-1)} \\
         \vdots & \ddots & \vdots \\
        \overadd{\frac{n-5}{2}}{\chi}_{5+k} & \ldots &\overadd{\frac{n-5}{2}}{\chi}_{4+k(n-1)} 
     \end{pmatrix}
     \,,\quad 
     \rho_k := 
     \begin{pmatrix}
         \kphi{5+k}\\
         \vdots \\
         \kphi{4+k(n-1)}
     \end{pmatrix}\,.
 \end{align}
 %
 We note that the system \eqref{4IX23.6} is just a subsystem of \eqref{4IX23.1}. (The other part of the system, namely those involving $\overadd{\frac{n-3}2+j}{q}_{AB}\,, j \geq 0$ has already been fully taken-cared of by the $\ell< N_1(k)$ consideration together with the gauge fields in \eqref{14VI.3} and \eqref{14VI.2}). Therefore we can use the same mode decomposition for it as \eqref{4IX23.7}. In addition, as written in \eqref{4IX23.6}, we can make use of the item (ii)'s of Section \peqref{e3IX23.1} and Section \peqref{e3IX23.2} to conclude that the operator $\hat\Lambda_k$ is elliptic in the sense of Agmon, Douglis and Nirenburg.
 By the same argument as that above \eqref{29VII23.11}, there exists $N_2(k)$ such that we can find a unique solution of the $\ell$-th mode of \eqref{4IX23.6} with  $\rho_{k,\ell}=0$ for all $\ell \geq N_2(k)$. 
 
 Now, for all $\ell < N_1(k)$, we use the same solution for the $\ell$-th mode of the subsystem \eqref{4IX23.6} as that obtained above for the full system \eqref{4IX23.7}. If $N_2<N_1$, then for any $\ell \geq N_1 > N_2$, it follows from the previous paragraph that we can solve the $\ell$-th mode of \eqref{4IX23.6}, setting $\rho_{k,\ell}=0$. Next, if $N_2 \geq N_1$, 
 it remains to show that  \eqref{4IX23.6} can be solved in the finite dimensional space of $\hat\upsilon_k$'s and $\rho_k$'s of the form
 %
 \begin{equation}\label{4IX23.11}
   \hat\upsilon_k= \sum_{\ell = N_1(k) }^{N_2(k)} \hat\upsilon_{k,\ell} \phi_\ell
   \,, \quad
   \rho_k= \sum_{\ell = N_1(k) }^{N_2(k)}  \rho_{k,\ell} \phi_\ell
   \,, \quad
  \hat t_k = \sum_{\ell = N_1(k) }^{N_2(k)}  \hat t_{k,\ell} \phi_\ell
   \,.
 \end{equation}
 %
However, that such a solution exists follows directly from Lemma \ref{L4IX23.1}.
\wcb{stopping here; to do: $\TTt$ case}

==> K2hS.tex <==
 In addition, \eqref{29VIII23.f3} and \eqref{29VIII23.f4} and \eqref{17X23f.1} show inductively that the operator $\ck{-2}{\ofPnoP}$ does not appear in the transport equation of $\overadd{p}{q}{}_{AB}^{S}$.
  Indeed, the first occurrence of the operator $\ck{-2}{\ofPnoP}$ in the transport equation \eqref{6III23.w6c} happens at $i=\frac{n-1}{2}$ in the expression
 %
 $$\overadd{\frac{n-1}{2}}{\psi}\ofP = \ck{-2}{\ofPnoP} \ck{-1}{\ofPnoP}\overadd{\frac{n-5}{2}}{\psi}\ofP \,,$$
 %
 which evaluates to zero when acting on $h^{\red[S]}$ by  \eqref{29VIII23.f3} and \eqref{29VIII23.f4}. That $\ck{-2}{\ofPnoP}$ does not occur further down the recurrence follows readily by induction (see \eqref{17X23f.1}). 

==> Kerr_deSitter.tex <==
\section{Kerr--(Anti-)deSitter black holes in higher dimensions}\label{Kerr-dS appendix}

In this appendix we wish to show that some families of solutions have enough parameters
to compensate for the obstructions for gluing. This comprises:
\input{Family}

We start with the Kerr-(A)dS metrics


\subsection{The Kerr-(A)dS metrics}

The full Kerr-(A)dS metric in $(n+1)$-spacetime dimensions, $\Lambda \in \R$, is given by
\cite{Gibbons:2004js}:%
\footnote{To facilitate the comparison with that reference we  note that $a_i$ is the negative of the one there, and recall that $a_{N+\delta}=0$ for $\delta=1$.}
%
\begin{align}\label{eq: Kerr AdS}
ds^2=&-W(1-\alpha^2r^2)dt^2+\frac{2m}{U}\Bigl(Wdt+\sum_{i=1}^\red{N} \frac{a_i \mu_i^2 d\phi_i}{\Xi_i}\Bigr)^2\nonumber\\
&+\sum_{i=1}^\red{N}\frac{r^2+a_i^2}{\Xi_i}\bigl(\mu_i^2d \phi_i^2+d\mu_i^2)
+\frac{Udr^2}{V-2m}+\delta r^2 d\mu_{\red{N}+\delta}^2\nonumber\\
&+\frac{\alpha^2}{W(1-\alpha^2r^2)}\Bigl(\sum_{i=1}^\red{N} \frac{r^2+a_i^2}{\Xi_i}\mu_i d\mu_i+\delta r^2 \mu_{\red{N}+\delta} d\mu_{\red{N}+\delta}\Bigr)^2\,,
\end{align}
%
where
%
\begin{align}
W&=\sum_{i=1}^{\red{N}} \frac{\mu_i^2}{\Xi_i}+\delta \mu_{\red{N}+\delta}^2\,,
\quad
V=r^{\delta-2}(1-\alpha^2r^2)\prod_{i=1}^\red{N}(r^2+a_i^2)\,,\nonumber\\
U&%=\frac{V}{1-\alpha^2r^2}\Bigl(1-\sum_{i=1}^\red{N}\frac{a_i^2\mu_i^2}{r^2+a_i^2}\Bigr)
=r^\delta\left( \sum_{i=1}^{N+\delta}\frac{\mu_i^2}{r^2+a_i^2}\right)\prod_{i=1}^\red{N}(r^2+a_i^2)\,,
\quad 
\Xi_i=1+\alpha^2 a_i^2
\,.
\end{align}
Here, $\delta=1, 0$ for even, odd spacetime dimensions, $N=\bigl[\frac{n}{2}\bigr]$ (where $[A]$ denotes the integer part of $A$) so that $d=n+1=2N+\delta+1$, and the coordinates $\mu_i$ obey a constraint
\begin{equation}\label{3VI24.f1}
\sum_{i=1}^{N+\delta} \mu_i^2=1\,.
\end{equation}
In these coordinates there is no rotation at spatial infinity and the angles $\phi_i$ are periodic with period $2\pi$.


==> LambdaKnew.tex <==
\section{The matrices $\Lambda^{[X]}_k$}
\subsection{Ellipticity}
\label{ss24IX23.2}
 \ptcheck{28IX23, read the whole section without checking the calculations; and then the calculations as well later}

\input{LambdakTable}


In this appendix we show that for each $X\in\{S,V\}$, the matrix of operators $\Lambda^{[X]}_k$ of \eqref{4IX23.1} is elliptic in the sense of Agmon, Douglis and Nirenberg. 

{\wblueca{9IV24}
First, we recall the definition of ellipticity in the sense of Agmon, Douglis and Nirenberg (ADN). Consider a differential system on $\secN$ of the form
%
\begin{align}
    \Lambda(\zspaceD) v(x) = u(x)
    \label{9IV24.1}
\end{align}
%
where $v(x)$ and $u(x)$ are $N$-vector valued functions on $\secN$ and $\Lambda$ is a $N\times N$ matrix of linear partial differential operators, with each $(\Lambda(\zspaceD))^i{}_j$ being a polynomial in $\zspaceD_A$. Here and below, the notation $(A\red{)^i{}_j}$ denotes the $ij$-entry of a matrix $A$. The system \eqref{9IV24.1} is said to be \textit{elliptic}, if there exists integers $s_i, t_j$ with $i,j \in [1,N]$, such that the order of the operator $(\Lambda)^i{}_j$ does not exceed $s_i+t_j$ and furthermore
%
\begin{align}
    \det \Lambda^0(k) \neq 0 \ \text{for all} \ k \neq 0 \ \text{vectors}\,.
    \label{9IV24.2}
\end{align}
%
In \eqref{9IV24.2}, $\Lambda^0$ denotes the matrix obtained from $\Lambda$ by keeping only those operators of order exactly $s_i+t_j$ in each $(\Lambda)^i{}_j$ entry.
}

\index{ellipticity!Lambda@$\Lambda^{[X]}_k$|(}%
\index{Lambda@$\Lambda_k$!ellipticity|(}%
To show that the matrix of operators $\Lambda^{[X]}_k$ of \eqref{4IX23.1} is elliptic in the sense of ADN, we choose $s_i \,, t_j$ as (see also Figure~\ref{f10IX23.1} and \ref{f10IX23.2})
 %
 \begin{align}
     s &=
     \begin{cases}
          2 \times (\frac{n-1}{2}\,, 2\,, 3\,, \dots \,, \frac{n-3}{2} \,, 2 \,, 3\,, \dots \,, k+1) \,, & k= \frac{n-3}{2} \,,
          \\
           2 \times (\frac{n+1}{2}\,, \frac{n-1}{2}\,, 2\,, 3\,, \dots \,, \frac{n-3}{2} \,, 2 \,, 3\,, \dots \,, k+1\,,k\,, k-1\,, \dots\,, \frac{n+1}{2}) \,, & k \geq \frac{n-1}{2} \,,
     \end{cases}
     \label{15IX23.2}
     \\
     t & =
     \begin{cases}
          (0 \,, \dots \,, 0 ) \,, & k=\frac{n-3}{2}
          \\
          2 \times (\underbrace{0 \,, \dots \,, 0 }_{2k-k_n \text{ terms}}\,, \underbrace{ -(k_n-1) \,, -(k_n-2) \,, \dots\,, -1, 0 }_{k_n \text{ terms}}) \,, & k \geq \frac{n-1}{2}
           \,,
     \end{cases}
     \label{15IX23.3}
 \end{align}
 %
%
 (recall that $k_n$ has been defined in \eqref{2X23.1}).
 Let $ \Lambda_k^{[0,X]}$ denote the matrix obtained by
  keeping in $(\red{\Lambda_k^{[X]}}\red{)^i{}_j}$
 only those operators which are of order $s_i + t_j$.
We wish to show
that  $ \Lambda_k^{[0,X]}$ is a lower triangular  matrix,
 with the diagonal entries being
 \FGp{14XI}
 %
 \begin{align}
 \begin{cases}
      \big(
     d_2^X \,,
     (\overadd{1}{\tilde\psi}%_{\frac{9-n}{2}}
     \,,
     \overadd{2}{\tilde\psi}%_{\frac{11-n}{2}}
     \,,
 \dots \,,
 \overadd{\frac{n-5}{2}}{\tilde\psi}%_{1}
 \,,
 \overadd{1}{\tilde\chi}%_{4}
 \,,
  \overadd{2}{\tilde\chi}%_{5}
  \,,
 \dots \,
  \overadd{k}{\tilde\chi}%_{4+k}
  )\circ \zdivtwo \circ\, C
 \big)
   \,,
 \\
  \big(
     \zdivtwo\circ  {\Lop} \,,
     d_2^X \,,
     (\overadd{1}{\tilde\psi}%_{\frac{9-n}{2}}
     \,,
     \overadd{2}{\tilde\psi}%_{\frac{11-n}{2}}
     \,,
 \dots \,,
 \overadd{\frac{n-5}{2}}{\tilde\psi}%_{1}
 \,,
 \overadd{1}{\tilde\chi}%_{4}
 \,,
  \overadd{2}{\tilde\chi}%_{5}
  \,,
 \dots \,
  \overadd{k}{\tilde\chi}%_{4+k}
  )\circ \zdivtwo \circ \, C \,,
  % \nonumber
  % \\
  % &\qquad
 \underbrace{\zdivtwo \circ \Lop \,,
 \dots \,,
 \zdivtwo \circ \Lop }_{k_n \text{ terms}}
 \big)  \,,
 \end{cases}
 \label{9IX23.11}
 \end{align}
%
with the first case for $k=\frac{n-3}{2}$ and the second case for $k\geq\frac{n-1}{2}$, and with
\FGp{14XI}
 %
 \begin{equation}
    d_2^X :=
    \begin{cases}
        \zdivtwo\circ  \underline{\hLop}_n \,, & X= S \,,
        \\
        \overadd{\frac{n-3}{2}}{\tilde\psi}\circ \zdivtwo \circ\, C \,, & X=V\,,
    \end{cases}
 \label{9IX23.12}
 \end{equation}
%
where the operators $\overadd{p}{\tilde\psi} = \overadd{p}{\tilde\psi}\ofDC$,  $\overadd{p}{\tilde\chi} = \overadd{p}{\tilde\chi}\ofDC$ and $\underline{\hLop}_n\,, \Lop$ are the gauge operators defined in Section \ref{ss9IX23.1}. We emphasise that the operators appearing in \eqref{9IX23.11} are all elliptic (see  Appendix \ref{App12XI22.1h}).
% We note that the operators appearing in \eqref{9IX23.11} and \eqref{9IX23.12} are of orders
% %
% \begin{align}
%    2\times [\frac{n+1}{2}\,,
%    \frac{n-1}{2} \,,
%     2 \,,
%     3\,,
%     \dots\,,
%     \frac{n-3}{2}\,,
%     2\,,
%     3\,, \dots\,,
%     k+1\,,
%     \frac{n+1}{2} \,,
%     \dots \,,
%     \frac{n+1}{2}
%     ] \,.
% \end{align}
% %

By definition of $u_k$ and $\upsilon_k$, it is clear that the terms in \eqref{9IX23.11} will appear in the respective spots on the diagonal of $ \Lambda_k^{[0,X]}$. Indeed, this follows directly from the transport equations and the gauge transformation of $\overadd{p}{q}_{AB}$ for $p \geq\frac{n-3}{2}$. It remains to show that $ \Lambda_k^{[0,X]}$ is lower-triangular.


First, consider the submatrix $(\Lambda^{[X]}_{k}\red{)^i{}_j}$ with $i,j\in [3, k+\frac{n-1}{2}]$, denoted as $A_1$ in
Figure \ref{f10IX23.1}. For these entries, the analysis is similar to the convenient case -- in each row, the operators involved are either $\overadd{i}{\tilde\psi}_n $ or $\overadd{i}{\tilde\chi}_n$ for some $n\in\{\frac{9-n}{2},4+k\}$. By the same reasoning as items (ii) of Section \pref{e3IX23.1} and Section \pref{e3IX23.2}, the operator of highest order amongst the $\overadd{i}{\tilde\psi}_n $'s, resp. $\overadd{i}{\tilde\chi}_n $'s, is
%
\begin{equation}
    \overadd{i}{\tilde\psi}\ofDC\,, \quad \text{resp.} \quad \overadd{i}{\tilde\chi}\ofDC \,,
    \label{10IX23.9}
\end{equation}
%
which is of order $2i$; all other $\overadd{i}{\tilde\psi}_n $ and $\overadd{i}{\tilde\chi}_n $ operators are of lower order. We note for later use that this is also true for the entries  $(\Lambda^{[X]}_{k}\red{)^i{}_j}$ with $i = 2 \,, j\in [3, k+\frac{n-1}{2}]$  
($A_2$ in Figure~\ref{f10IX23.1}).
The above justifies that $(\Lambda^{[0,X]}_{k}\red{)^i{}_j}$ with $i,j\in [3, k+\frac{n-1}{2}]$ is lower triangular.
\FGp{14XI}

Next, we consider the gauge transformations of the fields $\zspaceD^A\overadd{i}{q}_{AB}$. From \eqref{6III23.w8b}, we have
%
\begin{align}
    \zspaceD^A\overadd{i}{q}_{AB}&= \partial_u \zspaceD^A\overadd{i-1}{q}_{AB}
    - \underbrace{\overadd{i-1}{\tilde\psi}\ofDC
     }_{
     { \text{order $2(i-1)$}}}
       \, \zspaceD^A\qh_{AB}^{(n-5-2i)/2}
    % - \alpha^{2(i-1)} \overadd{i-1}{\psi}_{[\alpha]} \qh_{AB}^{(n-9+2i)/2}
    % \nonumber
    % \\
    % &\quad
    - m^{i-1} \underbrace{\overadd{i-1}{\psi}_{\red{[m]}}}_{
     { \text{order $0$}}
     }
     \zspaceD^A\qh^{(\frac{n-7-2(i-1)(n-1)}{2})}_{AB}
    % - \alpha^2 \mathcal{\tilde K}(2(i-1),P)  \overadd{i-2}{q}_{AB}
    \nonumber
    \\
    &\quad
    - \sum_{j=1}^{p-1}  m^{j}
    % \alpha^{2\ell}
    \underbrace{\overadd{i-1}{\tilde\psi}_{j,0}\ofDC}_{
     { \text{order $2(i-1-j)$}}
     } \, \zspaceD^A\qh^{(\frac{1}{2} (n-7- 2 (i-1) - 2 j (n-2)))}_{AB}
    \, ,
     \quad 1 \leq i \leq k \,.
    \label{10IX23.1}
\end{align}
%
Using \peqref{7III23.w1} and \peqref{23IV23.1} it can be shown inductively
 that for each $1\leq i \leq \frac{n-3}{2}$, in the gauge transformation of $\zspaceD^A\overadd{i}{q}_{AB}$,

\begin{enumerate}
    \item[1.]   the operators acting on the gauge fields $\zspaceD_A \xi{}^u$ and $\xi_A$ are both
     {\text{of order $2(i+1)$}},
         \ptcheck{29IX23 }
         \FGp{14XI}
    \item[2.] %for each $1\leq i \leq k$,
    the order of the operators acting on $\partial^j_u\xi_A$, $1\leq j\leq i-1$, is { $2(i-j-1)$}
%    $\red{\sim P}^{i-(j-1)}$
(relevant for region $B$ in Figure~\ref{f10IX23.1}).
    \ptcheck{29IXVI}
\end{enumerate}
%
To see this, note that the gauge transformation law of $\zspaceD^A\qh^{(n)}_{AB}$, given in \eqref{23IV23.1}, involves only the gauge fields $\zspaceD_A\xi^u$, $\xi_A$ and $\partial_u \xi_A$. The associated operators acting on these fields are of orders four, four and two
%$P^2$, $P^2$ and $P$
respectively. Thus, modulo the first term in \eqref{10IX23.1}, the operators of the highest order in the gauge transformation of $\zspaceD^A\overadd{i}{q}_{AB}$ must come from the second term in \eqref{10IX23.1}, and are given by that acting on $\zspaceD_A\xi^u$ and $\xi_A$. Furthermore, they are of order $2(i+1)$.
%$P^{i+1}$.
Next, the fact that   the operators acting on $\partial^j_u\xi_A$, $1\leq j\leq i-1$, are of order { $2(i-(j-1))$}
%$\red{\sim P}^{i-(j-1)}$
follows easily by induction; we leave the details to the reader, after using  \eqref{7III23.w1} for initialisation.
\seccheck{21XII}
 By a similar analysis for the gauge transformation of the $\overadd{i}{\Hf}_{uA}$ fields,
 using the recursion formula \eqref{6III23.w4}, and \eqref{30IX23.1} and \eqref{28II23.1} for initialisation, we have:
\ptcheck{ 29IX }\FGp{14XI}%
for each $1\leq i \leq k$,  the operators acting on the gauge fields $\zspaceD_A \xi{}^u$ and $\xi_A$ are
     {\text{of order $2(i+1)$}},
%     $\red{\sim P}^{i+1}$
while those acting on $\partial^j_u\xi_A$, $1\leq j\leq i+1$, are of order
     { $2(i-(j-1))$}.
%     $\red{\sim P}^{i-(j-1)}$.
Together with the previous paragraph, we conclude that, for rows $i \in [1, k+\frac{n-1}{2}]$, the conditions for $ \Lambda_k^{[0,X]}$ being lower triangular are satisfied.

For the first row with $k\ge \frac{n-1}2$ we have $(\Lambda^{[X]}_k\red{)^1{}_3}=0$, which follows from \eqref{22VIII23.2c} with $p=\frac{n-1}{2}$.
Next,
we also have $(\Lambda^{[V]}_k\red{)^1{}_2}=0$, while $(\Lambda^{[S]}_k\red{)^1{}_2}$
     { \text{is of order $n-1$}}.
       %$\red{\sim P}^{\frac{n-1}{2}}$.
The first equality follows from the fact that the field $\kphi{2}_{AB}$ does not appear in the integrated transport equation \eqref{9IX23.w1} of $\overadd{\frac{n-1}{2}}{q}_{AB}$. The second statement follows from the following calculation of the gauge term associated to $\zspaceD_A\xi^u$ in the gauge transformation of $\overadd{\frac{n-1}{2}}{q}_{AB}$:
 Namely, using \eqref{23IV23.1},  \eqref{10IX23.1},  and what has been said so far, this term is of the form
%
\begin{align}
    -\frac{2}{(n-2)r}
    &
    \underbrace{ \overadd{\frac{n-3}{2}}{ \psi}\ofP  \circ P \circ\, C(\zspaceD_A\xi^u)}_{=0}
    \nonumber
\\
 &     +
    { \text{an operator of order $(n-1)$ acting on}}
    %(
    %\red{\sim P}^{\frac{n-1}{2}}(
    \ \zspaceD_A\xi^u
    %)
    %)
    \,,
    \label{15IX23.1}
\end{align}
%
 where  the second term comes from the last term on the right-hand side of \eqref{10IX23.1} with $i=\frac{n-3}{2}$ and $j=1$.
The first term vanishes by the fact that
%
\begin{equation}
    \overadd{\frac{n-3}{2}}{ \psi}\ofP h^{\red[S]} = 0 \,,
\end{equation}
%
see \eqref{29VIII23.f3}.
 \ptcheck{3X23}
 \FGp{14XI}

That the operators appearing on columns four to $k+\frac{n-1}{2}$ (region $D$ in Figure~\ref{f10IX23.1}) are all of orders $\leq \frac{n-1}{2}$ follows from the same argument as that around \eqref{10IX23.9} (for regions $A_1$ and $A_2$).
Finally, concerning the first line of region $B$ of Figure~\ref{f10IX23.1},  we note that the part of items 1.\ and 2.\ below \eqref{10IX23.1} concerning $\xi_A$ and its $u$-derivatives continues to hold for the gauge transformation of $\overadd{\frac{n-1}{2}}{q}_{AB}$.
 \ptcheck{4X23}
\FGp{14XI}

Let us turn our attention now to the last $k_n$-lines of Figure~\ref{f10IX23.1}.
The vanishing of the first term in \eqref{15IX23.1} modifies the order of the operators appearing in the gauge transformation of $\overadd{i}{q}_{AB}$, $i \geq \frac{n+1}{2}$ ,
as compared to point 2.\ below \eqref{10IX23.1}. Indeed, restarting the induction from $\overadd{\frac{n-1}{2}}{q}_{AB}$, it follows from \eqref{10IX23.1} (where now the second term at the right-hand side vanishes) that
\begin{enumerate}
    \item[3.]  the operators acting on the gauge fields $\zspaceD_A\xi^u$ and $\xi_A$ are both
     {\text{of order $2i$}};
%     $\red{\sim P}^i$
    \item[4.] that acting on $\partial_u^j \xi_A$ is
     {\text{of order $2(i-j)$}}
%     $\red{\sim P}^{i-j}$
for $1 \leq j \leq i-\frac{n+1}{2}$, and
     {\text{of order $2\big(i-(j-1)\big)$}}
%     $\red{\sim P}^{i-(j-1)}$
for $i-\frac{n-1}{2} \leq j \leq i-1$.
 \ptcheck{4X23}
 \FGp{14XI}
\end{enumerate}

One readily verifies that the choice \eqref{15IX23.2} and \eqref{15IX23.3} results in a lower triangular matrix in the lower right $k_n \times k_n$ block,
(cf.\ block $C$ of
Figure~\ref{f10IX23.1})
 submatrix of $ \Lambda_k^{[0,X]}$. See also Figure~\ref{f10IX23.2}.
 \ptcheck{4X23}

Finally, we come to the second row of $\Lambda^{[X]}_k$, $X\in\{V,S\}$. For the term on the diagonal, it follows directly from the transport equation \eqref{9IX23.w1} with $i= \frac{n-3}{2}$ and the gauge transformation equation \eqref{24IV23.1xs} that this term is
{ of order $ {n-1} $} for $X=S$ and $X=V$ respectively. Meanwhile, it follows from the statement below \eqref{10IX23.9}
with  $i= \frac{n-3}{2}$, together with  that below \eqref{10IX23.1}, that the operators from columns three to $2k$ are all of order lower than or equal to ${n-3}$. Specifically, for the last $k_n$ columns (i.e., in region $B$), the operator associated to the $\partial_u^j\kxi{2}_A$ column is of order $ 2\big(i-(j-1)\big) $
%\xout{$\red{\sim P}^{i-(j-1)}$}}
(cf.\ below \eqref{10IX23.1}, item 2.).
 \ptcheck{4X23}
\FGp{20XI}

We now justify the first and last $k_n$ entries of equation \eqref{9IX23.11}. The analysis in Section \ref{ss9IX23.1} of the main text shows that in the gauge transformation formulae
of $\overadd{\frac{n-1}{2}+j}{r}$ for $j=0,...,k_n$, respectively $\overadd{\frac{n-3}{2}}{r}$, the   operators $\zdivtwo\circ\Lop$ acting on the field $\partial^j_u\kxi{2}$,  resp.  $\zdivtwo \circ \underline{\hLop}_n$ acting on $\zspaceD_A\kxi{2}^u$,
appear on the diagonal  of $\Lambda_k$.
It is not difficult to see that these are
 the only operators of order  $ {n+1} $ acting on $\partial^j_u\kxi{2}$, respectively of order $ {n-1} $ acting on $\zspaceD_A\kxi{2}^u$.
Indeed, a comparison of length-dimensions of the fields $\partial^j_u\kxi{2}$ and $\overadd{\frac{n-1}{2}+j}{r}$, resp. $\zspaceD_A\kxi{2}^u$ and $\overadd{\frac{n-3}{2}}{r}$, shows that
the gauge operators must be dimensionless. Thus each term contributing to these operators must  a)  either be  $r$-independent, in which case we obtain
 $\zdivtwo\circ\underline{\hLop}_n$, of order ${n+1} $, for
 $\overadd{\frac{n-1}{2}+j}{r}$ and $\zdivtwo\circ\hLop_n $, of order ${n-1} $,  for $\overadd{\frac{n-3}{2}}{r}$; or
   b)
   come with the dimensionless combination $m^i\alpha^{2\ell}r^{-i(n-2)+2\ell}$ for some $0\leq i,\ell$, and $i+\ell\geq 1$; the analysis involving $\alpha$ is included for later reference in Appendix \ref{ss18XI23.1}. However, looking at \eqref{5III23.5}-\eqref{5III23.5b} and \eqref{23IV23.1} we see that each factor of $m$ or $\alpha^2$ will decrease the order of the operator by two.
   It ensues that a gauge operator associated with the field $\overadd{\frac{n-1}{2}+j}{r}$, respectively with the field $\overadd{\frac{n-3}{2}}{r}$,  and containing a prefactor $  m^i\alpha^{2\ell} $  is of order ${n+1} -2i-2\ell $, respectively $ {n-1} -2i-2\ell$. This justifies the first and last $k_n$ entries of equation \eqref{9IX23.11}.

It follows that $ \Lambda_k^{[0,X]}$ is lower triangular, with elliptic operators lying on the diagonal.

\subsection{Mode solvability}
 \label{ss30XI23.2}
 In this section, we explain the mode solvability of the system~\eqref{4IX23.1}.
Suppose that all entries of $u_k^{[X]} $, $\upsilon_k^{[X]} $ and $\rho_k^{[X]}$ are eigenvectors of the Laplace operator with the same eigenvalue $-\lambda_\ell\ge 0 $. We then have
%
$$
  \red{\Lambda_k^{[X]}} \upsilon_k^{[X]} = B_{k,\ell}^{[X]} \upsilon_k^{[X]}
  \,,
  \qquad
  \mathcal{N}^{[X]} _k \, \rho_k ^{[X]} = D_{k,\ell}^{[X]} \rho_k^{[X]}
  \,,
$$
%
with  real-valued matrices $B_{k,\ell}^{[X]}$ and $D_{k,\ell}^{[X]}$. The $(ij)$ entries $(B_{k,\ell}^{[X]})^i{}_j$ of the matrix $B_{k,\ell}^{[X]}$ are polynomials in $\lambda_\ell$ of  order lower than or 
equal to 
$(s_i+t_j)/2$ (recall that all $s_i$'s and $t_j$'s are even), or vanish. The system
%
\begin{align}
    u_k^{[X]} = \Lambda _k^{[X]} \upsilon_k^{[X]} + \mathcal{N} _k^{[X]}  \rho_k^{[X]}
    \label{30XI23.1-}
\end{align}
%
becomes
%
\begin{align}
    u_k^{[X]} = B_{k,\ell}^{[X]} \upsilon_k^{[X]} + D_{k,\ell}^{[X]} \rho_k^{[X]}
     \,.
    \label{30XI23.1}
\end{align}
%
For $\lambda _\ell  \ne 0$ define  the (invertible) diagonal matrices $A_{\ell} $ and $C_{\ell} $ as
%
$$
   A_{\ell}  = \mbox{\rm diag} (\lambda_\ell ^{-s_i/2}  )
  \,,
  \quad
   C_{\ell}  = \mbox{\rm diag} (\lambda_\ell ^{-t_i/2}  )
   \,.
$$
% 
The equation \eqref{30XI23.1} can be rewritten as
%
\begin{align}
     \check u^{[X]}:= A_\ell  u_k^{[X]} = 
     \underbrace{A_{\ell}  B_{k,\ell}^{[X]} C_\ell
     }_{=:\check B^{[X]}}
     \underbrace{  C_\ell ^{-1}  \upsilon_k^{[X]}
      }_{=: \check \upsilon^{[X]}} +
%     \underbrace{ A_\ell   D_{k,\ell}  \rho_k}_{=:\check \rho}
 A_{\ell}    D_{k,\ell}^{[X]}  \rho_k^{[X]}
     \,.
    \label{30XI23.3}
\end{align}
%
The $(ij)$ entry of the matrix $ A_{\ell}  B_{k,\ell}^{[X]} C_{\ell} $ equals
%
$$
  (A_{\ell}  B_{k,\ell}^{[X]} C_{\ell} )^i{}_j = \lambda_{\ell}^{-s_i/2} (B_{k,\ell}^{[X]})^i{}_j \lambda_{\ell}^{-t_j/2}
   \,.
$$
%
Since  $|\lambda_{\ell}|\to_{\ell\to\infty}\infty$, from what has been said the matrix
$ A_\ell B_{k,\ell}^{[X]} C_\ell$ tends to a lower-triangular matrix with non-zero entries at the diagonal when $\ell$ tends to infinity. It follows that there exists $N$ so that,  for any given $\check u^{[X]} $ and $\rho_k^{[X]} $, the system \eqref{30XI23.3}
%
\begin{align}
     \check u^{[X]} = \check B^{[X]}  \check \upsilon^{[X]} +  A_\ell ^{[X]}  D_{k,\ell}^{[X]}  \rho_k^{[X]}
    \label{30XI23.4}
\end{align}
%
has a solution $\check \upsilon^{[X]}$ for  all $\ell\ge N$:
%
\begin{align}
      \check \upsilon^{[X]}  = (\check B^{[X]})^{-1} (\check u^{[X]} -  A_{\ell}    D_{k,\ell} ^{[X]} \rho_k^{[X]})
      \,.
    \label{30XI23.4b}
\end{align}
%
 Setting
%
\begin{align}
     u_k^{[X]} =  (A_{\ell} )^{-1} \check u^{[X]}
     \,,
     \quad  \upsilon_k^{[X]} = C_{\ell}   \check \upsilon^{[X]}
     \,,
    \label{30XI23.3b}
\end{align}
%
one obtains a solution of the original system \eqref{30IX23.1}.



\input{ADN}

\index{ellipticity!Lambda@$\Lambda^{[X]}_k$|)}%
\index{Lambda@$\Lambda_k$!ellipticity|)}% 

==> LandHatL.tex <==
\subsection{\protect$\hLop$ and \protect$\Lop$}
 \label{ss12XI22.11}

To continue, we wish to analyse the operator \eqref{26II23.1}, namely
%
\begin{align}
    \hLop = C \underbrace{
     \bigg(\frac{2}{\ddim} \zspaceD \zdivone - \frac{4}{\ddim+2} \zdivtwo C + \frac{\ddim}{2} (\twoscsign - r^2 \alpha^2) \bigg) 
     }_{=:L}\,.
    \label{26II23.2}
\end{align}
%
thus 
 \ptcr{are these the relevant operators? stopping here? keep the sign?
 \\--\\
 wan: operator replaced by \eqref{30VI.1}}
%
\begin{equation}\label{24X22.11a}
 \hLop  =    C \Lop
 \,.
\end{equation}
%
recall that $\zdivone  \xi  = \zspaceD_A \xi^A$, $(\zdivtwo  h)_A = \zspaceD^B h_{AB}$,  and that $\twoscsign\in \{0,\pm 1\}$ is the sign of the scalar curvature of the Einstein metric $\zgamma$. 

We consider  first  the operator $\xi \mapsto \zdivtwo C(\xi)$. One finds
 \ptcr{this is probably in dim 2, and so is probably everything that follows}
%
\begin{equation}\label{30X22.32}
   \big(\zdivtwo C(\xi)\big)_A = \frac 12 (\dDelta  + \twoscsign) \xi_A
   \,,
\end{equation}
%
which is elliptic, self-adjoint,
with kernel and cokernel spanned by conformal Killing vectors.


Next, we turn our attention to   $\Lop$:
%
\begin{eqnarray}
 \Lop (\xi)_A
  &  = &
  \blue{\zspaceD_A \zspaceD^C \xi_C}+\frac 12
   \big(
     \underbrace{
     \zspaceD_A \zspaceD^C \xi_C
     -
     \zspaceD^C ( \zspaceD_A \xi_C
     }_{-\mathring R^C{}_A \xi_C}
    + \zspaceD_C \xi_A
    )
    \big)
     +\twoscsign\xi_A
      \nonumber
\\
  &  = &
 \zspaceD_A \zspaceD^C \xi_C  +
  \frac 12
   \big(
     -
     \zDelta
     +\twoscsign
    \big)\xi_A
     \label{30X22.31}
\end{eqnarray}
%
%, which can be rewritten as
%%
%\begin{equation}\label{30X22.33}
%%
% \Lop (\xi)_A
%     \equiv
%  {\zspaceD_A \zspaceD^C \xi_C} +
%  \frac 12
%   \big(
%     -
%     \zDelta
%     +\twoscsign
%    \big)\xi_A
%    = 0
%  \,.
%\end{equation}
%%
One readily checks that $\Lop$ is also elliptic and self-adjoint.


Applying $\dnabla^A$ to \eqref{30X22.31}, commuting derivatives, and using
%
\begin{equation}\label{30X22.CKV2c}
  \dR_{AB} = \twoscsign \dmetric _{AB}
%  \,.
\end{equation}
%
one finds that the kernel of $\Lop$ consists of vector fields satisfying
 \ptcheck{28XI:
 wan : checked for all $\myGauss$}
%
\begin{equation}\label{30X22}
 \frac 12  \dDelta \dnabla_A \xi^A = 0
  \,,
\end{equation}
%
hence $\dnabla_A \xi^A = c$ for some constant $c$. Integrating this last equality over $\dmanif$ shows that $c=0$.
It now follows that the kernel  of  $\hLop$ consists of vector fields satisfying
\ptcheck{1XI  by wan}
%
\begin{equation}\label{30X22.35}
  \big(
     -
     \zDelta
     +\twoscsign
    \big)\xi_A
    = 0
    \,,
    \qquad
    \dnabla_A \xi^A = 0
    \,.
\end{equation}
%
Recall the Hodge decomposition: on a compact two dimensional oriented manifold every one-form can be decomposed as
%
\begin{equation}\label{27XI22.31}
  \xi_A = \zspaceD_A \psi  +\epsilon_{AB} \zspaceD^B \phi + r_A
  \,,
\end{equation}
%
where $r_A$ is a harmonic one-form, i.e.\ a covector field satisfying
%
\begin{equation}\label{27XI22.32}
  \zspaceD^A r_A =0 =   \epsilon^{AB}\zspaceD_A r_B =  (
     -
     \zDelta
     +\twoscsign
    )r_A
  \,.
\end{equation}
%
On $S^2$ the forms $r_A$ vanish  identically, and   on manifolds with genus $\genus$ the space of  $r_A$'s is  $2\genus$-dimensional; cf., e.g., \cite[Theorems~19.11 and 19.14]{ForsterRiemann} or \cite[Theorem~18.7]{ArminRiemann}.
 \ptchd{refs added, both in the papers folder; see also \url{https://arxiv.org/pdf/0802.3174.pdf}, both here and in higher dim,}

From the second equation in \eqref{30X22.35} together with \eqref{27XI22.31}-\eqref{27XI22.32}
 we find that the Laplacian of $\psi$ vanishes, hence $\psi$ is constant, and  the first equation in \eqref{30X22.35} gives
  \ptcheck{again with $r_A$ on 1XII}
%
\begin{equation}\label{30X22.356}
  \epsilon ^{AB} \dnabla_B
     \zDelta \phi
    = 0
    \,.
\end{equation}
%
It readily follows that $\phi$ is also constant, hence $\xi_A=r_A$, and we conclude that:

\begin{Lemma}
   \label{L30X22.1b}
   The operator $\Lop$ is elliptic, self-adjoint, with kernel and cokernel consisting of one-forms $r_A$ satisfying \eqref{27XI22.32}, hence of dimension equal to twice the genus of the compact, oriented, two-dimensional manifold.
\end{Lemma}

We are ready now to pass to the proof of:

\begin{Proposition}
   \label{P30X22.1a}
   The operator  $\hLop$ is elliptic, self-adjoint, with
   %
   {\rm
   $$
    \ker\hLop = \coker \hLop=\CKV +\harm
    \,.
   $$
   %
   }In particular:
   \begin{enumerate}
     \item on $S^2$ and on $T^2$ we have $\ker\hLop = \coker \hLop=\CKV$;
     \item on two-dimensional compact orientable manifolds of genus $\genus\ge 2$ both the kernel and cokernel of $\hLop$ are spanned by the $2\genus$-dimensional space of harmonic 1-forms.
   \end{enumerate}
\end{Proposition}

\proof
%
We first check that $\Lop$ and $-\zdivtwo C$ commute. In view of \eqref{30X22.32}-\eqref{30X22.31} it suffices to check the identity
%
\begin{equation}
 (\dDelta  + \twoscsign) \zspaceD_A \zspaceD^C \xi_C
=
  \zspaceD_A \zspaceD^C  (\dDelta  + \twoscsign)\xi_C
   \,,
\end{equation}
%
which follows from a straightforward commutation of derivatives. %\wcb{workings commented out here.}
% %
% \begin{align}
%     \dDelta  \zspaceD_A \zspaceD^C \xi_C  = \zspaceD^B\zspaceD_B \zspaceD_A \zspaceD^C \xi_C
%     &=
%     \zspaceD^B\zspaceD_A \zspaceD_B \zspaceD^C \xi_C
%     \nonumber
% \\
%     &=
%     \zspaceD_A \zspaceD^B\zspaceD_B \zspaceD^C \xi_C
%     \underbrace{- R^D{}_B{}^B{}_A \zspaceD_D\zspaceD^C\xi_C}_{\twoscsign \zspaceD_A \zspaceD^C\xi_C}
%     \nonumber
% \\
%     &=
%     \zspaceD_A \zspaceD^B(\zspaceD^C \zspaceD_B \xi_C - \underbrace{R^A{}_{CB}{}^C\xi_A}_{\twoscsign \xi_B}) + \twoscsign \zspaceD_A \zspaceD^C\xi^C
%     \nonumber
% \\
%     &=
%     \zspaceD_A \zspaceD^C \dDelta \xi_C - \underbrace{\zspaceD_A R^D{}_B{}^{BC} \zspaceD_D \xi_C}_{-\twoscsign \zspaceD_A \zspaceD^C\xi_C} - \underbrace{\zspaceD_A R^D{}_C{}^{BC}\zspaceD_B\xi_D}_{\twoscsign \zspaceD_A \zspaceD^C\xi_C}
%     \nonumber
% \\
%     &=
%     \zspaceD_A \zspaceD^C \dDelta \xi_C \,.
% \end{align}
% %
This shows that
$\hLop$ is the composition of two  commuting self-adjoint elliptic operators, hence elliptic and self-adjoint.

On $S^2$ the operator $\Lop$ is an isomorphism by Lemma~\ref{L30X22.1b}, hence the cokernel of $\hLop$ is determined by that of $-\zdivtwo C$. The claim on the kernel follows by duality.

It should be clear that in manifestly flat coordinates on  $\T^2$   the kernels of both $\Lop$ and $-\zdivtwo C$ consist  of covectors $\xi_A$ with constant entries, which span the space of conformal Killing vectors on $\T^2$. Self-adjointness implies the result for the cokernel.

In the higher genus case the operator $-\zdivtwo C$ is an isomorphism, so that the kernel of $\hLop$ coincides with the kernel of $\Lop$, as given by Lemma~\ref{L30X22.1b}. One concludes as before.
%
\qed
%









==> Lnwrong.tex <==
\subsection{$L_n$}
 \label{ss10XI23.1}
\index{Ln@$\underline{\Lop}$}%
 \ptcr{started 10XI; in progress; please ignore for the moment}

 \ptcr{it follows from Proposition~\ref{P16X23.2} that $\Lopdagger$ is semi-Fredholm??}
 Recall that (cf.~Remark~\pref{R16X23.1}})
\index{Ln@$\underline{\Lop}$}%
\index{Ln@$\Lop$}%
%
\begin{align}
    \Lop
    &= \overadd{\frac{n-5}{2}}{\psi}\ofP \, \underline{\Lop}
\\
     \underline{\Lop}(\xi)_{AB} &=
     \begin{cases}
        \frac{1}{8} (\TSzlap +2 \tric-4 \myGauss ) (\TSzlap +2 \tric-6 \myGauss )  C(\xi)_{AB}
        &
        \\
        \qquad\qquad\qquad
        - \frac{1}{6}  (\TSzlap + 2 \tric - 5 \myGauss ) \TS[\zspaceD_A\zspaceD_B\zspaceD_C\xi^C] \,, & n=5\,,
        \\
        \frac{1}{(n-1)(n-5)}
     \bigg( (\TSzlap  +2 \tric -2 (n-2) \myGauss) (\TSzlap +2 \tric +(1-n) \myGauss)
     C(\xi)_{AB} &
     \\
     \qquad\qquad\qquad
     -\frac{2 (n-3)}{n-2} (\TSzlap +2 \tric +(5-2 n) \myGauss )
     \TS[\zspaceD_A\zspaceD_B\zspaceD_C\xi^C]
     \bigg) \,, & n\neq 5\,.
     \end{cases}
     \label{30VI.1Ln}
\end{align}
%
In the proof of Proposition~\ref{P16X23.1}
 \ptc{ add "below" or move the section down}
 we show that the operators
 %
$$
\mbox{$\zdivone\circ\zdivtwo\circ \Lop \circ \zspaceD$,
$\zdivone\circ\zdivtwo\circ P\circ \underline{\Lop} \circ \zspaceD$,
and
$\zdivone\circ\zdivtwo\circ P\circ C \circ \zspaceD$}
$$
%
are   elliptic.
The following observation turns out to be useful:

\begin{Lemma}
 \label{L10xi23.1}
Let $k\ge 0$ and let $A$ and $B$ be   linear partial differential operators of order $a$ and $b$ such that $A\circ B$ is elliptic.
%If {\rm $\im B \subset (\ker A)^\perp$,}
Then

\begin{enumerate}
  \item $\ker B$ is finite dimensional with $\ker B\subset C^\infty$, and
  \item
{\rm
%
$\im \big(
  B|_{\MMHkab}
  \big)
  \label{10XI23.4}$
%
}%
%
is closed in $\MMHka$.
\end{enumerate}
%
\end{Lemma}

\proof
%
1. $\ker B\subset \ker A\circ B$, and the result follows form ellipticity.

2.
Let $\psi\in\overline{\im B|_{\MHkab}}$, thus there exists a sequence $\psi_n\in\im B|_{\MHkab}$  converging to $\psi$ in $\MHka$. By definition there exists  $\phi_n\in \MHkab$ such that $\psi_n = B \phi_n$. 
{\redca{13XI}
Since $\ker A\circ B$ is finite dimensional we have the $L^2$-orthogonal decomposition
%
$$
 \MHkab = \ker (  A\circ B) \oplus \Big( \big(\ker  (A\circ B)\big)^\perp \cap \MHkab\Big)
 \,.
$$
%. 
Indeed, let $\phi_i$, with $i=1,\cdots N$ for some $N$, be a basis of $\ker  ( A\circ B)$, then $\big(\ker  (A\circ B)\big)^\perp$ is the intersection of the zero-sets of the finite number of continuous functionals
%
$$
 \MHkab \ni \psi \mapsto \int  \phi_i B^\dagger \psi
 \,,
$$
%
and is therefore closed. Hence we can 
write $\phi_n = \phi_n^\parallel + \phi_n^\perp$, with 
$\phi_n^\parallel \in \ker  (A\circ B)$ and  $\phi_n^\perp \in \big(\ker  (A\circ B)\big)^\perp$, and it holds that
 %
 \begin{equation}\label{11XI23.1}
   \psi_n = B \phi_n^\perp
   \,.
 \end{equation}
 %
The sequence $\psi_n\in\im B|_{\MHkab}$  is Cauchy in $\MHka$. By continuity and linearity the sequence  $A \psi_n = A B \phi_n^\perp$ is Cauchy in $\MHk$.  
 Since   $\phi_n^\perp \in \big( \ker (A\circ B)\big)^\perp$  we can use \eqref{25X23.2}
  }
  with $L=A\circ B$ to conclude that the sequence
$\phi_n^\perp$ is Cauchy in $\MHkab$,
thus there exists  $\phi =\lim_{n\to\infty} \phi_n^\perp$.
%, and we have
%%
%\begin{equation}\label{10XI23.2}
%  0 =  A \circ B \phi_n - A \psi_n  = A ( B \phi_n -   \psi_n)
%  \,.
%\end{equation}
%%
%Since $B\phi_n $ and $\psi_n\in (\ker A)^\perp$ we conclude that $B\phi_n=\psi_n$.
Continuity of $B:\MHkab\to\MHka$ shows that
%
\begin{equation}\label{10XI23.3}
 \psi:= \lim_{n\to\infty} \psi_n =
   \lim_{n\to\infty} B\phi_n^\perp = B\phi
   \,,
\end{equation}
%
and $\im B$ is a closed subspace of $\MHka$, as desired.
%
\qedskip
%

{\redca{13XI}
\input{MoreSteps}
}
\ptcr{still missing div composed with chi} 

==> Notation.tex <==
\section{Introduction}














\section{Notation}
 \label{s26XI22.1}

 Let $\zgamma=\zgamma_{AB}dx^A dx^B$ be a  metric on a $d$-dimensional, compact, orientable manifold $\secN$, with covariant derivative $\zspaceD$.
 We let $\zdivone$, respectively $\zdivtwo$, denote the divergence operator on vector fields $\xi$, respectively on  two-index  tensor fields $h$:
 %
 \begin{equation}\label{12XI22.1}
   \zdivone \xi := \zspaceD_A \xi^A
   \,,
   \qquad
   (\zdivtwo h)_A := \zspaceD^B h_{BA}
   \,.
 \end{equation}
 %
Given a function $f$ we denote by $f^{[1]}$ the $L^2$-orthogonal projection of $f$ on the constants:
%
\begin{equation}\label{15XI22.1}
  f^{[1]}:= \frac{1}{|\secN|_{\zgamma}} \int_{\secN} f d\mu_{\zgamma}
  \,,
  \quad
  \text{where}\quad {|\secN|_{\zgamma}} = \int_{\secN}   d\mu_{\zgamma}
  \,.
\end{equation}
%
We set
%
\begin{equation}\label{15XI22.2}
  f^{[1^\perp]}:= f -  f^{[1]}
  \,.
\end{equation}
%
We will also use the notation $f^{[=0]}$ for $f^{[1]}$, as motivated by decompositions in eigenfunctions of the Laplacian.   In particular $f^{[1]}$ should not be confused with $f^{[=1]}$, which we use when decomposing a function or a tensor field in spherical harmonics on $S^d$.

 Let $\CKV$,
  respectively $\KV$,
  denote the space of conformal Killing vector fields on $\secN$, respectively Killing vector fields. Thus (cf.\ Appendix~\ref{App30X22}), $\CKV$ is $\frac{(d+1)(d+2)}{2}$-dimensional on $S^d$, consists of covariantly constant vectors on $\T^d$, and is trivial on manifolds of higher genus. Given a vector field $\xi$ on $\secN$ we denote by $(\xi^A)^{[\CKV]}$  the $L^2$-orthogonal projection on the space $\CKV$, with
 %
 $$
  (\xi^A)^{[\CKV^\perp]}
  := \xi^A -  (\xi^A)^{[\CKV]}
 \,,
 $$
 %
 with a similar notation for $(\xi^A)^{[\KV]}$  and $(\xi^A)^{[\KV^\perp]}$.

\wc{not sure if below still needed}
We will denote by $\harm$ the space of harmonic 1-forms:
 %
 \begin{equation}\label{12XI.22h}
   \harm=\{\xi_{A } \, | \,    \zspaceD^A \xi_{A } =0 =  \epsilon^{AB}\zspaceD_A \xi_{B } \}
   \,.
 \end{equation}
 %
 By standard results (cf., e.g., \cite[Theorems~19.11 and 19.14]{ForsterRiemann} or \cite[Theorem~18.7]{ArminRiemann}), the space $\harm$ has dimension $2\genus$ on cross-sections $\secN$ with genus $\genus$, in particular it is trivial on spherical sections. We will denote by $\xi_A^{[\harm]}$ the $L^2$-orthogonal projection of $\xi_A$ on $\harm$, and by $\xi_A^{[\harm^\perp]}$ the projection on the $L^2$-orthogonal to $\harm$.

 Let $\TTt$ denote the space of transverse-traceless symmetric two tensors:
 %
 \begin{equation}\label{12XI.22}
   \TTt=\{h_{AB} \, | \, h_{[AB]}= 0=\zgamma^{CD}h_{CD}= \zspaceD^E h_{EF}\}
   \,.
 \end{equation}
 %
 The space $\TTt$ is infinite dimensional
 {\redca{22IV22; to be justified}
 and closed
 }
 on all compact $d$-dimensional manifolds with $d\equiv n-1>2$.

 Given a tensor field $h=h_{AB}dx^Adx^B$ we denote by $h_{AB}^{[\TTt]}$ the $L^2$-orthogonal projection of $h $ on $\TTt$, and set
 %
 \begin{equation}\label{12XI.23}
   h_{AB}^{[\TTt^\perp]}:= h_{AB} -h_{AB}^{[\TTt]}
   \,.
 \end{equation}
 %


We will often use terminology and notation similar to~\cite{ACR1}. In particular, scalar functions, vector fields, and traceless two-covariant symmetric tensors on  $S^d$ will be decomposed into spherical harmonics, see Appendix~\ref{ss20X22.1} for a summary.
   \ptcr{not necessarily?}
  The notation $t^{[= \ell]}$ will denote the $L^2$-orthogonal projection of a tensor $t$ on the space of $\ell$-spherical harmonics. Then
 %
 \begin{equation}\label{29X22}
   t^{[\le \ell]} = \sum_{i=0}^\ell t^{[=i]}
    \,,
    \qquad
   t^{[> \ell]} = t - t^{[\le \ell]}
   \,,
 \end{equation}
 %
 with obvious similar definition of $ t^{[< \ell]}$, etc.
 
 Given any linear differential operator $\hat D$ acting on any tensor field $T$ on $\secN$, we will write $T^{[\ker \hat D]}$ for the $L^2$-orthogonal projection of $T$ on the kernel of $\hat D$, and $T^{[(\ker \hat D)^\perp]}$ for the projection on  $(\ker \hat D)^\perp$; $T^{[\im \hat D]}$ and $T^{[(\im \hat D)^\perp]}$ are defined similarly. 





==> PandLikes.tex <==
%\subsection{$P$ and polynomials in $P$}
\subsubsection{$S^2$}
%
As already discussed in Section~\ref{ss20X22.1}, it follows from \cite{ACR2,Czimek:2016ydb} that  on $S^2$ we can write  symmetric trace-free $2$-tensors $\varphi_{AB}$ as
%
\begin{equation}
    \varphi_{AB} = \sum_{\ell\geq 2 }\sum_{-\ell\leq m\leq \ell}\varphi^{(\ell m)}_{\psi} \psi^{(\ell m)}_{AB}
        + \varphi^{(\ell m)}_{\phi} \phi^{(\ell m)}_{AB}\,.
\end{equation}
%
It follows from \eqref{18X22.2w} and \eqref{18X22.1w} that
the operator $P$ of \eqref{16V22.1}, namely
%
\begin{equation}\label{16V22.1app}
  P\varphi_{AB}  = TS[\zspaceD_A \zspaceD^C \varphi_{BC}]
  \equiv C (\zspaceD^C \varphi_{CD})_{AB}
  \,,
\end{equation}
%
 acts on $\varphi_{AB}$ as
%
\begin{align}
    P\varphi_{AB} &= \sum_{\ell\geq 2 }\sum_{-\ell\leq m\leq \ell}
    \varphi^{(\ell m)}_{\psi} C(\zspaceD^B\psi^{(\ell m)}_{AB})
        + \varphi^{(\ell m)}_{\phi} C(\zspaceD^B\phi^{(\ell m)}_{AB})
        \nonumber
\\
    &=
    \sum_{\ell\geq 2 }\sum_{-\ell\leq m\leq \ell}
    \sqrt{\frac{1}{2}\ell(\ell+1)-1}\left(\varphi^{(\ell m)}_{\psi} C(E^{(\ell m)})_{AB}
        + \varphi^{(\ell m)}_{\phi} C(H^{(\ell m)}_{AB})\right)
        \nonumber
\\
    &=
    -\sum_{\ell\geq 2 }\sum_{-\ell\leq m\leq \ell}
    \underbrace{\left(\frac{1}{2}\ell(\ell+1)-1\right)}_{>0 \text{ for } \ell\geq 2}\left(\varphi^{(\ell m)}_{\psi}\psi^{(\ell m)}_{AB}
        + \varphi^{(\ell m)}_{\phi} \phi^{(\ell m)}_{AB}\right)\,.
        \label{26X22.w3}
\end{align}
%
In particular the operator $P$ is self-adjoint and has trivial kernel on $S^2$. On the other hand the operator $\zdivtwo(P+2)$, which appears in \eqref{24X22.91} with $p=1$ and $m=0$,
 acts according to
%
\begin{align}
   \zdivtwo 
   &
   (P+2)(\varphi)_B  :=  \zspaceD^A(P+2)\varphi_{AB}
 \nonumber
\\
    &=
    -\sum_{\ell\geq 2 }\sum_{-\ell\leq m\leq \ell}
    \left(\frac{1}{2}\ell(\ell+1)-1-2\right)
    \zspaceD^A\left(\varphi^{(\ell m)}_{\psi}\psi^{(\ell m)}_{AB}
        + \varphi^{(\ell m)}_{\phi} \phi^{(\ell m)}_{AB}\right)
        \nonumber
\\
    &=
    -\sum_{\ell\geq 2 }\sum_{-\ell\leq m\leq \ell}
    \underbrace{
    \left(\frac{1}{2}\ell(\ell+1)-3\right)
    \sqrt{\frac{1}{2}\ell(\ell+1)-1}}_{\substack{
    =0 \text{ for } \ell= 1,2 \\
    >0 \text{ for } \ell> 2
    }
    }
    \left(\varphi^{(\ell m)}_{\psi}E^{(\ell m)}_{B}
        + \varphi^{(\ell m)}_{\phi} H^{(\ell m)}_{B}\right)
         \,.
          \label{30XI22.1}
\end{align}
%
It follows that
the $L^2$-orthogonal
 $\big(\im(\zdivtwo(P+2))\big)^{\perp}$ of
 $\im(\zdivtwo(P+2)) $
 is spanned by conformal Killing vectors together with spherical harmonic vector fields with $\ell = 2$. Subsequently, for any covector field $X_A\in L^2$ the equation
%
\begin{equation}
    \zspaceD^B\left(P+2\right)\varphi_{AB}
     	 -
        \xi_A^{[\leq 2]}
            = X_{A}
\end{equation}
%
admits a unique solution
with a symmetric traceless $2$-tensor $\varphi_{AB}$ and a covector field $\xi_A^{[\leq 2]}$.
\ptcheck{19X22}


For a $\Ctwo$ gluing we need the operator
%
$$
 \zdivtwo( P ^2 + 7 \twoscsign P  +10 \twoscsign)
  \,,
$$
%
as determined from the coefficients of $\hkappa_6$ in the formulae \eqref{3VIII22.2} for $\overset{(2,i)}\chi$.
On $S^2$, a calculation  similar  to that in \eqref{30XI22.1} shows that its kernel consists of spherical harmonic tensors with $\ell=1, 2,3$, which results in a cokernel spanned on spherical harmonic vectors with $\ell=1, 2,3$.


\input{orderkkernel} 

==> RegularityFrom4D.tex <==

\subsection{Regularity}
  \label{ss25IV22.1}
\wcb{from 4D, needs checking in HD \\ -- \\ ptc: ignore at this stage, probably not needed}

The regularity analysis carried-out so far is summarised by the following inequalities for the regularity of the  metric components:
%
\begin{align}
    h_{uA} \text{ equation}: \quad & k_{\beta} \geq k_U+1\,,\quad k_{\gamma}\geq k_U +1 \,,
    \label{24IV22.2a}
\\
    h_{uu} \text{ equation}: \quad & k_{\gamma} \geq k_V + 2\,, \quad k_U \geq k_V +1 \,,
    \label{24IV22.2b}
\\
    \partial_u h_{AB} \text{ equation}: \quad & k_{\beta} \geq k_{\partial_u \gamma} + 2 \,, \quad k_U \geq k_{\partial_u \gamma} + 1\,,
    \label{24IV22.2c}
\\
    \partial_u\partial_r h_{uA} \text{ equation}: \quad & k_{U} \geq k_{\partial_u U} + 2\,, \quad k_V \geq k_{\partial_uU} +1 \,, \quad k_{\partial_u\gamma} \geq k_{\partial_u U} + 1
     ,,
    \label{24IV22.2d}
\\
   \partial_u h_{uu} \text{ equation}: \quad & k_{U} \geq k_{\partial_uV} + 1\,, \quad k_V \geq k_{\partial_u V} + 2 \,,\quad k_{\gamma} \geq k_{\partial_u V} + 2\,.
    \label{24IV22.2e}
\end{align}
%
A consistent scheme for the linearised equations will thus be obtained if we choose any field $h_{AB}$ such that $h_{AB}(r,\cdot) \in \Hgamma$,  for all  $r\in[r_1,r_2]$, with $k_\gamma \ge 4$ and
%
\begin{equation}\label{25IV22.p6}
  k_\beta = k_\gamma
  \,,\quad
  k_U = k_\gamma -1
  \,,\quad
  k_V = k_\gamma -2
  \,,\quad
  k_{\partial_u U} = k_{\gamma} - 3
  \,,\quad
  k_{\partial_u V} = k_\gamma - 4
  \,,\quad
  k_{\partial_u \gamma}  = k_\gamma -2
  \, .
\end{equation}
%
Note that the question of regularity of $r$-derivatives of $\gamma$ has been swept under the rug using integration by parts. This question will need to be addressed when dealing with the nonlinear problem.

The regularity properties of the metric will be compatible with  gauge transformations~\eqref{24IX20.1}-\eqref{24IX20.23} if we assume, using obvious notation,
%
\begin{align}
        h_{uA} \text{ equation}: \quad &
        k_{\xi^u} \geq k_U+ 3\,,\quad
        k_{\partial_u\xi^u} \geq k_U+1\,,\quad
        k_{\xi^A}\geq k_U + 2 \,,
    \label{24IV22.3a}
\\
    h_{ur} \text{ equation}: \quad &
        k_{\partial_u\xi^u} \geq k_\beta\,,\quad
        k_{\xi^A}\geq k_{\beta} + 1\,,
    \label{24IV22.3b}
\\
    h_{uu} \text{ equation}: \quad & k_{\partial_u\xi^u}\geq k_{V} + 2\,, \quad k_{\partial_u\xi^B}\geq k_V +1 \,,\quad k_{\xi^u}\geq k_V +2\,,\quad k_{\xi^B}\geq k_V + 1\,,
    \label{24IV22.3c}
\\
    h_{AB} \text{ equation}: \quad & k_{\xi^A}\geq k_{\gamma} + 1\,,\quad k_{\xi^u} \geq k_{\gamma} + 2 \,,
    \label{24IV22.3d}
\\
    \partial_u h_{AB} \text{ equation}: \quad & k_{\partial_u\xi^A}\geq k_{\partial_u\gamma} + 1\,,\quad k_{\partial_u\xi^u} \geq k_{\partial_u\gamma} + 2 \,.
    \label{24IV22.3e}
\end{align}
%



==> TableOfOperators.tex <==
\ptcheck{2VI23, but without logs; refs of equations to recheck; \peqref{26V23.1} not checked so far so needs checking }
 \ptcr{consider removing the table, perhaps not needed anymore?}
%
\begin{table}[t]
\hspace{-2.8cm}
{\small 
 \begin{tabular}{||c|c|c|c|c|c||}
  \hline
  \hline
     Gluing field
        & defined
            & exponent $q$
                & Gluing operator $\hat D$
                    & Gauge operator $\hat L$
                        & Equation
     \\
  \hline
    $\red{\overadd{*}{\Hf}_{uA}}$
    \checkmark
      & \peqref{24VII22.1b}
        &   $n-4$
                & $ \zdivtwo$
                     & % $m \zspaceD_A \kxi{2}^u$
                     no gauge
                        &   \peqref{7III23.4}
  \\
  \hline
    $  \overadd{0}{H}_{uA}$
    \checkmark
     & \peqref{21II23.1}
        & $-4$
                & $\zdivtwo$
                     & $ \partial_u \kxi{2}_A  + \alpha^2  \zspaceD_A \kxi{2}^u
                     + O(\alpha^4)$
                        &\peqref{7III23.7}
  \\
  \hline
    $\overadd{p}{\Hf}_{uA}$, $ p\ge 1$
     \checkmark
      & \peqref{6III23.w4}
        &  $-p-4$
                &  $\zspaceD^B \overadd{p}{\chi}\ofP  $ (\peqref{6III23.w2})
                     &  $
       \partial_u^{p+1} \kxi{2}_A + \alpha^2 \overadd{p}{D}(\partial^{p-1}_u\xi)_A + O(\alpha^4)$
                        &    \peqref{26V23.1}
  \\
  \hline
   $ \chi$
    \checkmark
     &\peqref{20II23.2}
        & $n-5$
            & $\zdivone\circ\zdivtwo$
                & % $\frac{2 n m}{n-1} \zspaceD_B \kxi{2}^B$
                no gauge
                        &  \peqref{7III23.1}
\\
  \hline
   $ \overadd{i}{q}_{AB}$, $n$ even,
    \checkmark
      & \peqref{6III23.w8}
         &  $\frac{n-7-2i}{2}$ ($\alpha=0$)
             &  $\overadd{i}{\psi}\ofP $ (\peqref{6III23.w9})
                 & no gauge
                        & \peqref{11III23.2}
\\
     or $n$ odd, $i<\frac{n-3}{2}$
        &
            & $\frac{n-7+2i}{2}$ ($\alpha\neq 0$)
                & $1$ ($\alpha\neq 0$)
                    &
                        &
\\
  \hline
   $ \overadd{i}{q}_{AB}$, $n$ odd,
        &
            &
                &
                    &
                        &
\\
     $i=\frac{n-3}{2}$,
     $\alpha = 0$
        &
            & $-2$
                & $\overadd{\frac{n-3}{2}}{\psi}\ofP $
                    & $\hLop(\xi^u)$
                        & \peqref{24IV23.1}
\\
    \phantom{$i=\frac{n-3}{2}$,}
     $\alpha \neq 0$
        &%
            & $\tcp{n-5}$
                & 1
                    &
                        &
\\
     $i=\frac{n-1}{2}$,
     $\alpha = 0$
        &
            & $-3$
                & $\overadd{\frac{n-1}{2}}{\psi}\ofP $
                    & $\Lop(\xi)$
                        & \peqref{24IV23.3}
\\
    \phantom{$i=\frac{n-3}{2}$,}
     $\alpha \neq 0$
        &%
            & $n-4$
                & 1
                    &
                        &
\\
     $i=\frac{n+1}{2}+j$
        & \peqref{17IV23.2}
            & $-j-4$
                &  $\overadd{\frac{n+1}{2}+j}{\psi}\ofP $
                    & $\Lop(\partial^{j+1}_u\xi) $
                        & \peqref{25IV23.1}
  \\
  \hline
  \hline
\end{tabular}
}
\caption{The operators appearing in \eqref{5V23.2} and \eqref{6V23.p1}. $P$ is defined in \peqref{16V22.1b}. The radially conserved charges belong to the kernel of the gluing operator $\hat D$, which provides an obstruction to gluing when non-empty. The case   $n=5$ and $i=1$, requires separate attention because then the exponents $n-5$ and $ (n-7+2i)/2$ coincide. {\redc n=5 not done yet  } \tcp{Actually this occurs whenever $i=\frac{n-3}{2}$. Also what about the matching of powers $n-4$, when $i=(n-1)/2$ in  $ (n-7+2i)/2$. }
}\label{T6V23.1}
\end{table}
% 

==> TableOfOperatorsM.tex <==
%
\begin{table}[t]
\hspace{-2.8cm} 
 \begin{tabular}{||c|c|c|c|c|c||}
  \hline
  \hline
     Gluing field 
        & defined
            & exponent $q$ 
                & Gluing operator $\hat D$ 
                    & Gauge operator $\hat L$ 
                        & Equation
     \\
  \hline
    $\overadd{-1}{\Hf}_{uA}$
      & \peqref{8V23.1}
        &   $n-4$
                & $ \zdivtwo$
                     & 
                        &   \peqref{7III23.4}
  \\
  \hline
    $  \overadd{0}{H}_{uA}$
     & \peqref{21II23.1} 
        & $-4$
                & $\zdivtwo$
                     & $n \partial_u \kxi{2}_A  + \alpha^2 n \zspaceD_A \kxi{2}^u$ 
                        &\peqref{7III23.7}
  \\
  \hline
    $\overadd{p}{\Hf}_{uA}$, $ p\ge 1$
      & \peqref{6III23.w4} 
        &  $-p-4$ 
                &  $\zspaceD^B \overadd{p}{\chi}(P) $ (\peqref{6III23.w2})
                     &  $ 
     n \partial_u^{p+1} \kxi{2}_A + \frac{\alpha^2 n}{n-1} \zspaceD_A\zspaceD_B\partial_u^{p-1}\kxi{2}^B$ 
                        &    \peqref{11III23.1}
  \\
  \hline
   $ \chi$  
     &\peqref{20II23.2} 
        & $n-5$  
            & $\zdivone\circ\zdivtwo$
                & 
                        &  \peqref{7III23.1}
\\
  \hline
   $ \overadd{i}{q}_{AB}$, $n$ even, 
      & \peqref{6III23.w8}
         &  $\frac{n-7+2i}{2}$
             &  
                 & no gauge 
                        & \peqref{11III23.2}
\\
     or $n$ odd, $i<\frac{n-3}{2}$
        &
            &
                &
                    &
                        &
\\
  \hline
   $ \overadd{i}{q}_{AB}$, $n$ odd,
        &
            &  
                &  
                    &  
                        & 
\\
     $i=\frac{n-3}{2}$
        &
            & $-2$
                & $\overadd{\frac{n-3}{2}}{\psi}(P)$
                    & $\hLop(\xi^u)$
                        & \peqref{24IV23.1}
\\
     $i=\frac{n-1}{2}$
        &
            & $-3$
                & $\overadd{\frac{n-1}{2}}{\psi}(P)$
                    & $\Lcheck(\xi)$
                        & \peqref{24IV23.3}
\\
     $i=\frac{n+1}{2}$
        &
            & $-4$, $\log$
                &  $\overadd{\frac{n+1}{2}}{\psi}(P)$,  $\overadd{\frac{n+1}{2}}{\psi}_L(P)$
                    & $\Lop(\partial_u\xi) + \alpha^2 \Lop_{\alpha}(\xi^u)$ 
                        & \peqref{24IV23.5}
\\
     $i=\frac{n+1}{2}+j$
        &
            & $-j-4$, $\log$
                &  $\overadd{\frac{n+1}{2}+j}{\psi}(P)$,  $\overadd{\frac{n+1}{2}+j}{\psi}_L(P)$
                    & $\Lop(\partial^{j+1}_u\xi) + \tilde{\Lop}_{\alpha}(\partial_u^{j-1}\xi)$
                        & \peqref{25IV23.1}
  \\
  \hline
  \hline
\end{tabular}
\caption{The operators appearing in \eqref{5V23.2} and \eqref{6V23.p1}. $P$ is defined in \peqref{16V22.1b};
}\label{T6V23.1a}
\end{table} 
%

==> TableinWords.tex <==
 \begin{enumerate}
        \item[i.] $\partial_r \tilde\hBo_{uA}$: When $m=0$, gauge invariant obstruction associated with $\overadd{-1}{\Hf}_{uA}$ implies the following condition on $\dt_{\secN_1}$ and $\dt_{\secN_2}$:
        %
        \begin{align}
            \label{8V23.2}
           \kQ{1}{}[\dt_{\secN_1}](\pi^A)&=\kQ{1}{}[\dt_{\secN_2}](\pi^A)
            \,,
        \end{align}
        %
        where $\pi^A \in \ker \zdivtwo^\dagger = \CKV$.

        When $m\neq 0$, the gauge invariant obstruction reduces to $\pi^A \in \KV$
        while the gauge dependent radial charge can be matched using the gauge field $(\zspaceD^A\kxi{2}_A)^{[=1]}$ on $S^2$.

        Regardless of the vanishing, or not, of $m$, the
         projected integrated transport equation \eqref{6V23.2} with $\tilde H$ equal to $\overadd{-1}{\Hf}_{uA}$
           determines the interpolating
          field $\kphi{4-n}_{AB}^{[\TTt^\perp]}$.
        %
        \item[ii.] $\tilde\hBo_{uA}$: The integrated transport equation, \eqref{7III23.7} below, for $\overadd{0}{\Hf}_{uA}$ determines the field $\kphi{4}_{AB}^{[\TTt^\perp]}$ as well as the gauge field $\partial_u\kxi{2}{}_A^{[\CKV]}$.
        %
        \item[iii.] $\tilde\hBo_{uu}$: When $m=0$, gauge invariant obstruction associated with $\chi$ implies the following condition on $\dt_{\secN_1}$ and $\dt_{\secN_2}$:
        %
        \begin{align}
            % \chi[\dt_{\secN_1}]^{[\ker \mrL^\dagger]} &= \chi[\dt_{\secN_2}]^{[\ker \mrL^\dagger]}
            % \nonumber
            % \\
            % \iff
            \label{16IV23.1}
           \kQ{2}{}[\dt_{\secN_1}](\lambda)&=\kQ{2}{}[\dt_{\secN_2}](\lambda)
            \,,
        \end{align}
        %
        where $\lambda \in \ker \mrL^\dagger$ with $\mrL = \zdivone\circ\zdivtwo$ (compare \eqref{1XI22.w1}).

        When $m\neq 0$, the gauge invariant obstruction reads
        %
        \begin{align}
           \kQ{2}{}[\dt_{\secN_1}](\lambda^{[1]})&=\kQ{2}{}[\dt_{\secN_2}](\lambda^{[1]})
            \,,
        \end{align}
        %
        while the gauge dependent radial charge can be matched using the gauge field $(\zspaceD^A\kxi{2}_A)^{[=1]}$ on $S^2$.

        For any $m$, the projection of Equation~\eqref{7III23.1} below  for $\chi$ determines the interpolating field $\kphi{5-n}_{AB}^{[(\ker \mrL)^\perp]}$.
        %
        \item[iv.] $\partial^p_u \tilde\hBo_{AB}$ for $1 \leq p \leq k$: When $n$ is even and $m=0=\alpha$,
        the gauge invariant obstruction associated with $\overadd{p}{q}_{AB}$ implies the following condition on $\dt_{\secN_1}$ and $\dt_{\secN_2}$:
        %
        \begin{align}
            \int_{\secN_2} (\overadd{p}{\kerpsi})^{AB} \overadd{p}{q}_{AB} \sm
            - \int_{\secN_1} (\overadd{p}{\kerpsi})^{AB} \overadd{p}{q}_{AB} \sm = 0\,,
        \end{align}
        %
        where $\overadd{p}{\kerpsi}\in\ker \overadd{p}{\psi}(P)$ (see \eqref{23IV23.3}).
        The projection on $(\ker \overadd{1}{\psi}(P))^\perp$ of Equation \eqref{11III23.2} below
        %for $\overadd{p}{q}_{AB}$
         determines the field $\kphit{AB}{(9-n-2p)/2}{}^{[(\ker \overadd{1}{\psi}(P))^\perp]}$.


        When $n$ is even and $m=0$ but $\alpha \neq 0$, there are no radially conserved charges and the ite-$\varphi$ for $\overadd{p}{q}_{AB}$ determines the field $\kphit{AB}{(9-n+2p)/2}$.

        When $n$ is odd and $m=0$, ...
         \ptcr{not done yet}

        When $m\neq 0$, there are no gauge invariant obstructions; the ite-$\varphi$ for $\overadd{p}{q}_{AB}$ determines the field $\kphit{AB}{(7-n+2p(n-1))/2}{}$.
        %
        \item[v.] $\partial_u^p\tilde\hBo_{uA}$ for $1\leq p \leq k$: When $n$ is even, the integrated transport equation for $\overadd{p}{\Hf}_{uA}$ determines the field $\kphit{AB}{p+4}^{[(\ker[ \zspaceD^A\overadd{p}{\chi}])^\perp]}$ as well as the gauge field $\partial_u^{p+1}\kxi{2}{}_A^{[\ker\overadd{p}{\chi}\circ C ]}$.
        %
    \end{enumerate}
    % 

==> TensorHarmonics.tex <==
\subsection{Vector and tensor spherical harmonics}
 \label{ss20X22.1}

For integers $\ell\geq 1$, $-\ell\leq m \leq \ell$, let $Y^{(\ell m)}$ be the standard spherical harmonics on the unit sphere. Following the notations and conventions of \cite{ACR2,Czimek:2016ydb},
we define the  \emph{vector spherical harmonics}, as well as
trace-free symmetric \emph{$2$-tensor spherical harmonics}
on $S^2$ as:

\begin{enumerate}
    \item For $\ell \geq 1$, $-\ell\leq m\leq \ell$, define the vector fields
%
    \begin{align}
        E_A^{(\ell m)}:= -  \frac{1}{\sqrt{\ell(\ell+1)}} \zspaceD_A Y^{(\ell m)}
        \,,\qquad
        H_A^{(\ell m)} := \frac{1}{\sqrt{\ell(\ell+1)}} \epsilon_{AB} \zspaceD^B Y^{(\ell m)}\,,
    \end{align}
%
    where $\epsilon_{AB}$ denote the volume two-form of $S^2$.
    \item For $\ell \geq 2$, $-\ell \leq m \leq \ell$, define the trace-free symmetric $2$-tensors
%
    \begin{align}
    \label{18X22.2w}
        \psi^{(\ell m)}_{AB}&:= -\frac{1}{\sqrt{\frac{1}{2}\ell(\ell+1)-1}} C(E^{(\ell m)})_{AB}
        \,, &
        \phi_{AB}^{(\ell m)}& := -\frac{1}{\sqrt{\frac{1}{2}\ell(\ell+1)-1}}
        C(H^{(\ell m)})_{AB}\,,
        % \nonumber
        % \\
        % & = -\frac{1}{\sqrt{\frac{1}{2}\ell(\ell+1)-1}} \TS[\zspaceD_A E_B^{(\ell m)}]
        % &
        % & = -\frac{1}{\sqrt{\frac{1}{2}\ell(\ell+1)-1}} \TS[\zspaceD_A H_B^{(\ell m)}]
    \end{align}
%
where the operator $C(\xi)_{AB} = TS(\zspaceD_A \xi_B)$ of \eqref{18X22.41}
corresponds to the operator  $-\slashed{\mathcal{D}}_2^*$
 of \cite{ACR2,Czimek:2016ydb}.
 \ptcheck{19X22}
\end{enumerate}

Let us summarise the properties of these
tensor harmonics, as needed in the main text. More details and proofs can be found   in \cite{Czimek:2016ydb}, see also~\cite{JezierskiPeeling}.

\begin{Lemma}
\label{l18X22.1}
The following holds.
\begin{enumerate}
    \item On $S^2$, $L^2$-integrable functions $f$, vector fields $\xi$ and trace-free symmetric $2$-tensors $\varphi$ can be decomposed as
%
    \begin{align}
        f &= \sum_{\ell\geq 0 }\sum_{-\ell\leq m\leq \ell} f^{\ell m} Y^{(\ell m)}\,,
        \nonumber
\\
        \xi_A &= \sum_{\ell\geq 1 }\sum_{-\ell\leq m\leq \ell}\xi^{(\ell m)}_E E^{(\ell m)}_A
        + \xi^{(\ell m)}_H H^{(\ell m)}_A\,,
        \nonumber
\\
        \varphi_{AB} &= \sum_{\ell\geq 2 }\sum_{-\ell\leq m\leq \ell}\varphi^{(\ell m)}_{\psi} \psi^{(\ell m)}_{AB}
        + \varphi^{(\ell m)}_{\phi} \phi^{(\ell m)}_{AB}\,,
    \end{align}
%
    where
%
    \begin{align}
        f^{(\ell m)} &:= \int_{S^2} f Y^{(\ell m)} \sm\,, & &
        \nonumber
\\
    \xi^{(\ell m)}_E &:= \int_{S^2} \xi^A E_A^{(\ell m)}
    \,, \qquad &
    \xi_H^{(\ell m)}&:= \int_{S^2} \xi^A H^{(\ell m)}_{A} \sm \,,
            \nonumber
\\
    \varphi_{\psi}^{(\ell m)} &:=\int_{S^2} \varphi^{AB} \psi_{AB}^{(\ell m)}
    \,, \qquad &
    \varphi_{\phi}^{(\ell m)}&:= \int_{S^2} \varphi^{AB} \phi^{(\ell m)}_{AB} \sm \,.
    \end{align}
%
    \item It holds that for $\ell \geq 2$,
%
    \begin{align}
    \label{18X22.1w}
        \zspaceD^A \psi_{AB}^{(\ell m)}=
          \sqrt{\frac{1}{2}\ell(\ell+1)-1}
           \,
             E_B^{(\ell m)}\,,
        \qquad
        \zspaceD^A \phi_{AB}^{(\ell m)} =
          \sqrt{\frac{1}{2}\ell(\ell+1)-1}
          \,
           H_B^{(\ell m)}\,.
    \end{align}
%
    \item The space of conformal Killing vector fields on $S^2$ is spanned by $E_A^{(1m)}$ and $H_A^{(1m)}$.
\end{enumerate}
\end{Lemma}






==> TopologicalSolutions.tex <==

\FG{Added discussion of different topologies here.}
\subsection{``Topological'' Kerr--AdS black holes in higher dimensions}
In order to compare to Birmingham--Kottler metrics~\eqref{23VII22.3}, which have different topologies of the transverse space $\secN$ when $\Lambda<0$, we would like a Kerr--AdS solution which can accommodate such topologies (at least in the slow rotation linearisation).
We note that in the literature such ``topological'' rotating black holes have been introduced in ~\cite{Klemm:1997ea,Klemm:1998kd} in two relevant cases.
First, in four dimensions~\cite{Klemm:1997ea} the parameters and coordinates can be analytically continued such that the resulting metric has a Birmingham--Kottler metric with $\myGauss=-1$ in the limit $a\to0$. Note however, the cross section of the four dimensional rotating 
topological black hole no longer has constant curvature. 
\ptcr{ not clear if it compactifies,?in which case irrelevant for us?
}
Second, for the higher 
dimensional metric~\eqref{eq: Kerr AdS} with one rotation parameter (introduced in \cite{Hawking:1998kw}) a similar analytic cont
inuation procedure can be implemented. 
%
\footnote{We note that there is a third case discuss
ed in~\cite{Klem
m:1997ea} where the analytic continuation starts from the Pleba\'nski--Demia\'nski~\
cite{Plebanski
:1976gy} metric representing a more general axi-symmetric spacetime which contains the Kerr--(A)dS spacetime as a limit. 
Again it involves an analytic continuation of some coordinates and parameters. 
However, it is not clear that the end result is relevant for our discussion since it carries an angle dependent angular velocity at spatial infinity and the Hamiltonian charges diverge there. 
In any case, such an example only applies in 4 dimensions since there is no higher dimensional generalization of the  Pleba\'nski--Demia\
'nski spacetime from which a similar such limit could be taken.
}.
\FG{needs further checking if the procedure mentioned in \cite{Klemm:1997ea} works and it is in fact relevant.} 
%

Let us reproduce this second case in detail. When only one rotation parameter is present it is convenient to write the constraint \eqref{3VI24.f1} as $\mu_{1}=\sin\theta$ and $\mu_i=\cos(\theta)x_i$ for $1< i\leq N+\delta$ and $\sum_{i=2}^{N+\delta}x_i^2=1$. Then, after some simplifications, the metric \eqref{eq: Kerr AdS} can be written  in the following way
%
\begin{align}\label{3VI24.f2}
	ds^2=&-\frac{\Delta_\theta}{\Xi_1}(1-\alpha^2r^2)dt^2+\frac{2mr^{5-d}}{\rho^2}\left(\frac{\Delta_\theta}{\Xi_1}dt+\frac{a\sin^2\theta}{\Xi_1}d\phi_1\right)^2
	\nonumber\\
	&+\frac{\rho^2}{\Delta_r}dr^2+\frac{r^2+a^2}{\Xi_1}\sin^2\theta d\phi_1^2 
 +\frac{\rho^2}{\Delta_\theta}d\theta^2
  +r^2  \cos^2\theta d\Omega_{d-4}^2\,,
\end{align}
%
where,
%
\begin{equation}
d\Omega_{d-4}^2=\sum_{i=2}^{N+\delta-1}\left(dx_i^2 + x_i^2d\phi^2_i\right) + dx_{N+\delta}^2\,,
\end{equation}
%
is the metric on the $(d-4)$-sphere, $\Xi_1=1+\alpha^2a_1^2$ as before, and we have introduced the metric functions
\wancheck{6VI}
%
\begin{align}
	\Delta_r&:=r^{(5-d)}(V-2m)\big|_{a_i=0,i>1}=(r^2+a^2)(1-\alpha^2 r^2)-2m r^{5-d}\,,\\
	\Delta_\theta&:=\Xi_1W\big|_{a_i=0,i>1}=1+\alpha^2 a_1^2\cos^2 \theta\,,\\
	\rho^2&:=r^{(5-d)}U\big|_{a_i=0,i>1}= r^2+a_1^2\cos^2\theta\,.
\end{align} 
%
The expression in \eqref{3VI24.f2} is the metric in \cite{Hawking:1998kw} written in coordinates which do not rotate at infinity (i.e. the angle $\phi_1$ here is related to the angle $\varphi$ in \cite{Hawking:1998kw} by $\phi_1=\varphi-a\alpha^2t$) and with the negative rotation parameter $a\to-a$.


Now the analytic continuation proceeds as follows; in order to convert the constraint \eqref{3VI24.f1} into one parameterising a constant curvature space we set $x_i=\sin\chi y_i$ for $2\leq i<N+\delta-1$ and $xy_{N+\delta}=\cos(\chi)$, where $\sum_{i=2}^{N+\delta-1}y_i^2 =1$. 
Next we introduce a parameter $\sigma$ which will control the continuation. We set, $\chi=\sigma\bar{\chi}$. Then, the metric on the $(d-4)$-sphere becomes
%
\begin{equation}
	d\Omega_{d-4}^2=\sigma^2\left[d\bar{\chi}^2+
	\sigma^{-2}\sin^2(\sigma\bar{\chi})d\Omega_{d-5}^2\right]:=\sigma^2d\Sigma^2_{d-4}\,,
\end{equation}
%
where $d\Omega_{d-5}^2$ is the standard metric on the $(d-5)$ sphere. Clearly when $\sigma\to i$ the metric becomes
%
\begin{equation}
d\Omega_{d-4}^2=i^2(d\bar{\chi}^2+
\sinh^2(\bar{\chi})d\Omega_{d-5}^2)\,,
\end{equation}
%
which is conformal to the standard metric on the hyperbolic $(d-4)$-space $H^{d-4}$. Similarly if we were to send $\sigma\to0$ we would obtain a conformally flat metric with (divergent) prefactor $\sigma^{-2}$. To amend this and retain the signature of the singly rotating 
Kerr-(A)dS metric \eqref{3VI24.f2} it is necessary to make the following rescalings
%
\begin{equation}\label{3VI24.f4}
	t=\sigma\bar{t}\,,\quad r= \sigma^{-1}\bar{r}\,, \quad \theta= \sigma\bar{\theta}\,\quad a=\sigma^{-1}\bar{a}\,,\quad m=\sigma^{-(d-1)}\bar{m}\,.
\end{equation}
%
Then 
%
\begin{align}\label{3VI24.f3}
ds^2_{\sigma}=&-\frac{\Delta_{\bar{\theta}}}{\bar{\Xi}_1}(\sigma^2-\alpha^2\bar{r}^2)d\bar{t}^2
+\frac{2\bar{m}\bar{r}^{5-d}}{\bar{\rho}^2}\left(\frac{\Delta_{\bar{\theta}}}{\bar{\Xi}_1}d\bar{t}+\frac{\bar{a}\sin^2(\sigma\bar{\theta})}{\bar{\Xi}_1}d\phi_1\right)^2
\nonumber\\
&+\frac{\bar{\rho}^2}{ \Delta_{\bar{r}} } d\bar{r}^2
+\frac{\bar{r}^2+\bar{a}^2}{\bar{\Xi}_1}\sin^2(\sigma\bar{\theta})d\phi_1^2+\frac{\bar{\rho}^2}{\Delta_{\bar{\theta}}}\sigma^2d\bar{\theta}^2
 +\bar{r}^2\cos^2(\sigma\bar \theta)
  d\Sigma_{d-4}^2\,,
\end{align}
where now, $\bar{\Xi}_1=\sigma^2+\alpha^2\bar{a}_1^2$, and
%
\begin{align}
\Delta_{\bar{r}}&:=(\bar{r}^2+\bar{a}^2)(\sigma^2-\alpha^2 \bar{r}^2)-2\bar{m} \bar{r}^{5-d}\,,\\
\Delta_{\bar{\theta}}&:=\sigma^2+\alpha^2 \bar{a}_1^2\cos^2 (\sigma\bar{\theta})\,,\\
\bar{\rho}^2&:=\bar{r}^2+\bar{a}_1^2\cos^2(\sigma\bar{\theta})\,.
\end{align} 
%


Under the substitution 
$\sigma\to i$ this reproduces the results of \cite{Klemm:1997ea,Klemm:1998kd}. Note in these coordinates it may appear that when 
$\sigma=i$ the $d\phi_1^2$ and $d\bar{\theta}^2$ terms in the second line of \eqref{3VI24.f3} change sign and so may the signature of the metric. In fact this does not occur. In the first case, there are extra $d\bar{\phi}_1^2$ terms proportional to $\bar{m}$ which compensate. In the second case, $\Delta_{\bar{\theta}}$ is in fact negative too since $\alpha^2<0$ for $\Lambda<0$ (note that the combination $\Delta_{\bar{\theta}}/\bar{\Xi}_1$ is positive). 

Moreover we can substitute $\bar{a}_1\to0$ yielding,
\begin{equation}
	\lim_{\bar{a}_1\to0}\lim_{\sigma\to i}ds^2_{\sigma}=ds^2_{BK}\big|_{\myGauss=-1}\,.
\end{equation}
That is, when the rotation is zero we recover the Birmingham--Kottler metric of \eqref{23VII22.3} in Boyer--Lindquist type coordinates with constant negative curvature $\myGauss=-1$.
\begin{equation}
ds^2_{BK}=fd\bar{t}^2+\frac{d\bar{r}^2}{f} +r^2\ringh_{AB}dx^Adx^B\,,\quad f=\myGauss-2mr^{n-2}-\alpha^2r^2\,.
\end{equation}
In the next section we will demonstrate explicitly that such metrics can be put into Bondi form in the standard way. Notice this construction 
 covers the hyperboloidal Kerr-AdS in four dimensions of \cite{Klemm:1997ea}.


On the other hand, the limit  $\sigma\to 0$ results in a degenerate metric and we thus cannot recover a flat Birmingham--Kottler metric. 
Interestingly, if we change the order of the limits we do recover the relevant Birmingham--Kottler spacetime
\begin{equation}
\lim_{\sigma\to 0}\lim_{\bar{a}_1\to0}ds^2_{\sigma}=ds^2_{BK}\big|_{\myGauss=0}\,.
\end{equation}
Because we are required to rescale $a=\sigma^{-1}\bar{a}_1$ in order to maintain the signature of the metric and keep its structure this makes the limit $\bar{a}_1\to0$ and $\sigma\to 0$ delicate.

Let us now try to apply such a continuation to the general Kerr--AdS metric. First rather than focusing on one particular angle we will directly rescale the constrained variables $\mu_i=\sigma\bar{\mu}_i$, for $1\leq i<N+\delta-1$, and $\mu_{N+\delta}=\bar{\mu}_{N+\delta}$. Then the constraint is
%
\begin{equation}\label{3VI24.f5}
\sum_{i=1}^{N+\delta-1} \bar{\mu}_i^2+	\sigma^{-2}\bar{\mu}^2_{N+\delta} =	\sigma^{-2}\,.
\end{equation}
%
Now the rescaling is clear, for $\sigma\to\{1,i,0\}$ 
 \ptcr{infty instead of o?}
we have a constraint which resembles how one would embed $N$-dimensional spherical, hyperbolic, or flat space in one higher dimension. For consistency, we are again required to scale
%
\begin{equation}\label{3VI24.f6}
t=\sigma\bar{t}\,,\quad r= \sigma^{-1}\bar{r}\,, \quad \,\quad a=\sigma^{-1}\bar{a}\,,\quad m=\sigma^{-(d-1)}\bar{m}\,.
\end{equation}
%
The new metric functions take the form,
%
\begin{align}
\bar{W}&=\sigma^2\sum_{i=1}^{\red{N+\delta-1}} \frac{\bar{\mu}_i^2}{\bar{\Xi}_i \,\sigma^{-2}}+ \frac{\bar{\mu}_{\red{N}+\delta}^2}{\bar{\Xi}_{N+\delta}\,\sigma^{-2}}\,,
\quad \bar{V}=\bar{r}^{\delta-2}(\sigma^2-\alpha^2\bar{r}^2)\prod_{i=1}^\red{N}(\bar{r}^2+\bar{a}_i^2)\,,\nonumber\\
U&%=\frac{\bar{V}}{\sigma^2-\alpha^2\bar{r}^2}\Bigl(1-\sigma^2\sum_{i=1}^\red{N}\frac{\bar{a}_i^2\bar{\mu}_i^2}{\bar{r}^2+\bar{a}_i^2}\Bigr)
=\bar{r}^\delta\left(\frac{\bar{\mu}_{N+\delta}^2}{\bar{r}^2+\bar{a}_{N+\delta}^2}+ \sigma^2\sum_{i=1}^{N+\delta-1}\frac{\bar{\mu}_i^2}{\bar{r}^2+\bar{a}_i^2}\right)\prod_{i=1}^\red{N}(\bar{r}^2+\bar{a}_i^2)\,,
\quad 
\bar{\Xi}_i=\sigma^2+\alpha^2 \bar{a}_i^2\,,
\end{align}
%
and likewise for the metric
 \ptcr{signature problem, forms not independent?}
%
\begin{align}\label{3VI24.f7}
ds^2_{K,\sigma}=&-\bar{W}(\sigma^2-\alpha^2\bar{r}^2)d\bar{t}^2+\frac{\bar{U}d\bar{r}^2}{\bar{V}-2\bar{m}}
 \nonumber
\\
&+\frac{2\bar{m}}{\bar{U}}\biggl(\bar{W}d\bar{t}+\sum_{i=1}^\red{N+\delta-1} \frac{\bar{a}_i \bar{\mu}_i^2 d\phi_i}{\bar{\Xi}_i\,\sigma^{-2}}+ \frac{\bar{a}_{N+\delta} \bar{\mu}_{N+\delta}^2 d\phi_{N+\delta}}{\bar{\Xi}_{N+\delta}} \biggr)^2
\nonumber\\
&+\sum_{i=1}^\red{N+\delta-1}\frac{\bar{r}^2+\bar{a}_i^2}{\bar{\Xi}_i\,\sigma^{-2}}\bigl(\bar{\mu}_i^2d \phi_i^2+d\bar{\mu}_i^2)
+ \frac{\bar{r}^2+\bar{a}^2_{N+\delta}}{\bar{\Xi}_{N+\delta}}\left( d\bar{\mu}_{\red{N}+\delta}^2+(1-\delta) \bar{\mu}_{N+\delta}^2d\phi_{N+\delta}^2\right)
\nonumber\\
&+\frac{\alpha^2\sigma^2}{\bar{W}(\sigma^2-\alpha^2\bar{r}^2)}\Bigl(\sum_{i=1}^\red{N+\delta-1} \frac{\bar{r}^2+\bar{a}_i^2}{\bar{\Xi}_i\,\sigma^{-2}}\bar{\mu}_i d\bar{\mu}_i
+\frac{\bar{r}^2+\bar{a}_{N+\delta}^2}{\bar{\Xi}_{N+\delta}}\bar{\mu}_{\red{N}+\delta} d\bar{\mu}_{\red{N}+\delta}\Bigr)^2\,.
\end{align}
%
Recall that here $a_{N+1}=0$ and similarly we define $\phi_{N+1}:=0$ in order to write both even and odd dimensions at once.
The metric can be meromorphically continued in $\sigma$ to the complex plane, and the  substitution $\sigma\to i$ now produces a ``new'' to our knowledge metric. In even dimensions, similarly to the singly rotating case, the signature of this metric does not change provided that $-1-\alpha^2\bar{r}^2>0$. 
%
\footnote{
	Note that $\bar{\Xi}_i\sigma^{-2}|_{\sigma=i}=1-\alpha^2\bar{a}_i>0$ for negative $\Lambda$ (and thence positive $-\alpha^2$).
}.
%
\FG{Needs double checking...}
In odd dimensions the extra angle $\phi_N$ results in a change of signature.

Happily, the Birmingham--Kottler metric with $\sigma^2=\myGauss=-1$ in Boyer--Lindquist coordinates can be recovered in both even and odd dimensions
%
\begin{equation}
	\lim_{\bar{a}_1\to0}\lim_{\sigma\to i}ds^2_{\sigma}=ds^2_{BK}\big|_{\myGauss=-1}\,.
\end{equation}
%


Finally, although the metric diverges in the $\sigma\to0$ limit we can again recover a flat Birmingham--Kottler metric from the following limit
\begin{equation}
\lim_{\sigma\to 0}\lim_{\bar{a}_1\to0}ds^2_{K,\sigma}=ds^2_{BK}\big|_{\myGauss=0}\,.
\end{equation}
Going forwards we shall drop the bars on the coordinates and parameters as they play no further role and hope that this will not lead to any confusion.








==> VectorScalar.tex <==
\subsection{Scalar-vector decomposition of vector fields}
\label{app16X23.1}
\input{decomp}

==> deltaBeta.tex <==
{\redca{6VI}
Let $Q|_{\delta\beta=0}$ be one of the radial charges  in the gauge $\delta\beta=0$. We can write
%
\begin{equation}\label{5VI24.4}
  Q|_{\delta\beta=0} = \sum_{i=-1}^{q}
 F_i  \Big[
	 \partial_{\tdu}^{i+1}  \xi^{u}(\tdu,x^A) 
\Big]
\,,
\end{equation}
%
for some $q\in \Z$, $q\ge -1$, and some differential operators  $F_i$. After rearrangements this can be rewritten as
%
\begin{equation}\label{5VI24.4}
  Q|_{\delta\beta=0} = \hat F_{-1}+  \sum_{i=0}^{q}
 F_i  \Big[
	 \partial_{\tdu}^{i+1}  \xi^{u}(\tdu,x^A) -
\frac{ \zspaceD_{\tdB} \partial_u^i\TSxi^{B}(\tdu, x^{A})}{n-1}
\Big]
\,,
\end{equation}
%
for some new functional $\hat F_{-1}$. 
We set
%
\begin{equation}\label{5VI24.5}
  Q =   \hat F_{-1}+ 
  \sum_{i=-1}^{q}
 F_i  \Big[
	 \partial_{\tdu}^{i+1}  \xi^{u}(\tdu,x^A) -
\frac{ \zspaceD_{\tdB} \partial_u^i\TSxi^{B}(\tdu, x^{A})}{n-1} - 2 \partial_u^i\delta\beta
\Big]
\,.
\end{equation}
% 
It is straightforward to check that $Q$ is gauge-invariant,  keeping in mind the gauge-transformation law of $\delta \beta$:
         %
\begin{equation}
 2 \partial_u^i\delta\beta \mapsto 	 2 \partial_u^i\delta\beta +  \partial_{\tdu}^{i+1}  \xi^{u}(\tdu,x^A) + 
\frac{ \zspaceD_{\tdB} \partial_u^i\TSxi^{B}(\tdu, x^{A})}{n-1} 
 \,.
  \label{5VI24.7}
\end{equation}
%
}

==> divchiold.tex <==
\subsection{\protect\rm $\zdivtwo\circ\chi$}
 \label{ss12XI22.2}
\index{div@$\zdivtwo \circ \overset{(i)}{\chi}$}%
\index{div@$\zdivtwo \circ \overset{(i)}{\chi} $!image}%
\index{image!div@$\zdivtwo \circ \overset{(i)}{\chi}$}%
\begin{Corollary}
 \label{C14XI23.1}
For $k\ge 0 $ the image
{\rm 
%
$$
 \im_k  
 \big(\zdivtwo \circ \overset{(i)}{\chi}  \big)
 :=
 \im 
 \big(\zdivtwo \circ \overset{(i)}{\chi}\ofP|_{\MMHktwonp} \big)
$$
%
}is closed in $\MMHk$, and we have 
%
{\rm
$$
\im_k  
 \big(\zdivtwo \circ \overset{(i)}{\chi}  \big)
  = 
 \Big(
   \ker \Big(\big(\zdivtwo \circ \overset{(i)}{\chi}  \big)^\dagger 
   \Big)
   \Big)^\perp\cap \MMHk
   \,.
$$
% 
}  
\end{Corollary}

\proof
%
 The operator $\overadd{i}{\chi}\ofP|_{\MHktwonp}$, 
  of order $2n$, is elliptic by Proposition~\ref{P18VIII23.1}, 
  hence its image is closed in $\MHkp$ by Proposition~\ref{P26X23.1}.
{\redca{19XI23.1} Set
%
$$ 
 \im_k  
   \overset{(i)}{\chi} 
 :=
 \im 
 \big( \overset{(i)}{\chi}\ofP|_{\MMHktwonp} \big)
 \,.
$$
%
By \eqref{6V23.1edxd} we have the splitting
%
$$
  \MHk =  \ker\overset{(i)}{\chi} ^\dagger   \oplus  \im_k  
   \overset{(i)}{\chi} 
   \,.
$$
%
Let $\psi_n \in \im \,\overadd{i}{\chi}\ofP (\MHktwonp)$ be Cauchy, thus    $\zdivtwo|_{\MHkp}$ is closed in $\MHk$ by Proposition~\ref{P30X22.1}, the 
 image of  $ \overadd{i}{\chi}\ofP (\MHktwonp)$ by $\zdivtwo$ is readily seen to be closed too.
  \ptcr{not clear...}
%
\qed
%
}  
\subsection{\protect\rm$\zdivone\circ \zdivtwo$}
 \label{ss12XI22.2axb}



\index{div@$\zdivone\circ \zdivtwo$}%
\index{div@$\zdivone\circ \zdivtwo $!image}%
\index{image!div@$\zdivone\circ \zdivtwo$}%
\begin{Proposition}
   \label{P30X22.1}
   Suppose that $(\dmanif,\ringh)$ is Einstein.
   For $k\ge 2$ it holds that
   %
   {\rm
   \begin{equation}\label{5XI23.9}
   \im\big(\zdivone\circ \zdivtwo|_{\MMHkpp}\big)=
   \Big( \ker\big((\zdivone\circ \zdivtwo)^\dagger\big)\Big)^\perp\cap \MMHk
   \,.
   \end{equation}
   }
   %
\end{Proposition}

\begin{Remark}{\rm
It seems clear that the hypothesis that the metric is Einstein is not necessary, but the result in this form is sufficient for our purposes.
%
\qed
%
}
\end{Remark}
\proof
For  all functions $\psi \in H^2$ and for for all symmetric and traceless tensors $h \in H^2$ we have
 %
 \begin{equation}\label{30X22.CKV5cd}
  \int \psi \dnabla^B \dnabla^A  h_{AB}
  =   \int \TS(\dnabla^A \dnabla^B \psi)  h_{AB}
   \,.
 \end{equation}
 %
 Thus
 %
 \begin{equation}\label{5XI23.11}
   (\zdivone\circ \zdivtwo)^\dagger
   =
 C\circ \zspaceD
   \,,
 \end{equation}
   %
   and
   %v
   $$
   \im\big(\zdivone\circ \zdivtwo|_{\MHkpp}\big)
   \subset
   \Big( \ker ( C\circ \zspaceD)\Big)^\perp\cap \MHk
   \,.
   $$
 %
 To obtain the reverse inclusion,
   let $h_{AB}= C(\zspaceD\phi)_{AB}$ for a function $\phi\in \MHkpppp$. Then
 %
 \begin{equation}\label{5XI23.12}
   \zspaceD^A \zspaceD^B h_{AB}
   \blue{=\frac{d-1}{d}\zDelta^2 \phi + \frac{1}{2}(\zspaceD^A \zR) \zspaceD_A\phi +\zR_{AB}\zspaceD^A\zspaceD^B\phi}
   = \frac{d-1}{d} \zDelta (\zDelta + \myGauss d ) \phi
   \,.
 \end{equation}
 %
 Since $d>2$, the operator at the right-hand side of this equation is an isomorphism between
 $\ker (C\circ \zspaceD)^\perp \cap \MHkpppp$
 and
 $\ker (C\circ \zspaceD)^\perp \cap \MHk$,
 \ptcr{refer to the relevant fact in the CKV section, and possibly move this section after the CKV's}
 which finishes the proof.
 %
 \qed
 % 
 


==> divchiold2.tex <==
\subsection{\protect\rm $\zdivtwo\circ\chi$}
 \label{ss12XI22.2}
\index{div@$\zdivtwo \circ \overset{(i)}{\chi}$}%
\index{div@$\zdivtwo \circ \overset{(i)}{\chi} $!image}%
\index{image!div@$\zdivtwo \circ \overset{(i)}{\chi}$}%
\begin{Proposition}
 \label{P14XI23.1}
For $k\ge 0 $ the image
{\rm 
%
$$
 \im_k  
 \big(\zdivtwo \circ \overset{(i)}{\chi}  \big)
 :=
 \im 
 \big(\zdivtwo \circ \overset{(i)}{\chi}\ofP|_{\MMHktwonp} \big)
$$
%
}is closed in $\MMHk$, and we have 
%
{\rm
$$
\im_k  
 \big(\zdivtwo \circ \overset{(i)}{\chi}  \big)
  = 
 \Big(
   \ker \Big(\big(\zdivtwo \circ \overset{(i)}{\chi}  \big)^\dagger 
   \Big)
   \Big)^\perp\cap \MMHk
   \,.
$$
% 
}  
\end{Proposition}

\proof
%
{\redca{19XI23.1} 
Let us for conciseness write $ \overset{(i)}{\chi} $ for $ \overset{(i)}{\chi} \ofP$. Set
%
$$ 
 \im_k  
   \overset{(i)}{\chi} 
 :=
 \im 
 \big( \overset{(i)}{\chi} |_{\MHktwonp} \big)
 \,.
$$
%
 The operator $\overadd{i}{\chi} |_{\MHktwonp}$, 
  of order $2n$, is elliptic and formally self-adjoint by Proposition~\ref{P18VIII23.1}.
By \eqref{6V23.1edxd} we have the $L^2$-orthogonal splitting
%
\begin{equation}
  \MHk =  (\ker\overset{(i)}{\chi} )^\dagger   \oplus  \im_k  
   \overset{(i)}{\chi} =  \ker\overset{(i)}{\chi}     \oplus  \im_k  
   \overset{(i)}{\chi} 
   \,,
   \label{19XI23.1}
\end{equation}   
%
with $\overadd{i}{\chi} |_{\MHktwonp}$ being an isomorphism from $ (\ker\overset{(i)}{\chi})^\perp \cap \MHktwonp$ to $ \im_k  
   \overset{(i)}{\chi}$.
    
Let $\psi_n \in \im \, \big(\zdivtwo \circ \overset{(i)}{\chi}|_{\MHktwonp}\big)$ be Cauchy in $\MHktwon$. 
%There exists a sequence $\phi_n \in \MHktwon$  such that $\psi_n = \zdivtwo \circ \overset{(i)}{\chi} $.   
Since the image of $\zdivtwo|_{\MHkp}$ is closed in $\MHk$ by Proposition~\ref{P30X22.1}, there exists a Cauchy sequence $\varphi_n\in  \MHkp$ such that $\psi_n = \zdivtwo \varphi_n$. In view of the splitting \eqref{19XI23.1} we can write, using obvious notation,
%
\begin{equation}\label{19XI23.2}
  \varphi_n = \varphi_n^{\ker} + \varphi_n^{\im}
  \,,
\end{equation}  
%
where both $\varphi_n^{\ker} $ and $ \varphi_n^{\im}$ are Cauchy. Since 
%
$$\overadd{i}{\chi} |_{\MHktwonp}: (\ker\overset{(i)}{\chi})^\perp \cap \MHktwonp\to \im_k  
   \overset{(i)}{\chi}$$ is  an isomorphism, there exists a Cauchy sequence  $\phi_n \in \MHktwonp$ such that $\varphi_n^\im =  \overset{(i)}{\chi} \phi_n $. Note that
   %
\begin{equation}
 (\zdivtwo \circ \overset{(i)}{\chi}) \phi_n = \zdivtwo \varphi_n^\im 
   = 
   \psi_n - \zdivtwo \varphi_n^{\ker}
   \,.
    \label{19XI23.3}
\end{equation}
   % 
   Since $\psi_n \in \im \, \big(\zdivtwo \circ \overset{(i)}{\chi}|_{\MHktwonp}\big)$
there exists a sequence $\hat \phi_n \in \MHktwon$  such that 
%
$$
 \psi_n = \zdivtwo \circ \overset{(i)}{\chi} \hat \phi_n 
 \,.
$$
%.
Comparing with  \eqref{19XI23.3} we find
\ptcr{so what? I am stuck}
%
\begin{equation}
\zdivtwo 
\big(\varphi_n^\im  - \overset{(i)}{\chi} \hat \phi_n 
   \big)
   = 
    - \zdivtwo \varphi_n^{\ker}
   \,.
    \label{19XI23.4}
\end{equation}
   % 




  
    Let $\phi=\lim_{n\to\infty} \phi_n$, then
% 
$$
\psi  : =  \lim_{n\to\infty} \psi_n = 
$$ 
% 
  \ptcr{not clear what next}
%
\qed
%
}   

==> divchiwrong.tex <==

\subsection{\protect\rm $\zdivtwo\circ\chi$}
 \label{ss12XI22.2}
\index{div@$\zdivtwo \circ \overset{(i)}{\chi}$}%
\index{div@$\zdivtwo \circ \overset{(i)}{\chi} $!image}%
\index{image!div@$\zdivtwo \circ \overset{(i)}{\chi}$}%
\begin{Proposition}
 \label{P14XI23.1}
For $k\ge 0 $ the image
{\rm 
%
$$
 \im_k  
 \big(\zdivtwo \circ \overset{(i)}{\chi}  \big)
 :=
 \im 
 \big(\zdivtwo \circ \overset{(i)}{\chi}\ofP|_{\MMHktwonp} \big)
$$
%
}is closed in $\MMHk$, and we have 
%
{\rm
$$
\im_k  
 \big(\zdivtwo \circ \overset{(i)}{\chi}  \big)
  = 
 \Big(
   \ker \Big(\big(\zdivtwo \circ \overset{(i)}{\chi}  \big)^\dagger 
   \Big)
   \Big)^\perp\cap \MMHk
   \,.
$$
% 
}  
\end{Proposition}

\proof
%
The principal symbol of   
%
$$
 \big(\zdivtwo \circ \overset{(i)}{\chi} \big)^\dagger
 \circ \big(\zdivtwo \circ \overset{(i)}{\chi} \big) 
$$
%
coincides with the principal symbol of  
%
$$
 (\overset{(i)}{\chi})^2 \circ \,  (\zdivtwo)^\dagger
 \circ  \zdivtwo 
 =  -  (\overset{(i)}{\chi})^2 \circ \,  C
 \circ  \zdivtwo 
 \,.
$$
%
Let us check that $  \mathfrak{L}:= C
 \circ  \zdivtwo $ is elliptic.
  \ptcr{is not}
  Denoting by $\sigma_{\mathfrak{L}}$ the symbol of ${\mathfrak{L}}$, for $0\ne k\in T^*(\dmanif)$ and for symmetric trace-free tensors $\chi$ we have
%
\begin{eqnarray*}
% \nonumber % Remove numbering (before each equation)
  \sigma_{\mathfrak{L}}(k)[\chi]_{AB} &=& \frac{1}{2}
  \Big(\k_A k_C \chi^C{}_B 
  +\k_B k_C  \chi^C{}_A 
  -\frac{2}{d}\k^C k^D  \chi_{CD}\ringh_{AB}  
   \Big) 
   \,.
\end{eqnarray*}
%
The equation $\sigma_{\mathfrak{L}}(k)[\chi]_{AB}k^A k^B =0$ gives, since $d\ne 1$,
%
\begin{eqnarray*} 
 \big (1-\frac{1}{d}\big) |k|^2 \k^C k^D  \chi_{CD}   =0
 \qquad
  \Longrightarrow 
  \qquad  
  \k^C k^D  \chi_{CD}   =0
   \,.
\end{eqnarray*}
%

 The operator $\overadd{i}{\chi} $, 
  of order $2n$, is elliptic by Proposition~\ref{P18VIII23.1}. 
  The result follows from  Lemma~\ref{L10xi23.1} with $A=\big(\zdivtwo \circ \overset{(i)}{\chi} \big)^\dagger$ and $B = 
 \zdivtwo \circ \overset{(i)}{\chi}$ . 
 %
 \qed
 % 

==> divtwoold.tex <==
\subsection{The conformal Killing operator}
 \label{App30X22}

 Consider the  \emph{conformal Killing operator} $C(\xi)$ on a closed $\ddim$-dimensional Riemannian manifold $(\dmanif,\dmetric)$:
 %
 \begin{equation}\label{30X22.CKV1a}
  \xi^A \mapsto  \dnabla _A \xi_B +  \dnabla _B \xi_A
    -  \frac 2 d   \dnabla ^C \xi_C
    \dmetric _{AB}
    =:  2  C(\xi)_{AB}
    \,,
 \end{equation}
 %
 where $\dnabla$ is the covariant derivative operator of the metric $\dmetric$.
 When invoking    $C(\xi)$ we will always assume implicitly that $\xi\in \HkdM$, for some $k\ge1$.


 Recall that: we use the symbol $\CKV$ to denote the space of conformal Killing vectors; $\TTt$ denotes the space of trace-free divergence-free symmetric two-tensors;  orthogonality is defined in $L^2$;  $\TS$ denotes the trace-free symmetric part of a two-tensor.

 We have:
  \ptchd{see conformally locally flat case \cite{Mars:2022qog}}

  \begin{Proposition}
   \label{P30X22.2}
   \begin{enumerate}
     \item
  There are no nontrivial Killing vectors or conformal Killing vectors on manifolds with negative Ricci tensor.
     \item On Ricci-flat manifolds all  conformal Killing vectors  are covariantly constant, hence Killing.
  \item
  \label{pP26II23.3}
   {\rm$\im (\zdivtwo C) = \CKVp$.} 
  \item For any vector field $\xi\in H^1(\dmanif)$ we have    $  C(\xi) ^{[ \TTt]} =0$.
   \end{enumerate}
  \end{Proposition}

  \proof
  %
1.\ and 2.:
%
Taking the divergence of the conformal Killing equation and commuting derivatives
leads to
 \ptcheck{20VI by
 wan}
 %
 \begin{equation}\label{30X22.CKV3}
    \dnabla ^A \dnabla _A \xi_B   + \zR_{BC} \xi^C
     + \frac{ \ddim-2 }{\ddim}\dnabla _B \dnabla^A \xi_A
    = 0
    \,.
 \end{equation}
 %
  Multiplying by $\xi^B$ and integrating over $\dmanif$ one finds
 %
 \begin{equation}\label{30X22.CKV4}
   \int ( | \dnabla   \xi|^2   + \frac{ \ddim-2 }{\ddim} |  \zdivone \xi |^2  -  \zR_{BC} \xi^B\xi^C)
    =  0
    \,.
 \end{equation}
 %
 If $\zR_{BC} \le 0$ we find that $\xi$ is covariantly constant, vanishing if  $\zR_{BC} < 0$.

 \medskip

 3.
 %
 %Let  $\eta$ be $L^2$-orthogonal to the   image of the elliptic operator $L:=\zdivtwo C$;  thus for any   covector field  $\xi$ we have
% %
% \begin{eqnarray}
%  0
%     &=&  \int_{\dmanif} \eta^A ( L\xi)_A   d\mu_{\dmetric}
%      \,.
% \end{eqnarray}
% %
% Equivalently, $\eta$ is a weak solution of the elliptic equation $L^\dagger \eta =0$. By elliptic regularity $\eta \in C^\infty$. We can therefore integrate by parts to obtain
% %
% \begin{eqnarray}
%  0
%     &=&  \int_{\dmanif} \eta^A  \dnabla _B(\dnabla _A \xi_B +  \dnabla _B \xi_A
%        -  \frac 2 d  \dnabla ^C \xi_C
%    \dmetric _{AB} ) d\mu_{\dmetric}
%    =2 \int_{\dmanif} \eta^A \dnabla ^B
%    \big( \TS (\dnabla _A \xi_B  )
%    \big)
%    d\mu_{\dmetric}
%     \nonumber
%\\
%     &=&
%      - 2 \int_{\dmanif} \dnabla^B \eta^A \TS (\dnabla _A \xi_B  ) d\mu_{\dmetric}
%      =
%      - 2 \int_{\dmanif} \TS (\dnabla^B \eta^A) \TS (\dnabla _A \xi_B  ) d\mu_{\dmetric}
%      \,.
% \end{eqnarray}
% %
% Setting  $\xi=\eta$ we conclude that $\eta$ is a conformal Killing vector.
The operator $L:=\zdivtwo C$ is elliptic and formally self-adjoint,  with 
 $\ker L = \CKV$, and 
 %
% %
% $$
%  \im (\zdivtwo C) ^\perp  = \CKV
%  \quad
%  \Longrightarrow
%  \quad  \CKVp = (\im (\zdivtwo C) ^\perp)^\perp
%   = \overline{(\im (\zdivtwo C)}
%   \,.
%   $$
% %
 we conclude by Proposition~\ref{P26X23.1}.

 \medskip


 4. The field  $  C(\xi) ^{[ \TTt]} $ is obtained by $L^2$-projecting  $  C(\xi)    $ on $\TTt$.
 So let $h\in L^2$ be a weak solution of the equation $\zdivtwo h=0$, i.e., for all $\xi \in H^1(\dmanif)$ we have
 %
 \begin{equation}\label{14VII23.1}
   \int_{\dmanif} \zspaceD^A\xi^B h_{AB} = 0
   \,,
 \end{equation}
 %
 which is precisely the statement that the $L^2$-projection  of $C(\xi ) $ on $\TTt$ vanishes.
 %Now, for any $h\in \TTt$ we have
%  \ptcr{there is a regularity problem here; the projection works well if all TT tensors are smooth, which is the case in two d, but not clear in higher dim; needs another look if used; but should work by density if xi is regular}
% %
% \begin{eqnarray}
%   \int_{\dmanif}  h^{AB}
%   C(\xi)_{AB}
%    \,
%    d\mu_{\dmetric}
%     &=&
%   \int_{\dmanif}  h^{AB}
%    \TS (\dnabla _A \xi_B  )
%    \,
%    d\mu_{\dmetric}
%    \nonumber
%\\
%     &=&
%     \int_{\dmanif} \TS (h^{AB})
%     \dnabla _A \xi_B
%    \,
%    d\mu_{\dmetric}  =
%     \int_{\dmanif}   h^{AB}
%     \dnabla _A \xi_B
%    \,
%    d\mu_{\dmetric}
%    \nonumber
%\\
% &    =
%  &
%   -    \int_{\dmanif} \underbrace{ \dnabla _A  h^{AB}}_0
%     \xi_B
%    \,
%    d\mu_{\dmetric}
%    =0
%      \,.
% \end{eqnarray}
% %
% Hence $  C(\xi) ^{[ \TTt]} =0 $.
% %
%%
%
 \qed
%  



\begin{Proposition}
 \label{P12XI22.1}
 The conformal Killing operator on $\ddim$-dimensional compact manifolds, $d\ge 3$, has the following properties:

 \begin{enumerate}
   \item $ \ddim (\ddim+1)/2$ dimensional kernel  on $S^d$ with the canonical metric;
   \item $\ddim$-dimensional kernel  on flat manifolds;
   \item no kernel  on negatively Ricci-curved
    manifolds.
 \end{enumerate}
 \end{Proposition}

 \proof
 %
 1. The conformal group of a $\ddim$-dimensional sphere is the same as the Lorentz group in $\ddim+2$ dimensions.

 The statements about the kernel in points 2.\ and 3.\ follow from   Proposition \ref{P30X22.2}.
 %
 \qedskip
 %
 
 
We note the following properties of conformal Killing vectors on Einstein manifolds, which will be needed in what follows:


 \input{LemmaCKV}

 \input{LemmaCKV2}



\medskip

 
\input{CKV}

\input{divtwo}

==> dukappa.tex <==
\section{Integral formulae for $\partial_u^i \Hf_{uA}$ and $\partial_u^i h_{AB}$}
\wc{perhaps not needed; replaced by App \ref{App6III23.1} below}

First, we obtain expressions for
%
\begin{align}
    \partial_u\int_{r_1}^r s^k h_{AB}\ ds
\end{align}
%
as needed for integral formulae of higher $u$-derivatives of metric functions in the main text.

From \eqref{3IX22.1HD} we have,
%
\begin{align}
    \partial_u h_{AB}
    &=
    \tkfbd
    + \frac{n-5}{4r^2}V h_{AB}
    + \frac{V}{2r} \partial_r h_{AB}
    \nonumber
\\
    &\quad
    + \frac{n-1}{8} r^{\frac{5-n}{2}} \int_{r_1}^r
     \left( \alpha ^2 (n+1) s^{\frac{n-5}{2}}
   - (n-3) \myGauss  s^{\frac{n-9}{2}}
   - 2 m (n-1)  s^{-\frac{n+5}{2}}
   \right) h_{AB}
   \ ds
   \nonumber
\\
    &\quad
     + \int_{r_1}^r
     \bigg(\frac{2 (n-1) r^{2-n} s^{n-4}}{n (n+1)}+\frac{(n-3) r^{\frac{5-n}{2}} s^{\frac{n-9}{2}}}{n+1}+\frac{2 r^2}{n s^4} \bigg) \ P(h)_{AB}
    \, ds
\nonumber
\\
    &\quad
     - r^{\frac{5-n}{2}} \int_{r_1}^r s^{\frac{n-9}{2}}
     \bigg( - \frac{1}{2} \TSzlap h_{AB} + P(h)_{AB} - \red{\tric(h)}_{AB} \bigg)
    \, ds
    \,.
    \label{15XII22.1a}
    \end{align}
%
\subsection{$\alpha = 0= m$}

For $k\neq -3, n-3, (n-7)/2$, we have
%
\begin{align}
     \int_{r_1}^r s^k \partial_u h_{AB} ds
&=
    \tkfbd
    +
    \int_{r_1}^r s^k
    \bigg(\frac{n-5}{4s^2}V h_{AB}
    + \frac{V}{2s} \partial_s h_{AB}\bigg)
    ds
    \nonumber
\\
    &\quad
     +
    \int_{r_1}^r s^k  \int_{r_1}^s \bigg[
     \bigg(\frac{(n-3) s^{\frac{5-n}{2}}}{n+1} P - (n-3)\frac{n-1}{8} s^{\frac{5-n}{2}}  \myGauss  \bigg) y^{\frac{n-9}{2}} h_{AB}|_{s}
     \nonumber
\\
    &\phantom{\quad\quad
     +
    \int_{r_1}^r s^k  \int_{r_1}^s }
    %
    + \bigg(\frac{2 (n-1) s^{2-n} y^{n-4}}{n (n+1)}+\frac{2 s^2}{n y^4} \bigg) \ P(h)_{AB}|_{y}\bigg] \ dy  \ ds
    \nonumber
\\
&=
    \tkfbd
    +
    \bigg[ \frac{V s^{k-1}}{2} h_{AB}|_{s} \bigg]_{r_1}^r
    +
    \int_{r_1}^r
    \bigg(\frac{n-5}{4}V s^{k-2}   - \partial_s \bigg(\frac{V s^{k-1}}{2}\bigg)
    \bigg)h_{AB}|_{s}
    ds
    \nonumber
\\
    &\quad
     +
    \int_{r_1}^r\int_{r_1}^s \bigg[
     \bigg(\frac{(n-3) s^{k+\frac{5-n}{2}}}{n+1} P - (n-3)\frac{n-1}{8} s^{k + \frac{5-n}{2}}  \myGauss  \bigg) y^{\frac{n-9}{2}} h_{AB}|_{y}
     \nonumber
\\
    &\phantom{\quad+\int_{r_1}^r s^k  \int_{r_1}^s }
    %
    + \bigg(\frac{2 (n-1) s^{k + 2-n} y^{n-4}}{n (n+1)}+\frac{2 s^{k+2}}{n y^4} \bigg) \ \red{P(h)}_{AB}|_{y} \bigg] \ dy \ ds
    \nonumber
\\
&=
    \tkfbd
    +
    \bigg[ \frac{V s^{k-1}}{2} h_{AB} \bigg]_{r_1}^r
    +
    \int_{r_1}^r
    \bigg(\frac{n-5}{4}V s^{k-2}   - \partial_s \bigg(\frac{V s^{k-1}}{2}\bigg)
    \bigg)h_{AB}|_{s}
    ds
    \nonumber
\\
    &\quad
     +
    \int_{r_1}^r\int_{s}^r  \bigg[
     \frac{n-3}{n+1}y^{k+\frac{5-n}{2}}\bigg( P - \frac{(n-1)(n+1)}{8}  \myGauss  \bigg) s^{\frac{n-9}{2}} h_{AB}|_{s}
     \nonumber
\\
    &\phantom{\quad
     +
    \int_{r_1}^r s^k  \int_{r_1}^s }
    %
    + \bigg(\frac{2 (n-1) y^{k + 2-n} s^{n-4}}{n (n+1)}+\frac{2 y^{k+2}}{n s^4} \bigg) \ \red{P(h)}_{AB}|_{s}
    \bigg] dy \ ds
    \nonumber
\\
&=
    \tkfbd
    +
    \bigg[ \frac{V s^{k-1}}{2} h_{AB} \bigg]_{r_1}^r
    +
   \int_{r_1}^r \bigg(\frac{2  r^{3 + k}}{(3  + k ) n s^4} + \frac{2 (n - 1)  r^{3 + k-n} s^{n-4}}{(3 + k -  n) n (1 + n) }\bigg) \red{P(h)}_{AB} \ ds
    \nonumber
\\
    &\quad
    -  \int_{r_1}^r\frac{(2 + k) (4 + k -  n) }{(3 + k) (3 + k -  n) (7 + 2 k -  n) } \bigl(  (3 + k) (3 + k -  n) \myGauss + 2 P\bigr)s^{k-1} \ h_{AB}  \ ds
    \nonumber
    \\
    &\quad
    + \int_{r_1}^r \frac{(n - 3) r^{-(n-7)/2 + k}  }{4 (7 + 2 k -  n) (1 + n) }(8 P + \myGauss -  n^2 \myGauss)s^{(n-9)/2} h_{AB}\ ds
    \label{1III23.2}
\end{align}
%

\subsection{$\partial_u^i\Hf_{uA}$}

We begin with the integral equation \eqref{21II23.2},
%
\begin{align}
    \Hf_{uA}|_r = \Hf_{uA}|_{r_1} +
    \int_{r_1}^r \frac{3}{s^4}  \zspaceD^B h_{AB} \ ds\,.
    \label{1III23.3}
\end{align}
%

By making use of \eqref{1III23.2} recursively, we arrive at the general form of $\partial^i_u\Hf_{uA}$ in \eqref{28II23.4b} of the main text:
 \ptcr{crossref}
%
\begin{align}
    \partial_u^i \Hf_{uA} &=
    \overadd{i}{X}[r,r_1, h_{\mu\nu}|_{r_1}, h_{\mu\nu}|_{r}]
    + \sum_{j=0}^i \int_{r_1}^r \overadd{i,j}{\chi}_{-4}(r,P) s^{-4-j} h_{AB} \ ds
    \nonumber
\\
    & \quad
    + \int_{r_1}^r \bigg[\overadd{i,n-4}{\chi}(r,P) s^{n-4}
    + \sum_{j=0}^{i} \overadd{i,j}{\chi}_{(n-9)/2}(r,P) s^{(n-9)/2-j}\bigg] h_{AB} \ ds \,.
\end{align}
%
We can read off $\overadd{0}{X}$ and the only non-zero $\overadd{0,j}{\chi}_k$ from \eqref{1III23.3}:
%
\begin{align}
    \overadd{0}{X} = \Hf_{uA}|_{r_1} \,, \quad \overadd{0,0}{\chi}_{-4}=3\,.
\end{align}
%

% For the purpose of characteristic gluing, we are mainly interested in the kernel of the operator $\overset{(i,i)}{\chi}_{-4}(r,P)$. It follows from \eqref{1III23.2} that
% %
% \begin{align}
%     \overadd{i+1,i+1}{\chi}_{-4}(r,P) &= K_i \bigl(  (3 - (i+4) ) (3 - (i+4) -  n) \myGauss + 2 P\bigr) \overadd{i,i}{\chi}_{-4}(r,P)
%     \nonumber
%     \\
%     &= K_i \bigl(  ( i + 1 ) (i+1+n) \myGauss + 2 P\bigr) \overadd{i,i}{\chi}_{-4}(r,P)
%     \\
%     K_i & = - \frac{(2 - (4+i)) (4 - (4+i) -  n) }{(3 - (4+i)) (3 - (4+i) -  n) (7 - 2(4+i) -  n) }
%     \nonumber
%     \\
%     & = \frac{(2 + i) (i +  n) }{(1+i)) ( i +  n+1) (n+2i) }\,.
% \end{align}
% %
% In particular, we have
% \begin{equation}
%     \ker\left(\overadd{i+1,i+1}{\chi}_{-4}(r,P)\right) = \ker\left(\overadd{i,i}{\chi}_{-4}(r,P)\right) \cup \ker\bigl(  ( i + 1 ) (i+1+n) \myGauss + 2 P\bigr) \,.
%     \label{1III23.4}
% \end{equation}


% On $S^{n-1}$, the spectrum of the operator $P$ is given by $-\frac{1}{2}(\ell-1)(\ell+n-1)$, $\ell \in \{0,1,2,...\}$ from \eqref{1III23.6}
% \wcb{to be checked; other topologies to be added; maybe section to be moved to after analysis of P}
% . Hence $\ker\bigl(  ( i + 1 ) (i+1+n)  + 2 P\bigr)$ is spanned by spherical harmonic tensors
% with mode $\ell$ satisfying
% %
% \begin{align}
% \bigl(  ( i + 1 ) (i+1+n)  -(\ell-1)(\ell+n-1) \bigr) = 0 \,,
% \end{align}
% %
% which admits the positive solution $\ell = i+2$. Since $\ker\left(\overadd{0,0}{\chi}_{-4}(r,P)\right) = 0$, it follows recursively from \eqref{1III23.4} that $\ker\left(\overadd{i,i}{\chi}_{-4}(r,P)\right)$ is spanned by spherical harmonic tensors with $\ell = 2,...,i+1$. 

==> end2.tex <==
%\backmatter
%\bibliographystyle{/usr/local/lib/texmf/bibtex/bst/amsplain}
%\bibliography{$HOME/prace/references/hip_bib,%
%$HOME/prace/references/reffile,%
%$HOME/prace/references/vienna,%
%$HOME/prace/references/newbiblio,%
%$HOME/prace/references/newbiblio2,%
%$HOME/prace/references/netbiblio,%
%$HOME/prace/references/bibl,%
%$HOME/prace/references/howard}
\bibliographystyle{JHEP}
%\bibliographystyle{amsplain}
\bibliography{../../../references/hip_bib,%
../../../references/reffile,%
../../../references/newbiblio4,%
../../../references/newbiblio,%
../../../references/newbiblio2,%
../../../references/besse2,%
../../../references/bibl,%
../../../references/howard,%
../../../references/bartnik,%
../../../references/myGR,%
../../../references/newbib,%
../../../references/Energy,%
../../../references/chrusciel,%
../../../references/dp-BAMS,%
../../../references/prop2,%
../../../references/netbiblio,%
../../../references/besse}
\end{document}


==> kappsWithLogs.tex <==
\input{HDkappas}
{\blueca{16viii22; log terms added; need to think this through}

When $n$ is odd the construction is marginally more involved. This is due to the fact that for $j<i$  the functions $\overset{(i,j)}{\psi}(s,r)$ and $\overset{(i,j)}{\chi}(s,r)$ are not polynomials in $1/s$ anymore, but are instead linear combinations of $s^k \ln ^\ell s$, $\Z\ni k \ge - (i+3)$, $\ell \in \N$, with coefficients which depend upon $r$. However, the key functions used for the gluing, namely $\overset{(i,i)}{\psi}(s,r)$ and $\overset{(i,i)}{\chi}(s,r)$ are independent of $\alpha$, and thus identical to the case $\alpha =0$.
 \ptcr{chi?}
We also note that the $\ln s$ terms appear only for $i\ge 3$.

The functions $\kappa_i$ are now constructed recursively as follows: \green{For $-2\leq i \leq 0$, let $\hkappa_i:=s^i$.} For $i\ge 1$ let $\{\hat \kappa_k\}_{k \le N_i}$ denote the minimal collection of functions
$s^k \ln ^\ell s$ so that the functions $\overset{(\ell,m)}{\psi}(s,r)$ and $\overset{(\green{\ell-1},m)}{\chi}(s,r)$ with $\ell\le i$ are linear combinations of the $\hat\kappa_k$. We order them so that the collection $\{\hat\kappa_k\}_{k \le N_i}$ are the first functions in $\{\hat\kappa_k\}_{k \le N_{i+1}}$, with
 \ptc{I still need to understand the $\chi$'s to write it right}
 $\hat\kappa_{N_i}= s^{-(i+3)}$.

We let the collection $\{f_k\}$ be obtained by a Gram -Schmidt orthonormalisation of    $\{\hat\kappa_k\}$, with respect to the scalar product  in the space $\mathbb{H}$ above. We set
%
$$   \red{\kappa}_i  = c_i \red{\chi} f_{N_i}
 \,,
$$
%
with a suitably chosen constant $c_i\ne 0$, so that the functions so-defined satisfy
%
\begin{eqnarray}
  &
  \displaystyle
\ip{\kappa_i}{\hat \kappa_j}  = 0
 \quad \mbox{for $j<N_i$}
  \,,
  &
  \label{13VIII22.1c}
   \\
   &
  \displaystyle
 \ip{\kappa_i}{\hat \kappa_{N_i}}  = 1
  \,.
  &
  \label{13VIII22.2c}
\end{eqnarray}
%
} 

==> nullWithr.tex <==
\ptc{ the case with nu A not zero in nullGeneral.tex, but not finished and probably not needed}
%The first step is to work-out the differentiability properties of $\mtdu$ and $\mtdx^A$ in the $r$-direction.
For this consider on $\secNtwoNew$ 
 \ptcr{if I had it everywhere I wouldn't have to consider it on $\zsecN$}
%
%%
%\begin{equation}\label{17VII23.1b}
%  \zsecN=
% %  \{\mtdu=0\}\cap \{\mtdr=r_2\}
%%   \equiv
%   \{\zu=0\}\cap \{r=r_2\}
%   \,,
%\end{equation}
%%
the field 
%
\begin{equation}\label{30III24.10}
 \zell= \partial_r + \zell^u \partial_u + \zell^A\partial_A
\end{equation}
 %
 of null normals  to the level sets of $\zu$. 
  Let  
$\mtdl$ be a field of null tangents to $\{\mtdu=0\}$ which coincides with $\zell$ on $\zsecN$.
Since  $\mtdu$ and $\mtdx^A$ are constant along the integral curves of $\mtdl$,  we have  $\mtdl(\mtdu)  =0=\mtdl(\mtdx^A) $. 
Hence
\wcb{RHS: $\zu \rightarrow \mtdu$?}
%
\begin{equation}\label{14IX23.1a}
  \partial_r \mtdu 
    = -
  (\mtdl^u \partial_u \zu + \mtdl^A
  \partial_A \zu)   
  \,,
\end{equation}
%
with an analogous formula for $\partial_r \mtdx^B$:
 \ptcr{needs adding a x A shift, here or elsewhere}
%
\begin{equation}\label{14IX23.1b}
  \partial_r \mtdx^B  = -
  (\mtdl^u \partial_u \mtdx^B
   + \mtdl^A
  \partial_A\mtdx^B
  )  
 %  =  |_\zsecN -
%  \zell^B
  \,,
\end{equation}
%


The components of $\mtdl$ can be calculated as follows. As $\mtdl$ is null
 we must have $\fourg_2(\mtdl,\mtdl)=0$, namely
%
\begin{equation}
    0= \alpha (\mtdl^u)^2 +2 \mtdl^u  \red{e^{2\beta}}   - g_{AB} \mtdl^A \mtdl^B
     \,.
     \label{9IX23.1}
\end{equation}
%
\ptcr{changes on 8IV24 from now on}
%Equivalently, after choosing the positive solution,
%%
%\begin{equation}
% \mtdl^u  =
%   \frac{- \red{e^{2\beta}} + \sqrt{\red{e^{4\beta}}+  \alpha g_{AB} \mtdl^A \mtdl^B}}\alpha
%     \,.
%     \label{9IX23.1}
%\end{equation}
%%
Next, let $X=X^u \partial_u + X^r \partial_r+ X^A \partial_A$ be tangent to a level set of $\mtdu$, thus 
 \ptcr{r component added}
%
\begin{equation}\label{8IV24.7}
 0=X(\mtdu)= X^u \partial_u\mtdu+ X^r \partial_r\mtdu+ X^A \partial_A\mtdu
 \quad
 \Longrightarrow
 \quad
  X^u= - 
   \frac{X^r \partial_r \mtdu + X^A \partial_A\mtdu}{\partial_u\mtdu}
  \,.
\end{equation}
%  }
Let $\cHtwo$ be the hypersurface defined by the cross-section function $\fr(x^A)$ of \eqrefl{30III24.1}:
%
\begin{equation}\label{8IV24.1}
  \cHtwo = \{r=\fr(x^A)
  \,, \ x^A \in \secN\,,
  \ u\in \R
  \}
  \,.
\end{equation}
%
Equation~\eqref{8IV24.7} shows that vector field $X$ which is both tangent  to the level sets of $\mtdu$ and to $\cHtwo$
 takes  the form, using \eqref{14IX23.1a},
%
\begin{eqnarray}
 \label{8IV24.3}
 X 
  & = & 
   X^A
   \big( 
    \partial_A  
   + \red{\partial_A\fr}  \partial_r   
   -
  %\underbrace{
    \frac{\red{\partial_A\fr} \partial_r \mtdu + \partial_A\mtdu}{\partial_u\mtdu} 
    % }_{=:\lowX_A}
   \partial_u 
   \big)
   \nonumber
\\    
  & = & 
   X^A
   \big( 
    \partial_A  
   +\red{\partial_A\fr}  \partial_r   
   +
  \underbrace{
    \frac{\red{\partial_A\fr}
  (\mtdl^u \partial_u \zu + \mtdl^B
  \partial_B \zu )    
  - \partial_A\mtdu}{\partial_u\mtdu} 
     }_{=:\lowX_A}
   \partial_u 
   \big)
  \,.
\end{eqnarray}
%
Since  $\mtdl$ is orthogonal to the level sets of $\mtdu$, 
on $\cHtwo$ for such $X$ we have
%
\begin{eqnarray}
  0 
  &=& \fourg(\partial_r + \mtdl^u \partial_u + \mtdl^A\partial_A
   ,X^u\partial_u + X^r\partial_r
   +X^B\partial_B
  )
     \nonumber
\\ 
 &=&
   - \red{e^{2\beta}} X^u  
   - \mtdl^u (\alpha X^u   + \red{e^{2\beta}} X^r  
   )   + g_{AB}  \mtdl^A X^B
     \nonumber
\\
    &=&
    \big(- 
     \red{e^{2\beta}}  \lowX_B  
     - \mtdl^u
     (
       \alpha   \lowX_B   
       +   \red{e^{2\beta}}\red{\partial_B\fr}  
       )
       + \mtdl^A  g_{AB}
       \big) X^B
 \,.
  \label{9IX23.4}
\end{eqnarray} 
%%
%{\bluec \ptc{old}
%%
%\begin{eqnarray}
%     \nonumber
%  0 &=& \fourg(\partial_r + \mtdl^u \partial_u + \mtdl^B\partial_B
%   ,\partial_A -    \frac{\partial_A\zu}{\partial_u\zu } \partial_u
%  )
%\\
%    &=&
%     \red{e^{2\beta}}     \frac{\partial_A\zu}{\partial_u\zu }
%     +\mtdl^u \alpha     \frac{\partial_A\zu}{\partial_u\zu }
%       + \mtdl^B  g_{AB}
% \,.
%  \label{9IX23.4}
%\end{eqnarray} 
%%
%}
Since $X^B$ is arbitrary we find
%
%
\begin{eqnarray}
        \mtdl^C |_{ \cHtwo }
        &=& 
        \inv^{AC}
        \big(
    (
     \red{e^{2\beta}}
        + \mtdl^u \alpha
        )     \lambda_A 
        +  \red{e^{2\beta}}\mtdl^u \red{\partial_A\fr}   
         \big)
         \nonumber
 \\         
        &=& 
        \inv^{AC}
        \big(
    (
     \red{e^{2\beta}}
        + \mtdl^u \alpha
        )       \frac{\red{\partial_A\fr}
  (\mtdl^u \partial_u \zu + \mtdl^B
  \partial_B \zu )    
 - \partial_A\mtdu}{\partial_u\mtdu} 
        +  \red{e^{2\beta}}\mtdl^u \red{\partial_A\fr}      
         \big)
 \,.
  \label{9IX23.8b}
\end{eqnarray}  
%
Multiplying by $\partial_C\zu$ we obtain
%
\begin{align}
   \big( 1  -  
    &   
  \frac{  (  \red{e^{2\beta}}
        + \mtdl^u \alpha)
        g^{AB}\partial_A\zr\partial_B\zu
        }{\partial_u\mtdu}  
        \big)
            \mtdl^C \partial_C\zu |_{ \cHtwo }
        \nonumber
\\
 &         =
        \inv^{AC}
        \big(
    (
     \red{e^{2\beta}}
        + \mtdl^u \alpha
        )       \frac{
  \mtdl^u \partial_u \zu  \red{\partial_A\fr}
  - \partial_A\mtdu}{\partial_u\mtdu} +   \red{e^{2\beta}}\cell \red{\partial_A\fr}   
         \big)\partial_C\zu
 \,.
  \label{9IX23.8}
\end{align}  
%
Equivalently, assuming that the denominator does not vanish, which will be the case for small $\partial_A\zu$,
%
\begin{align}
            \mtdl^C \partial_C\zu |_{ \cHtwo } 
 &         =
 \frac{
        \inv^{AC}
        \big(
    (
     \red{e^{2\beta}}
        + \mtdl^u \alpha
        )       \frac{
  \mtdl^u \partial_u \zu  \red{\partial_A\fr}
  - \partial_A\mtdu}{\partial_u\mtdu} +   \red{e^{2\beta}}\cell \red{\partial_A\fr}   
         \big)\partial_C\zu
         }{ 
         1  -   
  \frac{  (  \red{e^{2\beta}}
        + \mtdl^u \alpha)
        g^{AB}\partial_A\zr\partial_B\zu
        }{\partial_u\mtdu}   
        }
 \,.
  \label{9IV24.1}
\end{align}  
%
This can be inserted into the right-hand side of \eqref{9IX23.8} to determine $\mtdl^A$ in terms of $\mtdl^u$. Inserting the result into \eqref{9IX23.1} gives an equation 
which determines now $\mtdl^u$ on $\cHtwo$  as 
{\redca{10IV}
a smooth function of  the remaining data when $(\fr,\zu)$ are near $(r_2,0)$.
 Inserting the result into \eqref{9IV24.1} gives the component of $\mtdl^A$ along $\partial_A \zu$. Using this in \eqref{9IX23.8b} gives $\mtdl^A$ in terms of the remaining data. We conclude that the components of $\mtdl$ are smooth functions of remaining data with
 %
 \begin{equation}
  \mtdl^\mu|_{\cHtwo}\in 
  H_{k_\gamma-1}
   ????
  \,.
\end{equation}
%  


}
%
%using \eqref{9IX23.1}:
%%
%\begin{equation}\label{30III24.10xd}
% \mtdl|_{ \cHtwo }= \partial_r + 
%   \frac{- \red{e^{2\beta}} + \sqrt{\red{e^{4\beta}}+  \alpha g_{AB} \mtdl^A \mtdl^B}}\alpha
%  \partial_u +  \mtdl^A\partial_A
%  \,.
%\end{equation}
% %




\ptc{some stuff went to recycling.tex}
 \reject


==> operators.tex <==
\subsection{$P$}
 \label{ss19XI22.1}

Consider the operator
%
\begin{align}
 \label{11XI22.2}
 P(h)_{AB} := \TS[\zspaceD_A \zspaceD^C h_{BC}]
    \,.
\end{align}
%
of \eqref{11XI22.1}. where $h$ is symmetric and $\zgamma$-traceless.
 \ptcr{already analysed on Sd; and this looks like 2d to me so far}


We have:

\begin{Proposition}
 \label{P12XI22.2}
 The   operator $P$ is elliptic, self-adjoint and negative, with
 \begin{enumerate}
   \item six-dimensional cokernel and   kernel on $S^2$;
   \item two-dimensional kernel and cokernel on $\T^2$;
   \item   $6(\genus-1)$-dimensional cokernel and  kernel on manifolds of genus $\genus\ge 2$.
 \end{enumerate}
 \end{Proposition}

\proof
%
Note that
%
\begin{equation}\label{27XI22.11}
  P = C \circ \zdivtwo
\end{equation}
%
is a composition of elliptic operators, hence is elliptic.
Using
%
\begin{equation}\label{30XI22a}
  \zdivtwo\!\!^\dagger = - C
  \,,
  \quad
  C^\dagger = - \zdivtwo
  \,,
\end{equation}
%
we have
%
\begin{equation}\label{30XI22}
  P = - \zdivtwo \!\!^\dagger \circ \zdivtwo
  \,,
\end{equation}
%
from which self-adjointness  follows.

Finally, we have
%
\begin{equation}\label{30XI22-11}
   \int h^{AB}Ph _{AB}
   = -  \int h \,  \zdivtwo \!\!^\dagger \circ \zdivtwo h
   =  - \int |\zdivtwo h |^2 \le 0
   \,,
\end{equation}
%
hence all eigenvalues of $P$ are negative, and $Ph=0$ implies
$\zdivtwo h=0$.
%, and the result follows by e.g.\  \cite{Tromba}, see the   paragraph after Theorem~8.2 there.
%
\qed
%






==> orderkkernel.tex <==
\subsubsection{Polynomials in $P$}
 \label{ss27XI22.1}

In this section we assume that $m=0$.

For $C^k$-gluing, the operator $\sum_{i=0}^{k}  \overset{(k,i)}{\ochi}_{k+4}  P^i $ appearing in \eqref{24X22.91} is of the form
%
\begin{align}
   \sum_{i=0}^{k}  \overset{(k,i)}{\ochi}_{k+4} (r_2)  P^i
   =
    \blue{\hat c_k}\prod_{i=1}^k (P+\twoscsign a_i )\,,\qquad
   a_i = \frac{1}{2}i(3+i)\,,
   \label{26X22.w1}
 \end{align}
%
where
 \ptcheck{28X}
%
$$\blue{\hat c_k}
= \frac{1}{ k!(k+3)}
\,.
$$
%
This can be verified by induction.

Indeed, when  $k=1$ this follows from \eqref{25XI22.3}-\eqref{25XI22.6} with $\hat c_1=1/4$. Using the recursion formula \eqref{16VIII22.12},
a straightforward calculation shows that the $\hkappa_{k+5}$ component of the $(k+1)$-order coefficient  are  given by
\ptcheck{27X22, and with $\myGauss$ and m=0 on 30XI}
%
\begin{equation}
    \overset{(k+1,i)}{\ochi}_{k+5} = \blue{c_k} \times \left\{
       \begin{array}{lll}
        \twoscsign a_{k+1} \overset{(k ,0)}{\ochi}_{k+4}\,,
          & \hbox{$i=0$}
           \,,
        \\[5pt]
          \twoscsign  a_{k+1} \overset{(k ,i)}{\ochi}_{k+4}  + \overset{(k,i-1)}{\ochi}_{k+4}\,,
           &  \hbox{$1\leq i \leq k$}
            \,,
        \\[5pt]
        \overset{(k ,k)}{\ochi}_{k+4}\,,
          &  \hbox{$i = k+1$}
           \,,
       \end{array}
     \right.
\end{equation}
%
with $\blue{c_k} = \frac{k+3}{(k+4)(k+1)}$. Therefore, assuming \eqref{26X22.w1}, the operator at order $k+1$ is actually $r_2$-independent and reads,
\ptcheck{27X22}
%
\begin{align}
    \sum_{i=0}^{k+1}  \overset{(k,i)}{\ochi}_{k+5} (r_2)  P^i
   &= \blue{c_k} \sum_{i=0}^{k}  \left(\overset{(k,i)}{\ochi}_{k+4}   P^{i+1}
   +
   \twoscsign a_{k+1}  \overset{(k,i)}{\ochi}_{k+4}   P^i \right)
   \nonumber
   \\
   &=
   \blue{c_k} \sum_{i=0}^{k}  \big(\overset{(k,i)}{\ochi}_{k+4}   P^{i} \big) (P+ \twoscsign a_{k+1}  )
      \nonumber
   \\
   &=
    \blue{c_k} \hat c_k  (P+ \twoscsign a_{k+1} ) \prod_{i=1}^k  (P+ \twoscsign a_i )
   \nonumber
   \\
    &=
    \blue{ \hat c_{k+1}}  \prod_{i=1}^{k+1} (P+\twoscsign a_i )\,,
    \qquad \text{with} \ \blue{\hat c_{k+1}}=  \blue{c_k} \hat c_k
    \,.
\end{align}
%
It thus follows from \eqref{26X22.w3} that, on $S^2$, spherical harmonic vector fields with mode $\ell\ge 0 $ satisfying
%
\begin{align}
    0&=\prod_{i=1}^{k} \left(-\frac{1}{2}\ell(\ell+1)+ 1 + a_i\right)
    =
    \frac{1}{2} \prod_{i=1}^{k} (1+i-\ell)(2+i+\ell)
\end{align}
%
  belong to $\ker\left(\sum_{i=0}^{k}  \overset{(k,i)}{\ochi}_{k+4}  P^i \right)$. The corresponding values of $\ell$ are  $\ell = 2,...,k+1$.
 \ptcheck{27X}
 
For the remaining topologies, each of the operators
%
$$
 P + \myGauss a_i
$$
%
appearing in \eqref{26X22.w1} is negative.
On $\T^2$ its kernel, when acting on traceless tensors, is two-dimensional, consisting of covariantly constant tensors. Hence, in the toroidal case, the kernel of the left-hand side of \eqref{26X22.w1} is also two-dimensional, which can be seen e.g.\ by a Fourier-series decomposition.

On higher genus manifolds  $P + \myGauss a_i$ is strictly negative and therefore has no kernel. Hence so does the left-hand side of \eqref{26X22.w1}.
%
%\wcb{Added 29XI. $\lambda^2 \in \N$ on $\T^2$??} For other topologies, we have analogously, that harmonic tensor fields $\varphi^{[\lambda]}$ with mode $\lambda$ (i.e., $\varphi^{[\lambda]}:= -1/\sqrt{1/2 \lambda^2 - \twoscsign} \, C(E^{[\lambda]})$, $E^{[\lambda]} := -1/\sqrt{\lambda^2} \zspaceD_A Y^{[\lambda]}$, where $\dDelta Y^{[\lambda]} = -\lambda^2 Y^{[\lambda]}$; $P \varphi^{[\lambda]} = (\twoscsign -1/2 \lambda^2)\varphi^{[\lambda]}$) satisfying \wcb{Not sure if there are more, e.g. from ''harmonic one forms'' on negatively curved sections}
%%
%\begin{align}
%    0&=\prod_{i=1}^{k} \left(-\frac{1}{2}\lambda^2 + \twoscsign + a_i\right)
%\end{align}
%%
%belong to $\ker\left(\sum_{i=0}^{k}  \overset{(k,i)}{\ochi}_{k+4}  P^i \right)$.
%}


==> psiMapOld.tex <==
\subsection{\protect\rm $\psi$} 
 \label{ss12XI22.2n}
 
 
 
\ptclater{LemmaClosed.tex can streamline several arguments above ...}
%\reject
\input{LemmaClosed}
%\reject

\index{psi@$\overset{(i)}{\psi}$}% 
\index{image!psi@$\overset{(i)}{\psi}$}%
\begin{Proposition}
 \label{P14XI23.1psi}
For $k\ge 1$ the image
{\rm
%
$$
 \im_k 
 \overset{(i)}{\psi}  
 :=
 \im
 \big( \overset{(i)}{\psi}\ofP|_{\MMHktwoi} \big)
$$
%
}is closed in $\MMHk$, and we have
%
{\rm
\begin{eqnarray}
 \im_k
 \overset{(i)}{\psi}  
   &= &
 \big(
   \ker   
 \overset{(i)}{\psi}   
   \big)^\perp\cap \MMHk 
   \,.
    \label{9XII23.31}
\end{eqnarray}
%
}
\end{Proposition}

\proof
%
We start by noting that the operators $\overset{(i)}{\psi}\ofP $ are formally self-adjoint, of order $2i$.
When $i < \frac{n-3}{2}$, or when the pair $(n,\ell)$ is convenient and $i\in \N$,  the  $\overset{(i)}{\psi}\ofP $'s are elliptic by Propositions~\ref{P22VIII23.1} and \ref{P17X23.1} below.
Our claim follows from  Proposition~\ref{P26X23.1}.

To continue, let the pair $(n,\ell)$  be inconvenient and $i> \frac{n-3}{2}$. Consider the operators 
%
\begin{align}
	{\cal L}_{\TTt} (j) 
  &:=  -\frac{1}{(7 - n + 2 j)}\left( \zTSlap_T+ [4+j(6-n+j)]\myGauss\right) 
\,,
\\
 \overset{(i)}{\psi}_{\TTt}
 & :=  \prod_{j=2}^{i} {\cal L}_{\TTt}(\tfrac{n-5-2j}{2})\overset{(1)}{\psi}\ofP 
 \,,
\end{align}
%
where%
\index{Delta@$\zTSlap_T$}%
%
\begin{equation}
	\zTSlap_T h\equiv\left[\TSzlap+2(\tric-(n-2)\myGauss)\right]h
  \,.
\label{8XII23.g6}
\end{equation}
%
{\redca{20XII}
The operators $\overset{(i)}{\psi}_{\TTt}$ are  elliptic, formally self adjoint, and therefore have closed image and finite dimensional kernel. This 
is accompanied with the $L^2$-orthogonal splitting
\ptcr{notation Sk and Vk perhaps not consistent}
%
\begin{equation}\label{20XII23.1}
  \MMHk= \ker \overset{(i)}{\psi}_{\TTt} \oplus
    \im \big(
   \overset{(i)}{\psi}_{\TTt}|_{\MHktwoi}\big) 
  \,.
\end{equation}
%
Let (compare Section~\ref{ss8IX23.1} below)
%
\begin{eqnarray}
% \nonumber % Remove numbering (before each equation)
 &\TTt^{k+2i} := \TTt\cap( \ker \overset{(i)}{\psi}_{\TTt})^\perp\cap\MHktwoi
    \,,
    \ V^{k+2i} := V\cap( \ker \overset{(i)}{\psi}_{\TTt})^\perp\cap\MHktwoi
     \,,
  &
\\
 &     
     S^{k+2i} := S\cap( \ker \overset{(i)}{\psi}_{\TTt})^\perp\cap\MHktwoi
     \,.
     &
\end{eqnarray}
%
All three spaces are  closed for $k+2i \ge 1$, and the restriction of  $\overset{(i)}{\psi}_{\TTt}$ to each of them is an isomorphism, in particular  their images by $\overset{(i)}{\psi}_{\TTt}$ are closed. This leads to the $L^2$-orthogonal splitting
(compare 
Proposition~\ref{P26X23.1})
%
\begin{equation}\label{20XII23.3}
  \MMHk= \ker \overset{(i)}{\psi}_{\TTt} \oplus
   \Big(
    \im \big(
   \overset{(i)}{\psi}_{\TTt}|_{\TTt^{k+2i}}\big) 
   \oplus
    \im \big(
   \overset{(i)}{\psi}_{\TTt}|_{V^{k+2i}}\big) 
   \oplus
    \im \big(
   \overset{(i)}{\psi}_{\TTt}|_{S^{k+2i}}\big) 
   \Big)
  \,.
\end{equation}
%
The operators  $\overset{(i)}{\psi}\ofP $ vanish on $V$ and $S$, and coincide  with $\overset{(i)}{\psi}_{\TTt}$  on $\TTt$  (compare \eqref{6III23.w9}, together with
\eqref{8XII2.g2} and \eqref{8XII23.g1}, Appendix~\ref{App8XII23.1} below).  This results, for  the $(n,\ell)$'s and $i$'s under consideration, in the desired $L^2$-orthogonal splitting
%
\begin{align}\label{20XII23.2}
  \MMHk=& \ker \overset{(i)}{\psi}_{\TTt} \oplus
   \Big(
   \underbrace{
     \im \big(
   \overset{(i)}{\psi}_{\TTt}|_{\TTt^{k+2i}}\big) 
   }_{=   \im 
   \overset{(i)}{\psi}\ofP }
   \oplus
   \underbrace{
    \im \big(
   \overset{(i)}{\psi}_{\TTt}|_{V^{k+2i}}\big) 
    }_{
     = V^k}
   \oplus
   \underbrace{
    \im \big(
   \overset{(i)}{\psi}_{\TTt}|_{S^{k+2i}}\big) 
    }_{=S^k}
   \Big)
   \nonumber
\\ 
 =&   
    \im 
   \overset{(i)}{\psi}\ofP
   \oplus
   \Big(
    \ker \overset{(i)}{\psi}_{\TTt} \oplus
  V^{k} 
   \oplus S^{k} 
   \Big)
  \,.
\end{align}
%


To finish the proof, let the pair $(n,\ell)$  be inconvenient and let $i= \frac{n-3}{2}$. Consider the operators 
%
\begin{align}
	{\cal L}_V (j) 
  &\equiv -\frac{(2+j)(4-n + j)}{(7 - n + 2 j)(3-n+j)(3+j)}\left( \zTSlap_T +(1+j)(5-n+j)\myGauss\right) 
\,,
\\
 \overset{(\frac{n-3}{2})}{\psi}_V
 & :=  \prod_{j=2}^{\frac{n-3}{2}}
   {\cal L}_V(\tfrac{n-5-2j}{2})\overset{(1)}{\psi}\ofP 
 \,;
\end{align}
%
cf.~\eqref{8XII2.g2} and \eqref{8XII23.g3}.
The operator  $\overset{(\frac{n-3}{2})}{\psi}\ofP $ vanishes on $S$ and coincides with the elliptic operators $\overset{(\frac{n-3}{2})}{\psi}_V$ on $V$ and  with $\overset{(\frac{n-3}{2})}{\psi}_{\TTt}$ on $\TTt$.


 {\blueca{23XII}
 We have the $L^2$-orthogonal splittings 
 %
 \begin{eqnarray}\label{23XII23.91}
%   V\cap \MHktwoi 
%     &= &   \ker 
%      \big(
%    \overset{(\frac{n-3}{2})}{\psi}_V |_V
%     \big)
%     \oplus 
%            \Big(
%            \underbrace{
%    \Big( \ker 
%      \big(
%    \overset{(\frac{n-3}{2})}{\psi}_V|_V
%     \big)
%    \Big)^\perp 
%    \cap \MHktwoi  
%    }_{=: V^{k+2i}}
%        \Big)
%         \,,
% \\
   (V\oplus \TTt)\cap \MHktwoi 
     &= &   \ker 
      \big(
    \overset{(\frac{n-3}{2})}{\psi}  |_{V\oplus\TTt}
     \big)
     \oplus 
            \Big(
            \underbrace{
    \Big( \ker 
      \big(
    \overset{(\frac{n-3}{2})}{\psi} |_{V\oplus\TTt}
     \big)
    \Big)^\perp 
    \cap \MHktwoi  
    }_{=: X^{k+2i}}
        \Big)
         \,,        
 %\\
%   \TTt\cap \MHktwoi 
%     &= &   \ker 
%      \big(
%    \overset{(\frac{n-3}{2})}{\psi}_{\TTt} |_{\TTt}
%     \big)
%     \oplus 
%            \Big(
%            \underbrace{
%    \Big( \ker 
%      \big(
%    \overset{(\frac{n-3}{2})}{\psi}_{\TTt} |_{\TTt}
%    \big)
%     \Big)^\perp 
%    \cap \MHktwoi  
%    }_{=: \TTt^{k+2i}}
%        \Big)
%         \,,
\\
 \MHktwoi
  & = &  
   \underbrace{
  \big(
  S\cap \MHktwoi 
  \big) \oplus \ker 
      \big(
    \overset{(\frac{n-3}{2})}{\psi}|_{V\oplus\TTt}
     \big)
     }_{= \ker  \overset{(\frac{n-3}{2})}{\psi}}
      \oplus       
         X^{k+2i} 
  \,.
 \end{eqnarray}
 %
Elliptiticity shows that the image of $X^{k+2i}$ by $ \overset{(\frac{n-3}{2})}{\psi}$ is $L^2$-closed and equals $X^{k}$, leading to
 %
 \begin{eqnarray}\label{23XII23.92}
 \MHk
  & = &   
  \big(
  S\cap \MHk
  \big) \oplus \ker 
      \big(
    \overset{(\frac{n-3}{2})}{\psi}|_{V\oplus\TTt}
     \big) 
      \oplus       
      \underbrace{   X^{k}
      }_{\im 
          \overset{(\frac{n-3}{2})}{\psi}
          }
  \,.
 \end{eqnarray}
 % 
 The first two summands are $L^2$-closed, and the result follows by Lemma~\ref{L18XI23.1bx}.
 } 
 
%Since $V\cap\MHk$ is closed for any $k\ge 1$, the image of the restriction of $\overset{(\frac{n-3}{2})}{\psi}_V$ to $V$ is closed.  
%Then
%%
%$$
% \im \overset{(\frac{n-3}{2})}{\psi}\ofP =  \overset{(\frac{n-3}{2})}{\psi}_V (V) \oplus  \overset{(\frac{n-3}{2})}{\psi}_{\TTt}(\TTt)
%$$
%%
%which is a sum of closed spaces, hence closed. This ends the proof 
% that the $ \im_k 
% \overset{(i)}{\psi}  $'s are closed in the $\MHk$-topology. 
 }
%
\qed
%


==> regularity.tex <==
\subsection{Add-on on regularity}

Note that the current choices of $s_i$ and $t_j$'s do not give the required regularity. From fig. \ref{f10IX23.2}, we have:
%
$$
 s = \max(s_i) = 2k+2 
  \,.
$$
%
The problem arises from the last few rows, for $\overadd{i}{r}$, with $i\geq \frac{n+1}{2}$. Recall that we have
%
$$\overadd{i}{r} \sim \zspaceD^A \partial_u^i h_{AB} \in H^{k_{\gamma}-2i-1}. $$
%
Thus, in order to make use of the estimate \eqref{27XI23.1}, we need for the corresponding $i$'s,
%
$$ s-s_i +\ell \leq k_{\gamma}-2i-1 \implies \ell \leq k_{\gamma} - 2k -3 \,.$$
%
However, this gives lower than required regularities for e.g. the $\TTtpvec{p}$'s: recall that $C(\TTtpvec{p}) = \overadd{p}{\varphi}$, and so we require $\TTtpvec{p} \in H^{k_{\gamma}+ 1}$; but the estimate \eqref{27XI23.1} only gives a bound for $||\TTtpvec{p}||_{H^{s+t_j+\ell}}$, and  (noting that $t_j$'s are zero) we have $ s+t_j+\ell\leq 2k+2+k_{\gamma} - 2k -3= k_{\gamma}  -1$.

\paragraph{Resolution.} One possible resolution would be to change the $s_i$'s and $t_j$'s corresponding to region C, see the new figs \ref{f10IX23.1a}-\ref{f10IX23.2b}, but this also requires moving the respective rows and columns to the beginning in order to keep $\Lambda_k^{[0,X]}$ lower triangular (because now those operators for the $\overadd{i}{s}$ rows in region B, will have order $ = s_i+t_j$ and is thus non-vanishing in the principle part of $\Lambda_k$). It can be verified that with this choice, (i) $\Lambda_k^{[0,X]}$ remains lower triangular, (ii) for each $(i,j)$-entry, the order of the operator lying there is $\leq s_i + t_j$, and thus the ADN criterion for ellipticity is met. These follow the same reasoning as before.

Moreover, this does give the required regularities for all $v_j$'s. Indeed for each $\overadd{i}{r}$ or $\overadd{i}{s}$'s, we now have $s_i = 2(i+1)$. Meanwhile, the regularities of these fields are $H^{k_{\gamma}-2i-1}$. Thus we need
%
$$ s-s_i + \ell \leq k_{\gamma}-2i-1 \implies \ell \leq k_{\gamma}-2k-1\,,$$
%
so in particular, we can take $\ell = k_{\gamma}-2k-1$. From \eqref{27XI23.1}, we have $(v_k)_j \in H^{s+t_j+\ell} =H^{k_{\gamma} + 1+t_j} $. Thus:
%
\begin{align}
    i \in [1, k_n]: \ \partial_u^i \kxi{2}_A &\in H^{k_{\gamma} + 1 - 2i}\,,
    \nn
    \\
    \text{all other $(v_{k})_j$'s}: \ (v_{k})_j  &\in H^{k_{\gamma} + 1}\,,
\end{align}
%
which are exactly the required regularities (cf. e.g. \eqref{28VIII23.4}).

\input{LambdakReg}

Simple example of system where different choices of $s_i$'s and $t_j$'s lead to different regularities:
%
\begin{align}
    \begin{pmatrix}
        u_1
        \\
        u_2
    \end{pmatrix} =
    \underbrace{\begin{pmatrix}
        \Delta^2 & \Delta \\
        \Delta^2 & \Delta^2
    \end{pmatrix}}_{=: L}
    \begin{pmatrix}
        v_1
        \\
        v_2
    \end{pmatrix}\,.
\end{align}
%
We can choose 
%
\begin{align}
    \text{either}: (s_i) &= (4,4) \,\quad (t_j) = (0,0)\\
    \text{or}:     (s_i) & = (4,6) \, \quad (t_j) = (0,-2)\,.
\end{align}
%
Keeping only the operators of order $s_i+t_j$ at the $(ij)$-th entry leads to (and denoting the resulting matrix as $L^{[0]}$):
%
\begin{align}
    \text{either}: 
    L^{[0]}(D) = \begin{pmatrix}
        \Delta^2 & 0 \\
        \Delta^2 & \Delta^2
    \end{pmatrix}  \implies  L^{[0]}(k)= \begin{pmatrix}
        |k|^4 & 0 \\
        |k|^4 & |k|^4
    \end{pmatrix}\\
    \text{or}:  
     L^{[0]}(D) = 
    \begin{pmatrix}
        \Delta^2 & \Delta \\
        0 & \Delta^2
    \end{pmatrix}
    \implies  L^{[0]}(k)= \begin{pmatrix}
        |k|^4 & |k|^2 \\
        0 & |k|^4
        \end{pmatrix}
        \,.
\end{align}
%
In either case, $\det L^{[0]}(k) \neq 0$ for $k\neq 0$, so both choices satisfy the ADN conditions. However for the first, we get from the ADN estimates $v_1 \in H_{4+\ell}, v_2 \in H_{4+\ell}$ while for the second, $v_1 \in H_{6+\ell}, v_2 \in H_{4+\ell}$.
\newpage 

==> tildeK1V.tex <==
 Finally, the operator $\mathcal{\tilde K}(-1,\ofDCnoDC) $, acting on divergenceless vectors, $\zspaceD^A\xi _A=0 $, takes the form
 %
 \begin{align}
     \mathcal{\tilde K}(-1,\ofDCnoDC) (\xi )_B
     & = -\frac{n-1}{(n-2)(n-5)} \zspaceD^A \circ C(\xi)_{AB} + \frac{1}{n-5}\TSzlap\xi_B
     \nonumber
     \\
     & =
     -\frac{n-1}{2(n-2)(n-5)} \zspaceD^A (\zspaceD_A\xi_B + \zspaceD_B\xi_A) + \frac{1}{n-5}\TSzlap\xi_B  \,,
 \end{align}
 %
can also be shown to be elliptic by a straightforward calculation of its symbol.  
